Two mixed finite element formulations for the weak imposition of the Neumann boundary conditions for the Darcy flow

We propose two different discrete formulations for the weak imposition of the Neumann boundary conditions of the Darcy flow. The Raviart-Thomas mixed finite element on both triangular and quadrilateral meshes is considered for both methods. One is a consistent discretization depending on a weighting parameter scaling as $\mathcal O(h^{-1})$, while the other is a penalty-type formulation obtained as the discretization of a perturbation of the original problem and relies on a parameter scaling as $\mathcal O(h^{-k-1})$, $k$ being the order of the Raviart-Thomas space. We rigorously prove that both methods are stable and result in optimal convergent numerical schemes with respect to appropriate mesh-dependent norms, although the chosen norms do not scale as the usual $L^2$-norm. However, we are still able to recover the optimal a priori $L^2$-error estimates for the velocity field, respectively, for high-order and the lowest-order Raviart-Thomas discretizations, for the first and second numerical schemes. Finally, some numerical examples validating the theory are exhibited.

==> Sections/burman.tex <==
Let $V_h\times Q_h$ be the Raviart-Thomas isogeometric element. Let us impose an extra constraint in order to filter out constant pressures:
\begin{equation*}
Q_I:=\{q_h\in Q_h: \int_{\Omega_{\mathcal T_I}}q_h=0\}.
\end{equation*}
where $\Omega_{\mathcal T_I}:=\Omega_{\mathcal T}\setminus \bigcup_{\Gamma_K\ne\emptyset}{K}$. Then, let us stabilize the whole pressure space:
\begin{equation*}
R_h\left(Q_I\right):=\{R_h\left(q_h\right): q_h\in Q_I\}.
\end{equation*}


Find $\left(\u_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ such that
\begin{equation}\label{burman_prob}
\begin{cases}
a_h(\u_h,\v_h)-&b_1(\v_h,p_h)= \int_{\Omega}\f\cdot \v_h\qquad\forall\ \v_h\in V_h \\
&b_0(\u_h,q_h)= 0\qquad\forall\ q_h\in R_h\left(Q_I\right),
\end{cases}
\end{equation}
where
\begin{equation*}
\begin{aligned}
a_h(\u_h,\v_h)&:=\int_{\Omega} D\u_h : D\v_h -\int_{\Gamma} R_h(\u_h)\cdot\v_h-\int_{\Gamma} \u_h\cdot R_h(\v_h) + \beta\int_{\Gamma}h^{-1}\u_h\cdot\v_h \\
b_m(\v_h,q_h)&:=\int_{\Omega}q_h\dive \v_h -m\int_{\Gamma}q_h\left(\v_h\cdot\n\right)\qquad m\in\{0,1\}
\end{aligned}
\end{equation*}
In order to prove stability, let us follow the following strategy. Fix $\left(\v_h,q_h\right)\in V_h\times R_h\left(Q_I\right)$. We need to construct/find $\left(\w_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ such that
\begin{enumerate}
\item $\norm{\left(\v_h,q_h\right)}^2\le C_1 \mathcal A\left(\left(\v_h,q_h\right),\left(\w_h,p_h\right) \right)$
\item $\norm{\left(\w_h,p_h\right)}\le C_2\norm{\left(\v_h,q_h\right)}$	
\end{enumerate}	


\begin{lemma}
\begin{equation}\label{1.4}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h)
\end{equation}	
\end{lemma}	
\begin{proof}
Let $\left(\u_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ be the solution to~\eqref{burman_prob}. Using Cauchy-Schwarz, the stability property of $R_h$ and Young's inequality with $\varepsilon:=\alpha$:
\begin{equation*}
\begin{aligned}
\abs{-b_1(\u_h,p_h)+b_0(\u_h,p_h)}\le& \norm{h^{\frac{1}{2}}p_h}_{L^2(\Gamma)}\norm{h^{-\frac{1}{2}}\u_h}_{L^2(\Gamma)}\le  C_S\norm{p_h}_{L^2(\Omega_{\mathcal T_I})}\norm{\u_h}_{1,h} \\
\le & \frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}+\frac{\alpha}{2}\norm{\u_h}^2_{1,h}.
\end{aligned}
\end{equation*}
Hence,
\begin{equation*}
 -\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\alpha}{2}\norm{\u_h}^2_{1,h}\le-b_1(\u_h,p_h)+b_0(\u_h,p_h).
\end{equation*}
By coercivity $\alpha\norm{\u_h}^2_{1,h}\le a_h(\u_h,\u_h)$, so
\begin{equation*}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h).
\end{equation*}
\end{proof}	

\begin{lemma}
	\begin{equation}\label{1.5}
	\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{C_I^2}{2}\norm{\u_h}^2_{1,h}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation}	
\end{lemma}	
\begin{proof}
Given $p_h\in R_h\left( Q_h\right)$, in particular $\restr{p_h}{\Omega_{\mathcal T_I}}\in L^2_0(\Omega_{\mathcal T_I})$, there exists $\v_p\in \left[H_0^1\left(\Omega_{\mathcal T_I}\right)\right]^2$ such that
\begin{equation}
\begin{cases}
-\dive \v_{p} &= \restr{p_h}{\Omega_{\mathcal T_I}} \quad\text{in}\;\Omega_{\mathcal T_I} \\
 \v_{p}\cdot\n &= 0 \quad\text{on}\;\partial\Omega_{\mathcal T_I} 
\end{cases}
\end{equation}
Burman says $\v_{p,h}:=\pi_{V_h}\v_p\in \left[H_0^1\left(\Omega_{\mathcal T_I}\right)\right]^2\cap V_h$. In particular it holds
\begin{equation}
-\dive \v_{p,h} = p_h \quad\text{in}\;\Omega_{\mathcal T_I},\; \norm{D \v_{p,h}}_{L^2(\Omega)}\le C_I \norm{p_h}_{L^2(;\Omega_{\mathcal T_I})}
\end{equation}
Let $\u_h$ be the solution for the velocity field. Since using $\restr{\v_{p,h}}{\Gamma}=0$
\begin{equation*}
\abs{a_h(\u_h,\v_{p,h})}\le \norm{D \u_h}_{L^2(\Omega_{\mathcal T_I})}\norm{D \v_{p,h}}_{L^2(\Omega_{\mathcal T_I})}
\end{equation*}	
By Young's inequality
\begin{equation*}
a_h(\u_h,\v_{p,h})\ge -\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\eps}{2}\norm{D \v_{p,h}}^2_{L^2(\Omega_{\mathcal T_I})}
\end{equation*}	
Again, since $\restr{\v_{p,h}}{\Gamma}=0$
\begin{equation*}
-b_1(\v_{p,h},p_h)= \norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}.
\end{equation*}	
So,
\begin{equation*}
-\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\eps}{2}\norm{D \v_{p,h}}^2_{L^2(\Omega_{\mathcal T_I})}+\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Using $ \norm{D \v_{p,h}}_{L^2(\Omega)}\le C_I \norm{p_h}_{L^2(;\Omega_{\mathcal T_I})}$
\begin{equation*}
-\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}+\left(1-\frac{\eps C_I^2}{2}\right)\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Choose $\eps>0$ such that $1-\frac{\eps C_I^2}{2}=\frac{1}{2}$, i.e. $\eps = \frac{1}{C_I^2}$, so that
\begin{equation*}
\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_I^2}{2}  \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Using $\norm{D \u_h}_{L^2(\Omega_{\mathcal T_I})}\le \norm{\u_h}_{1,h}$
\begin{equation*}
\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_I^2}{2}  \norm{\u_h}^2_{1,h}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
\end{proof}	

\begin{lemma}
\begin{equation*}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h} + \frac{\alpha}{8C_I^2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} -\frac{C^2}{2\alpha\gamma}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\w_h) - b_1(\w_h,p_h)
\end{equation*}	
\end{lemma}	
\begin{proof}
Let us compute \eqref{1.4}$+\frac{\alpha}{4C_I^2}$\eqref{1.5}:
\begin{equation*}
\begin{aligned}
\frac{1}{2}\frac{\alpha}{4C_I^2}&\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}+\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\norm{\u_h}^2_{1,h}\\
\le& a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h) + \frac{\alpha}{4C_I^2}a_h(\u_h,\v_{p,h})-\frac{\alpha}{4C_I^2}b_1(\v_{p,h},p_h)
\end{aligned}
\end{equation*}	
Let us define $\w_h:=\u_h+\frac{\alpha}{4C_I^2}\v_{p,h}$
\begin{equation*}
\begin{aligned}
	\left(\frac{1}{2}\frac{\alpha}{4C_I^2}-\frac{C_S^2}{2\alpha}\right)&\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} +\left(\frac{\alpha}{2}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\right) \norm{\u_h}^2_{1,h}\\
	\le & a_h(\u_h,\w_h)-b_1(\w_h,p_h)+b_0(\u_h,p_h)
\end{aligned}
\end{equation*}	
and we have
\begin{equation*}
\begin{aligned}
\frac{\alpha^2-4C_I^2C_S^s}{8\alpha C_I^2}&\norm{p_h}^2_{L^2(\Omega)}+\left(\frac{3\alpha}{8}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\right) \norm{\u_h}^2_{1,h}\\
\le & a_h(\u_h,\w_h)-b_1(\w_h,p_h)+b_0(\u_h,p_h)
\end{aligned}
\end{equation*}	
Attention, in general $\frac{\alpha^2-4C_I^2C_S^s}{8\alpha C_I^2}$ is negative!
\end{proof}	


==> Sections/burman_2.tex <==
Let $V_h\times Q_h$ be the Raviart-Thomas isogeometric element. Let us impose an extra constraint in order to filter out constant pressures:
\begin{equation*}
Q_I:=\{q_h\in Q_h: \int_{\Omega_{\mathcal T_I}}q_h=0\}.
\end{equation*}
where $\Omega_{\mathcal T_I}:=\Omega_{\mathcal T}\setminus \bigcup_{\Gamma_K\ne\emptyset}{K}$. Then, let us stabilize the whole pressure space:
\begin{equation*}
R_h\left(Q_I\right):=\{R_h\left(q_h\right): q_h\in Q_I\}.
\end{equation*}


Find $\left(\u_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ such that
\begin{equation}\label{burman_prob}
\begin{cases}
a_h(\u_h,\v_h)-&b_1(\v_h,p_h)= \int_{\Omega}\f\cdot \v_h\qquad\forall\ \v_h\in V_h \\
&b_0(\u_h,q_h)= 0\qquad\forall\ q_h\in R_h\left(Q_I\right),
\end{cases}
\end{equation}
where
\begin{equation*}
\begin{aligned}
a_h(\u_h,\v_h)&:=\int_{\Omega} D\u_h : D\v_h -\int_{\Gamma} R_h(\u_h)\cdot\v_h-\int_{\Gamma} \u_h\cdot R_h(\v_h) + \beta\int_{\Gamma}h^{-1}\u_h\cdot\v_h \\
b_m(\v_h,q_h)&:=\int_{\Omega}q_h\dive \v_h -m\int_{\Gamma}q_h\left(\v_h\cdot\n\right)\qquad m\in\{0,1\}
\end{aligned}
\end{equation*}
In order to prove stability, let us follow the following strategy. Fix $\left(\v_h,q_h\right)\in V_h\times R_h\left(Q_I\right)$. We need to construct/find $\left(\w_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ such that
\begin{enumerate}
\item $\norm{\left(\v_h,q_h\right)}^2\le C_1 \mathcal A\left(\left(\v_h,q_h\right),\left(\w_h,p_h\right) \right)$
\item $\norm{\left(\w_h,p_h\right)}\le C_2\norm{\left(\v_h,q_h\right)}$	
\end{enumerate}	


\begin{lemma}
\begin{equation}\label{1.4}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h)
\end{equation}	
\end{lemma}	
\begin{proof}
Let $\left(\u_h,p_h\right)\in V_h\times R_h\left(Q_I\right)$ be the solution to~\eqref{burman_prob}. Using Cauchy-Schwarz, the stability property of $R_h$ and Young's inequality with $\varepsilon:=\alpha$:
\begin{equation*}
\begin{aligned}
\abs{-b_1(\u_h,p_h)+b_0(\u_h,p_h)}\le& \norm{h^{\frac{1}{2}}p_h}_{L^2(\Gamma)}\norm{h^{-\frac{1}{2}}\u_h}_{L^2(\Gamma)}\le  C_S\norm{p_h}_{L^2(\Omega_{\mathcal T_I})}\norm{\u_h}_{1,h} \\
\le & \frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}+\frac{\alpha}{2}\norm{\u_h}^2_{1,h}.
\end{aligned}
\end{equation*}
Hence,
\begin{equation*}
 -\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\alpha}{2}\norm{\u_h}^2_{1,h}\le-b_1(\u_h,p_h)+b_0(\u_h,p_h).
\end{equation*}
By coercivity $\alpha\norm{\u_h}^2_{1,h}\le a_h(\u_h,\u_h)$, so
\begin{equation*}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h).
\end{equation*}
\end{proof}	

\begin{lemma}
	\begin{equation}\label{1.5}
	\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{C_I^2}{2}\norm{\u_h}^2_{1,h}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation}	
\end{lemma}	
\begin{proof}
Given $p_h\in R_h\left( Q_h\right)$, in particular $\restr{p_h}{\Omega_{\mathcal T_I}}\in L^2_0(\Omega_{\mathcal T_I})$, there exists $\v_p\in \left[H_0^1\left(\Omega_{\mathcal T_I}\right)\right]^2$ such that
\begin{equation}
\begin{cases}
-\dive \v_{p} &= \restr{p_h}{\Omega_{\mathcal T_I}} \quad\text{in}\;\Omega_{\mathcal T_I} \\
 \v_{p}\cdot\n &= 0 \quad\text{on}\;\partial\Omega_{\mathcal T_I} 
\end{cases}
\end{equation}
Burman says $\v_{p,h}:=\pi_{V_h}\v_p\in \left[H_0^1\left(\Omega_{\mathcal T_I}\right)\right]^2\cap V_h$. In particular it holds
\begin{equation}
-\dive \v_{p,h} = p_h \quad\text{in}\;\Omega_{\mathcal T_I},\; \norm{D \v_{p,h}}_{L^2(\Omega)}\le C_I \norm{p_h}_{L^2(;\Omega_{\mathcal T_I})}
\end{equation}
Let $\u_h$ be the solution for the velocity field. Since using $\restr{\v_{p,h}}{\Gamma}=0$
\begin{equation*}
\abs{a_h(\u_h,\v_{p,h})}\le \norm{D \u_h}_{L^2(\Omega_{\mathcal T_I})}\norm{D \v_{p,h}}_{L^2(\Omega_{\mathcal T_I})}
\end{equation*}	
By Young's inequality
\begin{equation*}
a_h(\u_h,\v_{p,h})\ge -\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\eps}{2}\norm{D \v_{p,h}}^2_{L^2(\Omega_{\mathcal T_I})}
\end{equation*}	
Again, since $\restr{\v_{p,h}}{\Gamma}=0$
\begin{equation*}
-b_1(\v_{p,h},p_h)= \norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}.
\end{equation*}	
So,
\begin{equation*}
-\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}-\frac{\eps}{2}\norm{D \v_{p,h}}^2_{L^2(\Omega_{\mathcal T_I})}+\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Using $ \norm{D \v_{p,h}}_{L^2(\Omega)}\le C_I \norm{p_h}_{L^2(;\Omega_{\mathcal T_I})}$
\begin{equation*}
-\frac{1}{2\eps} \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}+\left(1-\frac{\eps C_I^2}{2}\right)\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Choose $\eps>0$ such that $1-\frac{\eps C_I^2}{2}=\frac{1}{2}$, i.e. $\eps = \frac{1}{C_I^2}$, so that
\begin{equation*}
\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_I^2}{2}  \norm{D \u_h}^2_{L^2(\Omega_{\mathcal T_I})}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
Using $\norm{D \u_h}_{L^2(\Omega_{\mathcal T_I})}\le \norm{\u_h}_{1,h}$
\begin{equation*}
\frac{1}{2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_I^2}{2}  \norm{\u_h}^2_{1,h}\le a_h(\u_h,\v_{p,h})-b_1(\v_{p,h},p_h)
\end{equation*}
\end{proof}	

\begin{lemma}
\begin{equation*}
\frac{\alpha}{2}\norm{\u_h}^2_{1,h} + \frac{\alpha}{8C_I^2}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} -\frac{C^2}{2\alpha\gamma}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} \le a_h(\u_h,\w_h) - b_1(\w_h,p_h)
\end{equation*}	
\end{lemma}	
\begin{proof}
Let us compute \eqref{1.4}$+\frac{\alpha}{4C_I^2}$\eqref{1.5}:
\begin{equation*}
\begin{aligned}
\frac{1}{2}\frac{\alpha}{4C_I^2}&\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} - \frac{C_S^2}{2\alpha}\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})}+\frac{\alpha}{2}\norm{\u_h}^2_{1,h}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\norm{\u_h}^2_{1,h}\\
\le& a_h(\u_h,\u_h)-b_1(\u_h,p_h)+b_0(\u_h,p_h) + \frac{\alpha}{4C_I^2}a_h(\u_h,\v_{p,h})-\frac{\alpha}{4C_I^2}b_1(\v_{p,h},p_h)
\end{aligned}
\end{equation*}	
Let us define $\w_h:=\u_h+\frac{\alpha}{4C_I^2}\v_{p,h}$
\begin{equation*}
\begin{aligned}
	\left(\frac{1}{2}\frac{\alpha}{4C_I^2}-\frac{C_S^2}{2\alpha}\right)&\norm{p_h}^2_{L^2(\Omega_{\mathcal T_I})} +\left(\frac{\alpha}{2}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\right) \norm{\u_h}^2_{1,h}\\
	\le & a_h(\u_h,\w_h)-b_1(\w_h,p_h)+b_0(\u_h,p_h)
\end{aligned}
\end{equation*}	
and we have
\begin{equation*}
\begin{aligned}
\frac{\alpha^2-4C_I^2C_S^s}{8\alpha C_I^2}&\norm{p_h}^2_{L^2(\Omega)}+\left(\frac{3\alpha}{8}-\frac{C_I^2}{2}\frac{\alpha}{4C_I^2}\right) \norm{\u_h}^2_{1,h}\\
\le & a_h(\u_h,\w_h)-b_1(\w_h,p_h)+b_0(\u_h,p_h)
\end{aligned}
\end{equation*}	
Attention, in general $\frac{\alpha^2-4C_I^2C_S^s}{8\alpha C_I^2}$ is negative!
\end{proof}	


==> Sections/introduction.tex <==
\section{Introduction}
Complex models are processed within Computer Aided Design (CAD) tools where several geometric manipulations are possible. Geometries are described as collection of their boundary surfaces, often defined as tensor-product splines or NURBS, and during the design process these surfaces can be joined, intersected or simply superflous parts can be cut away. All these Boolean operations act on the original surfaces through a common procedure of trimming. When part of a surface is cut away by trimming, the visualization of the geometric object in CAD tools is adapted, but the mathematical description of the surface, \textcolor{magenta}{given by the original surface along with the trimming curves}, remains. This description of the geometry is called ``boundary representation'' (B-rep), and we defer the interested reader to \cite{piegl_ten_2005,Stroud2006}, or to the recent review \cite{Marussig2017} and references therein. This representation is clearly not well suited for the simulation of partial differential equations (PDEs).

Several efforts have been undertaken in the last years to improve the usability of CAD geometries in the solution of PDEs, especially after the advent of Isogeometric Analysis (IGA) \cite{Cottrell:2009:IAT:1816404,HUGHES20054135}. Indeed, IGA has been a tremendous success since 2005 with a wide range of applications (see for instance \textcolor{magenta}{the special issue \cite{CMAME-IGA2017}}), and it is becoming a \textcolor{magenta}{mature method}: its mathematical analysis is now well understood \cite{buffa}, fast assembly and solvers exist today \cite{MR3761002,MR3811621} and strategies for adaptive refinement with a sound mathematical theory are now available, see \cite{1078-0947_2019_1_241} and the references therein. The geometric modelling community has also provided important inputs to this scientific challenge \cite{Cohen15}, and new strategies to define geometric entities through the volume they occupy instead of their boundaries are now emerging, for instance, the volumetric representations (V-reps) proposed in \cite{Massarwi}. On the other hand, trimming remains a main tool for the design of complex models via Boolean operations, and basically all developments of IGA described above rely on strong requirements on the underlying geometric models and, in general, do not support trimmed geometric entities. The aim of this paper is to contribute to the design of isogeometric methods that robustly support trimming in the geometric description of the computational domain, and do not require the construction of a global re-parametrization (meshing).


The two main issues arising when dealing with trimmed geometries are the presence of elements unfitted with the boundary, making the research for efficient quadrature rules and the stable imposition of boundary conditions a challenge, and the existence of basis functions whose support has been cut, affecting the conditioning of the related linear system. In this regard, ideas from fictitious domain and immersed boundary approaches in the FEM literature can be adapted to the IGA setting, and the related engineering literature includes (but is not limited to) the pioneering works regarding the integration with CAD and numerical quadrature \cite{NAGY2015165,Wang2015}, the shell analysis on geometric models with B-reps \cite{BREITENBERGER2015401,PHILIPP2016312}, and the finite cell method combined with IGA \cite{Dauge2015,RANK2012104,MR3003066,MR3706626}. \textcolor{magenta}{I would remove \cite{Dauge2015} (it is $p$-FEM)} Concerning the lack of stability, we should mention stabilizations based on extrapolation \cite{ doi:10.1137/S0036142900373208,MARUSSIG201879}, and the Cut-IGA method proposed in \cite{1812.08568}, which is related to the many contributions of Cut-FEM and ghost penalty methods \cite{BURMAN20101217,NME:NME4823,BURMAN2012328,Burman2012,Hansbo434217}.

We now describe the simplified mathematical setting. Let $\Omega_0\subseteq \R^d$ (here $d=2,3$)  be a domain described by a bijective spline map $\mathbf{F}: (0,1)^d \to \Omega_0$, i.e., a patch in the isogeometric terminology, and let $\Omega_1,\ldots \Omega_N$ be Lipschitz regular domains in $\R^d$. We assume that $\bigcup_{i=1}^N\overline{\Omega}_i$ are to be cut away from $\Omega_0$ and that our computational domain reads:  
\begin{equation}\label{48}
\Omega=\Omega_0\setminus\bigcup_{i=1}^N\overline{\Omega}_i.
\end{equation}
After trimming the mathematical description of the domain remains unchanged, that is, the elements and basis functions fit the boundary of $\Omega_0$ instead of that of $\Omega$. In this paper, we focus on a simple Poisson problem, with weakly imposed boundary conditions, on the domain $\Omega$ described above. First of all, we discuss the difference between bad matrix conditioning and lack of stability. The first one can be improved by modifying the chosen basis (preconditioning), while the second one needs to act on the bilinear form directly. 

Regarding the lack of stability, we propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that affect stability. For example, in the case of a Neumann condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements. For the stabilization we follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two different versions of the stabilization technique. The first one in the parametric domain, easier to implement from the numerical point of view, but suboptimal. The second , a projection-based stabilization performed directly on the physical domain, which allows us to recover optimal a priori error estimates.

Concerning the bad conditioning of the matrix, we show numerical evidence that a rescaling of the stiffness matrix seems to consistently  resolve the issue. However, the analysis on the linear algebra side is not presented, as it is beyond the scope of this work.

The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. %An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization technique. Two possible constructions of the stabilization operator are suggested and analysed in Section~\ref{sec:construction}, and error estimates are provided in Section~\ref{sec:estimate}. 
Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs \cite{VAZQUEZ2016523}, confirming the theoretical results.


%Complex models are processed within Computer Aided Design (CAD) tools where several geometric manipulations are possible. One procedure that is  basically ubiquitous is \emph{trimming}. Geometries are described as collection of  surfaces that can be joined, intersected or simply superflous parts can be cut away. Often surfaces are bivariate splines or NURBS surfaces and this representation is called ``boundary representation'' (B-rep).  We defer the interested reader to \cite{piegl_ten_2005,Stroud2006}, or to the recent review \cite{Marussig2017} and the references there in. 

%When superflous parts are cut away, the geometric object changes but its mathematical description does not. Clearly this representation is not well suited for the simulation of PDEs and, as a matter of fact, several efforts have been undertaken in the last years to improve the usability of CAD geometries in analysis, especially after the advent of Isogeometric Analysis (IGA) \cite{Cottrell:2009:IAT:1816404,HUGHES20054135}. Indeed, since 2005, also the geometric modelling community has provided important inputs to this scientific challenge \cite{Cohen15} and new strategies to define geometric entities through the volume they occupy instead of their boundaries are now emerging. For instance, in \cite{Massarwi} volumetric representations (V-reps) are proposed as a new, more analysis friendly, geometric design paradigm. On the other hand, trimming remains a main tool allowing for the design of complex models via Boolean operations (such as union, intersection, difference). Thus, in order to guarantee interoperability, in the spirit of isogeometric analysis, we wish to  design tools for the approximation of PDEs that support trimming in the geometric description of the computational domain and do not require the construction of global re-parametrization (meshing). 

%Indeed, isogeometric analysis has been a tremendous success since 2005. It has been successfully applied to many problems, from elasticity \cite{laura18b,MR3610117,Cottrell:2009:IAT:1816404,laura14,MR3196811}, to phase fields models \cite{MR3527591}, to fracture analysis \cite{laura16}, to electromagnetics \cite{mio2,mio1}; its mathematical analysis is now well understood \cite{buffa}, fast assembly and solvers exist today \cite{MR3761002,MR3811621} and strategies for local refinements are now well understood, also from a mathematical stand point e.g., \cite{1078-0947_2019_1_241} and the references therein. This list could continue long.


%On the other hand, basically all developments described above rely on strong requirements on the underlying geometric models and, in general, do not support trimmed geometric entities. The aim of this paper is to contribute to the design of isogeometric methods that robustly support  the use of trimmed geometries.   

%We consider the following simplified situation. Let $\Omega_0\subseteq \R^d$   (here $d=2,3$)  be a domain described by a bijective spline map $\mathbf{F}: (0,1)^d \to \Omega_0$, i.e., a patch in the isogeometric terminology and let $\Omega_1,\ldots \Omega_N$ be Lipschitz regular domains in $\R^d$. We assume that $\bigcup_{i=1}^N\overline{\Omega}_i$ are to be cut away from $\Omega_0$ and that our computational domain reads:  
%\begin{equation}\label{48}
%\Omega=\Omega_0\setminus\bigcup_{i=1}^N\overline{\Omega}_i. 
%\end{equation}
%Let us put ourselves in a situation in which we want to numerically approximate a PDE in a computational domain of the type \eqref{48}. 
%When the superfluous surface areas are cut away, the mathematical description of the domain remains unchanged. It turns out that we have to deal with elements unfitted with the boundary, making the research for efficient quadrature rules and the imposition of boundary conditions a challenge. Moreover there are basis functions, whose support has been cut, affecting the conditioning of the related linear system. In this regard, ideas from fictitious domain and immersed boundary approaches in the FEM literature come to help.

%Indeed, the related engineering literature includes (but is not limited to) the pioneering work  \cite{NAGY2015165,Wang2015} or \cite{BREITENBERGER2015401,PHILIPP2016312} for shell analysis and the finite cell method \cite{Dauge2015,RANK2012104,MR3003066,MR3706626}. 

%In order to guarantee robustness, some stabilization is needed, and our work is related to the previous contributions in this context. In particular, we should mention stabilizations based on extrapolation \cite{ doi:10.1137/S0036142900373208,MARUSSIG201879}, and the Cut-Iga method proposed in \cite{1812.08568},  which is related to the many contributions \cite{BURMAN20101217,NME:NME4823,BURMAN2012328,Burman2012,Hansbo434217}.

%In this paper, we focus on a simple Poisson problem on the domain $\Omega$ described above, with weakly imposed boundary conditions. First of all, we discuss the difference between bad matrix conditioning and lack of stability. The first one can be improved by modifying the chosen basis (preconditioning), while the second one needs to act on the bilinear form directly. 

%Regarding the lack of stability, we propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that generate the lack of stability. For example, in the case of Neumann boundary condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements. For the stabilization we follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two different versions of the stabilization technique. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allows us to recover optimal a priori error estimates.

%Concerning the bad conditioning of the matrix, we show numerical evidence that a rescaling of stiffness matrix seems to consistently  resolve the issue. However, the analysis on the linear algebra side is not presented, as it is beyond the scope of this work. 

%We propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that generate lack of stability, and leave all issues concerning bad conditioning to a further analysis on the linear algebra side. For example, in the case of Neumann boundary condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements.  Moreover, a rescaling of stiffness matrix seems to consistently  resolve the issue of bad conditioning. 

%The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, the Poisson equation in a trimmed domain, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
%After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization technique. 
%%We follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two new stabilization techniques. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allow us to recover optimal a priori error estimates.
%Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs \cite{VAZQUEZ2016523}, confirming the theoretical results.

%The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, the Poisson equation in a trimmed domain, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
%After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization. We follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two new stabilization techniques. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allow us to recover optimal a priori error estimates.
%Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs (\cite{VAZQUEZ2016523}), confirming the theoretical results.
%


==> Sections/introduction_2.tex <==
\section{Introduction}
Complex models are processed within Computer Aided Design (CAD) tools where several geometric manipulations are possible. Geometries are described as collection of their boundary surfaces, often defined as tensor-product splines or NURBS, and during the design process these surfaces can be joined, intersected or simply superflous parts can be cut away. All these Boolean operations act on the original surfaces through a common procedure of trimming. When part of a surface is cut away by trimming, the visualization of the geometric object in CAD tools is adapted, but the mathematical description of the surface, \textcolor{magenta}{given by the original surface along with the trimming curves}, remains. This description of the geometry is called ``boundary representation'' (B-rep), and we defer the interested reader to \cite{piegl_ten_2005,Stroud2006}, or to the recent review \cite{Marussig2017} and references therein. This representation is clearly not well suited for the simulation of partial differential equations (PDEs).

Several efforts have been undertaken in the last years to improve the usability of CAD geometries in the solution of PDEs, especially after the advent of Isogeometric Analysis (IGA) \cite{Cottrell:2009:IAT:1816404,HUGHES20054135}. Indeed, IGA has been a tremendous success since 2005 with a wide range of applications (see for instance \textcolor{magenta}{the special issue \cite{CMAME-IGA2017}}), and it is becoming a \textcolor{magenta}{mature method}: its mathematical analysis is now well understood \cite{buffa}, fast assembly and solvers exist today \cite{MR3761002,MR3811621} and strategies for adaptive refinement with a sound mathematical theory are now available, see \cite{1078-0947_2019_1_241} and the references therein. The geometric modelling community has also provided important inputs to this scientific challenge \cite{Cohen15}, and new strategies to define geometric entities through the volume they occupy instead of their boundaries are now emerging, for instance, the volumetric representations (V-reps) proposed in \cite{Massarwi}. On the other hand, trimming remains a main tool for the design of complex models via Boolean operations, and basically all developments of IGA described above rely on strong requirements on the underlying geometric models and, in general, do not support trimmed geometric entities. The aim of this paper is to contribute to the design of isogeometric methods that robustly support trimming in the geometric description of the computational domain, and do not require the construction of a global re-parametrization (meshing).


The two main issues arising when dealing with trimmed geometries are the presence of elements unfitted with the boundary, making the research for efficient quadrature rules and the stable imposition of boundary conditions a challenge, and the existence of basis functions whose support has been cut, affecting the conditioning of the related linear system. In this regard, ideas from fictitious domain and immersed boundary approaches in the FEM literature can be adapted to the IGA setting, and the related engineering literature includes (but is not limited to) the pioneering works regarding the integration with CAD and numerical quadrature \cite{NAGY2015165,Wang2015}, the shell analysis on geometric models with B-reps \cite{BREITENBERGER2015401,PHILIPP2016312}, and the finite cell method combined with IGA \cite{Dauge2015,RANK2012104,MR3003066,MR3706626}. \textcolor{magenta}{I would remove \cite{Dauge2015} (it is $p$-FEM)} Concerning the lack of stability, we should mention stabilizations based on extrapolation \cite{ doi:10.1137/S0036142900373208,MARUSSIG201879}, and the Cut-IGA method proposed in \cite{1812.08568}, which is related to the many contributions of Cut-FEM and ghost penalty methods \cite{BURMAN20101217,NME:NME4823,BURMAN2012328,Burman2012,Hansbo434217}.

We now describe the simplified mathematical setting. Let $\Omega_0\subseteq \R^d$ (here $d=2,3$)  be a domain described by a bijective spline map $\mathbf{F}: (0,1)^d \to \Omega_0$, i.e., a patch in the isogeometric terminology, and let $\Omega_1,\ldots \Omega_N$ be Lipschitz regular domains in $\R^d$. We assume that $\bigcup_{i=1}^N\overline{\Omega}_i$ are to be cut away from $\Omega_0$ and that our computational domain reads:  
\begin{equation}\label{48}
\Omega=\Omega_0\setminus\bigcup_{i=1}^N\overline{\Omega}_i.
\end{equation}
After trimming the mathematical description of the domain remains unchanged, that is, the elements and basis functions fit the boundary of $\Omega_0$ instead of that of $\Omega$. In this paper, we focus on a simple Poisson problem, with weakly imposed boundary conditions, on the domain $\Omega$ described above. First of all, we discuss the difference between bad matrix conditioning and lack of stability. The first one can be improved by modifying the chosen basis (preconditioning), while the second one needs to act on the bilinear form directly. 

Regarding the lack of stability, we propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that affect stability. For example, in the case of a Neumann condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements. For the stabilization we follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two different versions of the stabilization technique. The first one in the parametric domain, easier to implement from the numerical point of view, but suboptimal. The second , a projection-based stabilization performed directly on the physical domain, which allows us to recover optimal a priori error estimates.

Concerning the bad conditioning of the matrix, we show numerical evidence that a rescaling of the stiffness matrix seems to consistently  resolve the issue. However, the analysis on the linear algebra side is not presented, as it is beyond the scope of this work.

The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. %An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization technique. Two possible constructions of the stabilization operator are suggested and analysed in Section~\ref{sec:construction}, and error estimates are provided in Section~\ref{sec:estimate}. 
Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs \cite{VAZQUEZ2016523}, confirming the theoretical results.


%Complex models are processed within Computer Aided Design (CAD) tools where several geometric manipulations are possible. One procedure that is  basically ubiquitous is \emph{trimming}. Geometries are described as collection of  surfaces that can be joined, intersected or simply superflous parts can be cut away. Often surfaces are bivariate splines or NURBS surfaces and this representation is called ``boundary representation'' (B-rep).  We defer the interested reader to \cite{piegl_ten_2005,Stroud2006}, or to the recent review \cite{Marussig2017} and the references there in. 

%When superflous parts are cut away, the geometric object changes but its mathematical description does not. Clearly this representation is not well suited for the simulation of PDEs and, as a matter of fact, several efforts have been undertaken in the last years to improve the usability of CAD geometries in analysis, especially after the advent of Isogeometric Analysis (IGA) \cite{Cottrell:2009:IAT:1816404,HUGHES20054135}. Indeed, since 2005, also the geometric modelling community has provided important inputs to this scientific challenge \cite{Cohen15} and new strategies to define geometric entities through the volume they occupy instead of their boundaries are now emerging. For instance, in \cite{Massarwi} volumetric representations (V-reps) are proposed as a new, more analysis friendly, geometric design paradigm. On the other hand, trimming remains a main tool allowing for the design of complex models via Boolean operations (such as union, intersection, difference). Thus, in order to guarantee interoperability, in the spirit of isogeometric analysis, we wish to  design tools for the approximation of PDEs that support trimming in the geometric description of the computational domain and do not require the construction of global re-parametrization (meshing). 

%Indeed, isogeometric analysis has been a tremendous success since 2005. It has been successfully applied to many problems, from elasticity \cite{laura18b,MR3610117,Cottrell:2009:IAT:1816404,laura14,MR3196811}, to phase fields models \cite{MR3527591}, to fracture analysis \cite{laura16}, to electromagnetics \cite{mio2,mio1}; its mathematical analysis is now well understood \cite{buffa}, fast assembly and solvers exist today \cite{MR3761002,MR3811621} and strategies for local refinements are now well understood, also from a mathematical stand point e.g., \cite{1078-0947_2019_1_241} and the references therein. This list could continue long.


%On the other hand, basically all developments described above rely on strong requirements on the underlying geometric models and, in general, do not support trimmed geometric entities. The aim of this paper is to contribute to the design of isogeometric methods that robustly support  the use of trimmed geometries.   

%We consider the following simplified situation. Let $\Omega_0\subseteq \R^d$   (here $d=2,3$)  be a domain described by a bijective spline map $\mathbf{F}: (0,1)^d \to \Omega_0$, i.e., a patch in the isogeometric terminology and let $\Omega_1,\ldots \Omega_N$ be Lipschitz regular domains in $\R^d$. We assume that $\bigcup_{i=1}^N\overline{\Omega}_i$ are to be cut away from $\Omega_0$ and that our computational domain reads:  
%\begin{equation}\label{48}
%\Omega=\Omega_0\setminus\bigcup_{i=1}^N\overline{\Omega}_i. 
%\end{equation}
%Let us put ourselves in a situation in which we want to numerically approximate a PDE in a computational domain of the type \eqref{48}. 
%When the superfluous surface areas are cut away, the mathematical description of the domain remains unchanged. It turns out that we have to deal with elements unfitted with the boundary, making the research for efficient quadrature rules and the imposition of boundary conditions a challenge. Moreover there are basis functions, whose support has been cut, affecting the conditioning of the related linear system. In this regard, ideas from fictitious domain and immersed boundary approaches in the FEM literature come to help.

%Indeed, the related engineering literature includes (but is not limited to) the pioneering work  \cite{NAGY2015165,Wang2015} or \cite{BREITENBERGER2015401,PHILIPP2016312} for shell analysis and the finite cell method \cite{Dauge2015,RANK2012104,MR3003066,MR3706626}. 

%In order to guarantee robustness, some stabilization is needed, and our work is related to the previous contributions in this context. In particular, we should mention stabilizations based on extrapolation \cite{ doi:10.1137/S0036142900373208,MARUSSIG201879}, and the Cut-Iga method proposed in \cite{1812.08568},  which is related to the many contributions \cite{BURMAN20101217,NME:NME4823,BURMAN2012328,Burman2012,Hansbo434217}.

%In this paper, we focus on a simple Poisson problem on the domain $\Omega$ described above, with weakly imposed boundary conditions. First of all, we discuss the difference between bad matrix conditioning and lack of stability. The first one can be improved by modifying the chosen basis (preconditioning), while the second one needs to act on the bilinear form directly. 

%Regarding the lack of stability, we propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that generate the lack of stability. For example, in the case of Neumann boundary condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements. For the stabilization we follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two different versions of the stabilization technique. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allows us to recover optimal a priori error estimates.

%Concerning the bad conditioning of the matrix, we show numerical evidence that a rescaling of stiffness matrix seems to consistently  resolve the issue. However, the analysis on the linear algebra side is not presented, as it is beyond the scope of this work. 

%We propose a minimal stabilization technique, inspired by \cite{Renard}, that acts only on those cut elements that generate lack of stability, and leave all issues concerning bad conditioning to a further analysis on the linear algebra side. For example, in the case of Neumann boundary condition on the trimmed boundary, no stabilization is needed. Our stabilization is parameter free, and its computation requires only local projections at the element level, and only for  ``bad'' cut elements.  Moreover, a rescaling of stiffness matrix seems to consistently  resolve the issue of bad conditioning. 

%The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, the Poisson equation in a trimmed domain, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
%After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization technique. 
%%We follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two new stabilization techniques. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allow us to recover optimal a priori error estimates.
%Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs \cite{VAZQUEZ2016523}, confirming the theoretical results.

%The document is organized as follows. Section \ref{4} presents an overview of isogeometric analysis in trimmed domains. In Section \ref{35} we set the model problem, the Poisson equation in a trimmed domain, and explain the main challenges we need to face, namely integration, conditioning and numerical stability of the associated linear system. An exhaustive discussion about the issues of integration and conditioning is beyond the scope of this work.
%After having explained in detail in Section \ref{section_stability} the causes for the lack of stability of the simple Nitsche's formulation, in Section \ref{36} we present our new stabilization. We follow a ``local approach'' (according to the review paper \cite{Marussig2017}), i.e. we modify the analysis, rather than the geometry, in order to be able to face the challenges arising from trimming. We present two new stabilization techniques. One in the parametric domain, easier to implement from the numerical point of view and, in our opinion, more ``natural'', but suboptimal. The other in the physical domain, a projection-based stabilization, which allow us to recover optimal a priori error estimates.
%Finally, we conclude by showing some numerical examples, obtained using the MATLAB library GeoPDEs (\cite{VAZQUEZ2016523}), confirming the theoretical results.
%


==> Sections/numerical_experiments_2.tex <==
\section{Numerical examples}
\subsection{Convergence results}
In this first set of numerical examples we verify that the optimal a priori error estimates of Theorems~\ref{apriori:theorem1_m=1},~\ref{apriori:theorem1_pert}. We also check that the result of Theorem~\ref{apriori:theorem1_m=1} holds in the non-symmetric case $m=0$, as already mentioned in Section~\ref{sec:fe_disc}. Moreover, we study the $L^2$ error of the pressure field, for which optimal convergence is observed in general and super convergence in the case of the lowest order Raviart-Thomas element and triangular meshes.
%The results are obtained with FreeFem++: we are allowed to use the Raviart-Thomas finite element just for $k\in\{0,1,2\}$.
\subsubsection{Unit square with triangular meshes}\label{unit_square_triangles}
We approximate the Darcy problem in the unit square $\Omega=\left(0,1\right)^2$ using a family of triangular meshes, with weakly enforced Neumann boundary conditions on the whole boundary, using as manufactured solutions
\begin{align*}
\u_{ex}=
\begin{pmatrix}
x\sin(x)\sin(y)\\
\sin(x)\cos(y) + x\cos(x)\cos(y)	
\end{pmatrix},\qquad
p_{ex} = x^3 y - 0.125.	
\end{align*}
Note that $\u_{ex}$ is divergence-free. The numerical results are in Figures~\ref{num_exp:fig1_ff},~\ref{num_exp:fig2_ff} and~\ref{num_exp:fig3_ff}.
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the velocity.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_square_ff}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_square_ff}
	}
	\caption{Convergence errors in the ``unit square'' using~\eqref{eq:prob_disc} with $m=1$ with triangular meshes.}\label{num_exp:fig1_ff}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the velocity.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_square_ff_m=0}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_square_ff_m=0}
	}
	\caption{Convergence errors in the ``unit square'' using~\eqref{eq:prob_disc} with $m=0$ with triangular meshes.}\label{num_exp:fig2_ff}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the velocity.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_square_ff_bis}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_square_ff_bis}
	}
	\caption{Convergence errors in the ``unit square'' using~\eqref{eq:prob_disc_bis} with triangular meshes.}\label{num_exp:fig3_ff}
\end{figure}

\subsubsection{Unit circle with triangular meshes}\label{unit_circle}
Now, we consider the unit circle $\Omega=\{(x,y)\in R^2:x^2+y^2\le 1\}$ which is meshed using triangles. We weakly impose the essential boundary conditions on the boundary and consider the following reference solutions:
\begin{align*}
	\u_ex=
	\begin{pmatrix}
		\frac{1}{10}e^x\sin(xy)\\
		x^4+y^2	
	\end{pmatrix},\qquad
	p_{ex} = 	x^3\cos(x)+y^2\sin(x).
\end{align*}
This time $\dive \u_{ex}=2y+\frac{1}{10}\left( e^x\sin(xy)+ye^x\cos(xy)\right)$. See Figures~\ref{num_exp:fig4_ff},~\ref{num_exp:fig6_ff} and~\ref{num_exp:fig8_ff}.
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_circle_ff}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_circle_ff}
	}
	\caption{Convergence errors in the``unit circle'' using~\eqref{eq:prob_disc} with $m=1$ with triangular meshes.}\label{num_exp:fig4_ff}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_circle_ff_m=0}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_circle_ff_m=0}
	}
	\caption{Convergence errors in the ``unit circle'' using~\eqref{eq:prob_disc} with $m=0$ with triangular meshes.}\label{num_exp:fig6_ff}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_circle_ff_bis}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_circle_ff_bis}
	}
	\caption{Convergence errors in the ``unit circle'' using~\eqref{eq:prob_disc_bis} with triangular meshes.}\label{num_exp:fig8_ff}
\end{figure}

%--------------------------
\subsubsection{Unit square with quadrilateral meshes}\label{unit_square_quads}
Let us consider the unit square $\Omega=\left(0,1\right)^2$ meshed using quadrilaterals. We impose natural boundary conditions on $\{(x,y): 0\le x\le 1, y=0\}$ and essential boundary conditions everywhere else in a weak sense. The reference solutions are:
\begin{align*}
\u_{ex} =
\begin{pmatrix}
\cos(x)\operatorname{cosh}(y\\
\sin(x)\operatorname{cosh}(y))	
\end{pmatrix},\qquad
p_{ex}= -\sin(x)\sinh (y)- \left(\cos(1)-1 \right)\left(\cosh(1)-1\right).
\end{align*}
We have $\dive\u_{ex}=0$. For the numerical results we refer to Figures~\ref{num_exp:fig1},~\ref{num_exp:fig1_m=0} and~\ref{num_exp:fig1_bis}.
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the velocity.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_square}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_square}
	}
	\caption{Convergence errors in the ``unit square'' using~\eqref{eq:prob_disc} with $m=1$ with quadrilateral meshes.}\label{num_exp:fig1}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the velocity.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_square_m=0}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_square_m=0}
	}
	\caption{Convergence errors in the ``unit square'' using~\eqref{eq:prob_disc} with $m=0$ with quadrilateral meshes.}\label{num_exp:fig1_m=0}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the velocity.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_unit_square_bis}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_unit_square_bis}
	}
	\caption{Convergence errors in the ``unit square'' using~\eqref{eq:prob_disc_bis} with quadrilateral meshes.}\label{num_exp:fig1_bis}
\end{figure}
%------------------------------------------------------------------------

\subsubsection{Quarter of annulus with quadrilateral isoparametric elements}\label{quarter_annulus}
Let us consider the quarter of annulus centered in the origin with inner and outer radii, respectively, $r=1$ and $R=2$, discretized using quadrilateral isoparametric elements~\cite{claes}. We impose natural boundary conditions on the straight edges $\{(x,y):1\le x\le 2, y=0\}$ and $\{(x,y):x=0, 1\le y\le 2\}$ and weak essential boundary conditions on the curved ones. The manufactured solutions are:
\begin{align*}
	\u_{ex} =
	\begin{pmatrix}
		 -xy^2\\
		-x^2y-\frac{3}{2}y^2
	\end{pmatrix},\qquad
	p_{ex}= \frac{1}{2}\left( x^2y^2 + y^3\right),
\end{align*}
with $\dive \u_{ex}= -x^2 - y^2 - 3y$. See Figures~\ref{num_exp:fig3},~\ref{num_exp:fig3_m=0} and~\ref{num_exp:fig3_bis}.
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_quarter_annulus}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_quarter_annulus}
	}
	\caption{Convergence errors in the ``quarter of annulus'' using~\eqref{eq:prob_disc} with $m=1$ with isoparametric quadrilateral elements.}\label{num_exp:fig3}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_quarter_annulus_m=0}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_quarter_annulus_m=0}
	}
	\caption{Convergence errors in the ``quarter of annulus'' using~\eqref{eq:prob_disc} with $m=0$ with isoparametric quadrilateral elements.}\label{num_exp:fig3_m=0}
\end{figure}
\begin{figure}[!ht]
	\centering
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_vel_l2_quarter_annulus_bis}
	}
	\subfloat[][Error with respect to $\norm{\cdot}_{L^2(\Omega)}$ for the pressure.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_press_quarter_annulus_bis}
	}
	\caption{Convergence errors in the ``quarter of annulus'' using~\eqref{eq:prob_disc_bis} with isoparametric quadrilateral elements.}\label{num_exp:fig3_bis}
\end{figure}
%----------------------------------------------------
\FloatBarrier
% Condition numbers
\subsection{A remark about the condition numbers}\label{conditioning}
Proceeding as in~\cite{ern_guermond_cond} it would be possible to prove that the $\ell^2$-condition number of the stiffness matrix arising from the discretizations~\eqref{eq:prob_disc}, for both $m\in\{0,1\}$,	scales as $h^{-2}$, as Figures~\ref{num_exp:fig6} and~\ref{num_exp:fig4} confirm. The penalty parameter for the weak imposition of the Neumann boundary conditions is the responsible of the deterioration of the conditioning with respect to the standard mixed finite element discretization of the Poisson problem, for which the condition number scales as $h^{-1}$. An even worse situation occurs when formulation~\eqref{eq:prob_disc_bis} is employed. In this case the condition number scales as $h^{-\left(s+2 \right)}$, $s=\min\{r,k\}$, $r$ being the Sobolev regularity of the exact solution for the pressure field and $k$ the polynomial degree of the Raviart-Thomas discretization, as confirmed by Figures~\ref{num_exp:fig7} and~\ref{num_exp:fig5}. 


In all numerical experiments, we do not detect any particular sensitivity of the convergence of the error of the velocities with respect to $\gamma$ in the case of method~\eqref{eq:prob_disc}. On the other hand, it is a different matter altogether as far as the formulation~\eqref{eq:prob_disc_pert} is concerned: this time we can realize the influence of $\gamma$ on the approximation power of the method.

\begin{figure}[!ht]
	\centering
	\subfloat[][$m=1$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{cond_unit_square}
	}
	\subfloat[][$m=0$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{cond_unit_square_m=0}
	}
	\caption{Condition numbers in the ``unit square'' using~\eqref{eq:prob_disc} -  GeoPDEs.}\label{num_exp:fig6}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{cond_unit_square_bis}
	\caption{Condition numbers in the ``unit square'' using~\eqref{eq:prob_disc_bis} -  GeoPDEs.}\label{num_exp:fig7}
\end{figure}


\begin{figure}[!ht]
	\centering
	\subfloat[][$m=1$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{cond_quarter_annulus}
	}
	\subfloat[][$m=0$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{cond_quarter_annulus_m=0}
	}
	\caption{Condition numbers in the ``quarter of annulus'' using~\eqref{eq:prob_disc} -  GeoPDEs.}\label{num_exp:fig4}
\end{figure}
\begin{figure}[!ht]
	\centering
\includestandalone[width=0.5\textwidth,keepaspectratio=true]{cond_quarter_annulus_bis}
	\caption{Condition numbers in the ``quarter of annulus'' using~\eqref{eq:prob_disc_bis} -  GeoPDEs.}\label{num_exp:fig5}
\end{figure}

\FloatBarrier
%---------------------------------------------------------------------------------------------------------
\subsection{The optimality of the penalty parameter}
We want to analyze the optimality of the penalty parameter, denoted through this subsection as $\gamma$, for both numerical schemes. We consider the Raviart-Thomas element of order $k=1$ and compare the numerical results for the $L^2$-error of the velocity field with respect to different powers of the mesh-size as penalty parameter. The first set of numerical experiences is performed using triangular meshes, then we move to quadrilaterals.


To obtain Figures~\ref{num_exp:fig10} and~\ref{num_exp:fig10_bis} the same setting of subsection~\ref{unit_square_triangles} is employed. Then, in Figures~\ref{num_exp:fig11} and~\ref{num_exp:fig11_bis}, we move to the configuration of subsection \ref{unit_circle}. Finally, in Figures~\ref{num_exp:fig8},~\ref{num_exp:fig8_bis} and~\ref{num_exp:fig9},~\ref{num_exp:fig9_bis} we use, respectively, the settings of subsections~\ref{unit_square_quads} and~\ref{quarter_annulus}.

\begin{figure}[!ht]
	\centering
	\subfloat[][$m=1$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_m=1_ff}
	}
	\subfloat[][$m=0$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_m=0_ff}
	}
	\caption{Compare $L^2$-errors for the velocity in the ``unit square'' using~\eqref{eq:prob_disc} with respect to different values of the penalty parameter $\gamma$ with triangular elements.}\label{num_exp:fig10}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_bis_ff}
	\caption{Compare $L^2$-errors for the velocity in the ``unit square'' using~\eqref{eq:prob_disc_bis} with respect to different values of the penalty parameter $\gamma$ with triangular elements.}\label{num_exp:fig10_bis}
\end{figure}
\FloatBarrier
%------------------------------------------------------------------------


\begin{figure}[!ht]
	\centering
	\subfloat[][$m=1$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_circle_compare_penalty_m=1_ff}
	}
	\subfloat[][$m=0$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_circle_compare_penalty_m=0_ff}
	}
	\caption{Compare $L^2$-errors for the velocity in the ``unit circle'' using~\eqref{eq:prob_disc} with respect to different values of the penalty parameter $\gamma$ with triangular elements.}\label{num_exp:fig11}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_circle_compare_penalty_bis_ff}
	\caption{Compare $L^2$-errors for the velocity in the ``unit circle'' using~\eqref{eq:prob_disc_bis} with respect to different values of the penalty parameter $\gamma$ with triangular elements.}\label{num_exp:fig11_bis}
\end{figure}
%-----------------------
\FloatBarrier
% GeoPDEs



\begin{figure}[!ht]
	\centering
	\subfloat[][$m=1$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_m=1}
	}
	\subfloat[][$m=0$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_m=0}
	}
	\caption{Compare $L^2$-errors for the velocity in the ``unit square'' using~\eqref{eq:prob_disc} with respect to different values of the penalty parameter $\gamma$ with triangular elements.}\label{num_exp:fig8}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_bis}
	\caption{Compare $L^2$-errors for the velocity in the ``unit square'' using~\eqref{eq:prob_disc_bis} with respect to different values of the penalty parameter $\gamma$ with quadrilateral elements.}\label{num_exp:fig8_bis}
\end{figure}
\FloatBarrier
%------------------------------------------------------------------------
%------------------------------------------------------------------------
\begin{figure}[!ht]
	\centering
	\subfloat[][$m=1$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_quarter_annulus_compare_penalty_m=1}
	}
	\subfloat[][$m=0$.]
	{
		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_quarter_annulus_compare_penalty_m=0}
	}
	\caption{Compare $L^2$-errors for the velocity in the ``quarter of annulus'' using~\eqref{eq:prob_disc} with respect to different values of the penalty parameter $\gamma$ with quadrilateral elements.}\label{num_exp:fig9}
\end{figure}
\begin{figure}[!ht]
	\centering
	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_quarter_annulus_compare_penalty_bis}
	\caption{Compare $L^2$-errors for the velocity in the ``quarter of annulus'' using~\eqref{eq:prob_disc_bis} with respect to different values of the penalty parameter $\gamma$ with quadrilateral elements.}\label{num_exp:fig9_bis}
\end{figure}
%------------------------------------------------------------------------
%\FloatBarrier
%% GeoPDEs - full boundary
%%------------------------------------------------------------------------
%We repeat the experiments on quadrilateral meshes, but this time imposing the Neumann boundary conditions weakly on the whole boundary. We observe a different behavior of the error for the method~\eqref{eq:prob_disc_bis}.
%\begin{figure}[!ht]
%	\centering
%	\subfloat[][$m=1$.]
%	{
%		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_m=1_fullbd}
%	}
%	\subfloat[][$m=0$.]
%	{
%		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_m=0_fullbd}
%	}
%	\caption{Compare $L^2$-errors for the velocity in the ``unit square'' using~\eqref{eq:prob_disc} with respect to different values of the penalty parameter $\gamma$ (GeoPDEs).}\label{num_exp:fig12}
%\end{figure}
%\begin{figure}[!ht]
%	\centering
%	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_unit_square_compare_penalty_bis_fullbd}
%	\caption{Compare $L^2$-errors for the velocity in the ``unit square'' using~\eqref{eq:prob_disc_bis} with respect to different values of the penalty parameter $\gamma$ (GeoPDEs).}\label{num_exp:fig12_bis}
%\end{figure}
%%------------------------------------------------------------------------
%%------------------------------------------------------------------------
%\begin{figure}[!ht]
%	\centering
%	\subfloat[][$m=1$.]
%	{
%		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_quarter_annulus_compare_penalty_m=1_fullbd}
%	}
%	\subfloat[][$m=0$.]
%	{
%		\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_quarter_annulus_compare_penalty_m=0_fullbd}
%	}
%	\caption{Compare $L^2$-errors for the velocity in the ``quarter of annulus'' using~\eqref{eq:prob_disc} -  GeoPDEs with respect to different values of the penalty parameter $\gamma$.}\label{num_exp:fig13}
%\end{figure}
%\begin{figure}[!ht]
%	\centering
%	\includestandalone[width=0.5\textwidth,keepaspectratio=true]{error_quarter_annulus_compare_penalty_bis_fullbd}
%	\caption{Compare $L^2$-errors for the velocity in the ``quarter of annulus'' using~\eqref{eq:prob_disc_bis} -  GeoPDEs with respect to different values of the penalty parameter $\gamma$.}\label{num_exp:fig13_bis}
%\end{figure}
%%------------------------------------------------------------------------
%


==> Sections/section1_2.tex <==
%----------------------------------------THE CONTINUOUS PROBLEM-----------------------------------------
\section{The Darcy problem and its variational formulation}
%------------------------------------------------ Notation-------------------------------------------------
We introduce some useful notations for the forthcoming analysis. Let $D$ be a Lipschitz-regular domain (subset, open, bounded, connected) of $\mathbb R^d$, $d\in\{2,3\}$. Standard Sobolev spaces $H^s(D)$ for any $s\in\R$ and $H^t(\gamma)$ for $t\in\left[-1,1\right]$ are defined on the domain $D$ and on a non-empty open subset of its boundary $\gamma\subset\partial D$, see~\cite{adams}, with the convention $H^0(D):=L^2(D)$, $H^0(\gamma):=L^2(\gamma)$. Moreover, we introduce the following usual notations:
\begin{align*}
	L^2_0(D):=& L^2(D)/\R, \\
	H_{0,\gamma}(D):= & \text{ closure of } C_{0,\gamma}^\infty(D) \text{ with respect to } \norm{\cdot}_{H^s(D)}=\{v\in H(D): \restr{ v}{\gamma}=0 \}, \\
	H_{f,\gamma}(D):= &\{v\in H(D): \restr{ v}{\gamma}=f \}, \\
	\bm H^s(D):=&\left( H^s(D)\right)^d, \quad \bm H_{0,\gamma}^s(D):=\left( H_{0,\gamma}^s(D)\right)^d,\quad \bm H_{f,\gamma}^s(D):=\left( H_{f,\gamma}^s(D)\right)^d,\quad \bm H^s(\gamma):= \left( H^t(\gamma)\right)^d,\\
	\bm H(\dive;D):=& \{\v\in \bm H^0(D): \dive \v\in H^0(D)\},\\
	\bm H_{0,\gamma}(\dive;D):= & \text{ closure of } \left(C_{0,\gamma}^\infty(D)\right)^d \text{ with respect to } \norm{\cdot}_{H(\dive;D)}=\{\v\in \bm H(\dive;D): \restr{\v\cdot\n}{\gamma}=0 \}, \\
	\bm H_{\sigma,\gamma}(\dive;D):= & \{\v\in \bm H(\dive;D): \restr{\v\cdot\n}{\gamma}=\sigma \}, \\
	\bm H^{0}(\dive;D):= &\{\v\in \bm H(\dive;D): \dive \v=0 \},
\end{align*}
where the divergence operator and the traces on $\gamma$ are defined in the sense of distributions, see~\cite{monk}. For the sake of convenience we are going to employ the same notation $\abs{\cdot}$ for the volume (Lebesgue) and surface (Hausdorff) measures of $\R^d$.

We also denote as $\mathbb Q_{r,s,t}$ the vector space of polynomials of degree at most $r$ in the first variable, at most $s$ in the second and at most $t$ in the third one (analogously for th case $d=2$), $\mathbb P_u$ the vector space of polynomials of degree at most $u$. For the sake of simplicity of the notation we may write $\mathbb Q_k$ instead of $\mathbb Q_{k,k}$ or $\mathbb Q_{k,k,k}$.

Note that throughout this document $C$ will denote generic constants that may change at each occurrence, but that are always independent of the local mesh size.

 Let $\Omega$ be a Lipschitz-regular domain of $\R^d$, $d\in\{2,3\}$. We assume its boundary $\Gamma$ to be partitioned into $\Gamma=\Gamma_N\cup\Gamma_D$ with $\Gamma_N\cap\Gamma_D=\emptyset$.
 Let us consider the following problem, often associated to a linearized model for the flow of groundwater through our domain $\Omega$, here representing a saturated porus medium with permeability $\kappa$.
  Given $\f\in L^2(\Omega;\R^d)$, $g\in L^2(\Omega)$, $u_N\in H^{-\frac{1}{2}}(\Gamma_N)$, $p_D\in H^{\frac{1}{2}}(\Gamma_D)$, we look for $\left(\u,p\right)\in  H_{u_N,\Gamma_N}(\dive;\Omega)\times L^2(\Omega)$ such that
\begin{equation}\label{eq:prob_cont}
	\begin{cases}
		\kappa^{-1} \u -\nabla p = \f \qquad & \text{in}\;\Omega,\\
		\dive\u = g\qquad&\text{in}\;\Omega,\\
		\u\cdot\n=u_N\qquad&\text{on}\;\Gamma_N,\\
		p=p_D\qquad&\text{on}\;\Gamma_D.
	\end{cases}
\end{equation}
The unknowns $\u$ and $p$ represent, respectively, the seepage velocity and the pressure of the fluid.  The first equation of \eqref{eq:prob_cont} is called \emph{Darcy law} relating the velocity and the pressure gradient of the fluid, the second one expresses \emph{mass conservation}, the third and the fourth equations are, respectively, a \emph{Neumann boundary condition} for the velocity field and a \emph{Dirichlet boundary condition} for the pressure. Moreover, $\kappa\in\mathbb R^{d\times d}$ is symmetric positive definite with eigenvalues $\lambda_i$ such that $0<\lambda_{\min}\le\lambda_i\le\lambda_{\max}<+\infty$, for every $i=1,\dots,d$.

\begin{remark}
Contrary to the case of the Poisson problem, here Dirichlet boundary conditions for the pressure are \emph{natural}, in the sense that they can be implicitly enforced in the weak formulation of the problem, while Neumann boundary conditions for the velocity are \emph{essential}, i.e., they are imposed on the functional space. Moreover, let us observe that in the case of purely Neumann boundary conditions, in order to have well-posedness, we have to ``filter out'' the constant pressures, i.e., the trial and test functions for the pressures are required to lie in $ L^2_0(\Omega)$, and to impose a compatibility condition on the data: $\int_\Gamma u _N = \int_\Omega g$.
\end{remark}

\section{A perturbed formulation}
Find $\left(\u^\eps,p^\eps\right)\in  H(\dive;\Omega)\times L^2(\Omega)$ such that
\begin{equation}\label{eq:prob_cont_bis}
	\begin{cases}
		\kappa^{-1} \u^\eps -\nabla p^\eps = \f \qquad & \text{in}\;\Omega,\\
		\dive\u^\eps = g\qquad&\text{in}\;\Omega,\\
		\eps^{-1}\u^\eps\cdot\n=\eps^{-1} u_N+ \left(\chi_{\Gamma_D}p_D-p^\eps\right)\qquad&\text{on}\;\Gamma_N,\\
		p^\eps=p_D\qquad&\text{on}\;\Gamma_D.
	\end{cases}
\end{equation}
Here, $\chi_{\Gamma_D}$ denotes the indicator function of the set $\Gamma_D$. Note that as $\eps\to 0^+$ problem~\eqref{eq:prob_cont_bis} formally degenerates to~\eqref{eq:prob_cont}. In this sense~\eqref{eq:prob_cont_bis} is a perturbation of problem~\eqref{eq:prob_cont}. 

In the subsequent analysis we are going to consider, for the sake of simplicity, $\kappa=I$ the identity matrix. 
%We introduce the following space:
%\begin{align*}
%H^1_{\overline 0}(\Omega):= \{\varphi \in H^1(\Omega): \langle 1,\varphi \rangle_{\Gamma}=0\} .
%\end{align*}
%For $f\in\bm L^2(\Omega)$, $g\in L^2_0(\Omega)$, $u_N\in H^{-\frac{1}{2}(\Gamma)}$, there exists $\left(\u,p \right)\in H(\dive;\Omega)\times H^1_{\overline 0}(\Omega)$ such that
%\begin{align}\label{burman:prob_cont}
%\begin{cases}
%\u-\nabla p = \f \qquad &\text{in}\; \Omega,\\
%\dive \u = g \qquad &\text{in}\; \Omega,\\
%\u\cdot \n = u_N \qquad &\text{on}\; \Gamma.
%\end{cases}
%\end{align}
%By standard theory, there exists a unique solution $\left(\u_\eps,p_\eps\right)$ to the the following Robin problem, for every $\eps>0$.
%\begin{align}\label{burman:prob_pert}
%	\begin{cases}
%		\u^\eps-\nabla p^\eps = \f \qquad &\text{in}\; \Omega,\\
%		\dive \u^\eps = g \qquad &\text{in}\; \Omega,\\
%		\u^\eps\cdot \n  +\eps^{-1}p^\eps= u_N \qquad &\text{on}\; \Gamma.
%	\end{cases}
%\end{align}
%\ \textcolor{red}{For the moment the following result is not used. It might be helpful for Proposition~\ref{prop:stability_eps}}
%\begin{lemma}
%There exists $C>0$ such that
%\begin{align*}
%\norm{\u^\eps}_{L^2(\Omega)} +\norm{p^\eps}_{H^1(\Omega)} \le C \left( \norm{\f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} + \norm{u_N}_{H^{\frac{1}{2}}(\Omega)} \right).
%\end{align*}	
%\end{lemma}
%\begin{proof}
%We consider the case $\\Gamma=\Gamma_N$. Let us define the functional $f\in H^{\frac{1}{2}}(\Gamma)$ as $f(\mu):= \langle 1,\mu \rangle_{\Gamma}$ for every $\mu\in H^{-\frac{1}{2}}(\Gamma)$. It holds
%\begin{equation*}
%f(p^\eps) = \langle 1,p^\eps \rangle_{\Gamma_N} =   \eps\langle 1,u_N-\u^\eps\rangle_{\Gamma}  =0,
%\end{equation*}	
%since the compatibility condition is $\int_{\Gamma} u_N = \int_{\Omega} g$.
%Hence, $p^\eps \in H^1_{\overline 0}(\Omega)$ and, by Poincar\'e-Friedrichs' inequality,
%\begin{align}\label{burman:eq1}
%c \norm{p^\eps}_{L^2(\Omega)} \le \norm{\nabla p^\eps}_{L^2(\Omega)} + \abs{f(p^\eps)} =  \norm{\nabla p^\eps}_{L^2(\Omega)}.
%\end{align}
%By testing the first equation of~\eqref{eq:prob_cont_bis} against $\nabla p_\eps$ and using Cauchy-Schwarz inequality, we obtain
%\begin{equation}\label{burman:eq2}
% \norm{\nabla p^\eps}_{L^2(\Omega)} \le \norm{\u^\eps}_{L^2(\Omega)} + \norm{\f}_{L^2(\Omega)}.	
%\end{equation}
%The following regularity estimate is known from page 84 of~\cite{grisvard} when the domain is at least class $C^{1,1}$, $\f\in\bm L^2(\Omega)$, $g\in L^2(\Omega)$ and $u_N\in H^{\frac{1}{2}}(\Gamma)$:
%\begin{equation}\label{burman:eq3}
%\norm{\u^\eps}_{L^2(\Omega)} +\norm{p^\eps}_{H^1(\Omega)} \le C \left( \norm{\f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} + \norm{u_N}_{H^{\frac{1}{2}}(\Omega)} \right).
%\end{equation}
%By testing the first equation of~\eqref{eq:prob_cont_bis} against $\u^\eps$, integrating by parts, using the second equation of~\eqref{eq:prob_cont_bis} and the boundary conditions
%\begin{align}
%\left( \u^\eps,\u^\eps\right)_{\Omega} + \left( \dive\u^\eps,p^\eps\right)_{\Omega} - \langle p^\eps, \u^\eps \rangle_{\Gamma} =& \left(\f,\u^\eps \right)_{\Omega} \\
%\norm{ \u^\eps}^2_{L^2(\Omega)} + \left( g,p^\eps\right)_{\Omega} +\eps^{-1}\norm{p_\eps}^2_{L^2(\Gamma)}=& \left(\f,\u^\eps \right)_{\Omega} +\langle p_\eps,u_N\rangle_{\Gamma}.
%\end{align}
%Hence,
%\begin{align}\label{burman:eq4}
%\norm{ \u^\eps}^2_{L^2(\Omega)}+\eps^{-1}\norm{p_\eps}^2_{L^2(\Gamma)}\le& \norm{\f}_{L^2(\Omega)}\norm{\u^\eps}_{L^2()\Omega)} +\langle p_\eps,u_N\rangle_{\Gamma} + \norm{g}_{L^2(\Omega)} \norm{p^\eps}_{L^2(\Omega)}.
%\end{align}
%By Cauchy-Schwarz, trace and Poincar\'e inequalities and the embedding $H^{\frac{1}{2}}(\Gamma)\hookrightarrow H^{-\frac{1}{2}} (\Gamma)$, it holds
%\begin{align*}
%\langle p^\eps,u_N \rangle_{\Gamma}	\le \norm{p_\eps}_{H^{\frac{1}{2}}(\Gamma)} \norm{u_N}_{H^{-\frac{1}{2}}(\Gamma)} \le C  \norm{\nabla p_\eps}_{L^2(\Omega)} \norm{u_N}_{H^{\frac{1}{2}}(\Gamma)}.
%\end{align*}	
%Coming back to \eqref{burman:eq4}, we have
%\begin{equation}\label{burman:eq9}
%	\begin{aligned}
%	\norm{ \u^\eps}^2_{L^2(\Omega)}+ \norm{\nabla p^\eps}^2_{L^2(\Omega)}+\eps^{-1}\norm{p_\eps}^2_{L^2(\Gamma)}\le& C \left(   \norm{\f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} + \norm{u_N}_{H^{\frac{1}{2}}(\Omega)}\right)^2\\
%	\le& dC \left( \norm{\f}^2_{L^2(\Omega)} + \norm{g}^2_{L^2(\Omega)} + \norm{u_N}^2_{H^{\frac{1}{2}}(\Omega)} \right).
%	\end{aligned}
%\end{equation}
%\end{proof}

\begin{proposition}\label{prop:conv_eps}
	Let $(\u^\eps,p^\eps),(\u,p)$ be respectively the solutions to~\eqref{eq:prob_cont_bis} and~\eqref{eq:prob_cont}, then there exists $C>0$ such that
	\begin{align*}
\norm{\u-\u^\eps}_{L^2(\Omega)} \le  C \eps\norm{p-p_D}_{L^2(\Gamma_N)}.
	\end{align*}	
\end{proposition}	
\begin{proof}
%\textbf{First attempt.}\\
%Let $\left(\bm\delta,\eta\right):=\left( \u^\eps-\u,p^\eps-p  \right)$ satisfying, by linearity,
%\begin{align}\label{burman:eq5}
%\begin{cases}
%\bm \delta-\nabla \eta = 0 \qquad&\text{in}\;\Omega, \\
%\dive \bm\delta = 0  \qquad&\text{in}\;\Omega, \\
%\bdelta \cdot\n +\eps^{-1}p^\eps =0  \qquad&\text{on}\;\Gamma.
%\end{cases}
%\end{align}
%\eqref{burman:eq5} is a well-posed Neumann problem with $\left( \bdelta,\eta\right) \in H(\dive;\Omega)\times H^1_{\overline 0}(\Omega)$. By Poincar\'e inequality we have
%\begin{align*}
%\norm{\eta}_{H^1(\Omega)} \le C \norm{\nabla \eta}_{L^2(\Omega)}.
%\end{align*}	
%By testing the first equation of~\eqref{burman:eq5} against $\nabla\eta$, we have
%\begin{align*}
%\left( \delta,\nabla \eta\right)_{\Omega} - \left( \nabla \eta, \nabla \eta \right)_{\Omega} =0,
%\end{align*}
%hence
%\begin{align}
%\norm{\nabla \eta}^2_{L^2(\Omega)} = &\left( \eta,\nabla \eta\right)_{\Omega} \le \norm{\delta}_{L^2(\Omega)} \norm{\nabla \eta}_{L^2(\Omega)},\\
%\norm{\nabla \eta}_{L^2(\Omega)}& \le \norm{\delta}_{L^2(\Omega)}.\label{burman:eq6}
%\end{align}
%On the other hand, let us integrate the first equation of~\eqref{burman:eq5} against $\delta$ and compute:
%\begin{align*}
%\norm{\delta}^2_{L^2(\Omega)} -\left(\nabla \eta,\delta \right)_{\Omega} = \norm{\delta }^2_{L^2(\Omega)} + \left( \eta,\dive \delta\right)_{\Omega} - \langle \eta, \delta\cdot\n\rangle_{\Gamma} = \norm{\delta}^2_{L^2(\Omega)} + 0 + \eps^{-1} \langle \eta, p^\eps\rangle_{\Gamma},
%\end{align*}
%hence by Cauchy-Schwarz and~\eqref{burman:eq6}, we get
%\begin{align}
%\norm{\delta}^2_{L^2(\Omega)} \le &\eps^{-1} \norm{p^\eps}_{L^2(\Gamma)} \norm{\eta}_{L^2(\Gamma)}\\
%\norm{\delta}^2_{L^2(\Omega)} + \norm{\nabla \eta}^2_{L^2(\Omega)} \le& 2 \norm{\delta}^2_{L^2(\Omega)} \le 2 \eps^{-1} \norm{p^\eps}_{L^2(\Gamma)} \norm{\eta}_{L^2(\Gamma)}.	\label{burman:eq7}
%\end{align}	
%by trace and Poincar\'e inequalities
%\begin{align}
%\norm{\eta}_{L^2(\Gamma)} \le C \norm{\eta}_{H^1(\Omega)} \le C \norm{\nabla \eta}_{L^2(\Omega)}. \label{burman:eq8}
%\end{align}
%Putting together~\eqref{burman:eq6},~\eqref{burman:eq7} and~\eqref{burman:eq8}, we have
%\begin{align*}
%\norm{\delta}_{L^2(\Omega)} + \norm{\nabla \eta}_{L^2(\Omega)} \le \frac{1}{\norm{\nabla \eta}^2_{L^2(\Omega)}} \left( \norm{\delta}^2_{L^2(\Omega)} + \norm{\nabla \eta}^2_{L^2(\Omega)} \right) \le 2C \eps^{-1} \norm{p^\eps}_{L^2(\Gamma)}.
%\end{align*}
%Using~\eqref{burman:eq9}, we conclude
%\begin{align*}
%\norm{\delta}_{L^2(\Omega)} + \norm{\nabla \eta}_{L^2(\Omega)} \le C \left( \norm{\f}^2_{L^2(\Omega)} + \norm{g}^2_{L^2(\Omega)} + \norm{u_N}^2_{H^{\frac{1}{2}}(\Omega)} \right).	
%\end{align*}	
%\textcolor{red}{It is not enough to conclude that the rhs goes like $\eps^{-1}$.}
%
%\textbf{Second attempt.} \\
Let us observe that if $\left( \u,p\right)$ and $\left( \u^\eps,p^\eps\right)$ solve, respectively, the problems~\eqref{eq:prob_cont} and~\eqref{eq:prob_cont_bis}, then $p$ and $p^\eps$ are the solutions of
 \begin{align}
&\begin{cases}\label{burman:eq10}
-\Delta p = -g +\dive \f \qquad&\text{in}\;\Omega,\\
\frac{\partial p}{\partial n} = u_N\qquad&\text{on}\;\Gamma_N,\\
p = p_D	\qquad&\text{on}\;\Gamma_D,
\end{cases}	
\\
&\begin{cases}\label{burman:eq11}
	-\Delta p^\eps = -g +\dive \f \qquad&\text{in}\;\Omega,\\
	\frac{\partial p^\eps}{\partial n} + \eps p^\eps = u_N + \eps p_D \qquad&\text{on}\;\Gamma_N,\\
	p^\eps = p_D	\qquad&\text{on}\;\Gamma_D.
\end{cases}	
\end{align}
Let $\delta:= p -p^\eps$, with $p$ and $p^\eps$ respectively the solutions of~\eqref{burman:eq10} and~\eqref{burman:eq11}, then $\delta$ solves
\begin{align}&\begin{cases}\label{burman:eq12}
-\Delta \delta = 0 \qquad& \text{in}\;\Omega, \\
\delta +\eps^{-1}\frac{\partial \delta}{\partial n} = p-p_D \qquad &\text{on}\;\Gamma_N,\\
\delta = 0	\qquad&\text{on}\;\Gamma_D.
\end{cases}
\end{align}
We rewrite~\eqref{burman:eq12} in variational form. Find $\delta \in H^1_{0,\Gamma_D}(\Omega)$ such that
\begin{align}\label{burman:eq13}
\left( \nabla \delta,\nabla \varphi\right)_\Omega + \eps \langle \delta, \varphi\rangle_{\Gamma_N} = \eps \langle p-p_D,\varphi \rangle_{\Gamma_N}\qquad\forall\ \varphi\in H^1_{0,\Gamma_D}(\Omega).
\end{align}
By standard theory~\eqref{burman:eq13} is well-posed and in particular the bilinear form inducing its left hand side is coercive, meaning that
\begin{align}\label{burman:eq14}
 \norm{\delta}^2_{H^1(\Omega)} \lesssim \norm{\nabla \delta}^2_{L^2(\Omega)} + \eps \norm{\delta}^2_{L^2(\Gamma_N)}.
\end{align}
By combining~\eqref{burman:eq13},~\eqref{burman:eq14}, the Cauchy-Schwarz and a trace inequalities:
\begin{align}\label{burman:eq15}
	\norm{\delta}^2_{H^1(\Omega)} \lesssim \eps \norm{p-p_D}_{L^2(\Gamma_N)}\norm{\delta}_{H^1(\Omega)},
\end{align}
meaning that $\norm{\delta}_{H^1(\Omega)} \lesssim \eps \norm{p-p_D}_{L^2(\Gamma_N)}$. Since $\u-\u^\eps = \nabla p + \f - \left( \nabla p^\eps +\f \right) = \nabla \left( p-p^\eps \right) = \nabla \delta$, then we are done.
\end{proof}
%\begin{proposition}\label{prop:stability_eps}
%Let $\left(\u^\eps,p^\eps\right)$ be the solution of~\eqref{eq:prob_cont_bis}. \textcolor{red}{Under suitable regularity assumptions on the data and on the domain}, there exists $C>0$ such that
%\begin{align}\label{burman:eq20}
%\norm{\u^\eps}_{H^{s+1}(\Omega)} \le C \left( \norm{\f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)}\right).
%\end{align}
%\end{proposition}
%\begin{proof}
%As before, let us consider an equivalent formulation for~\eqref{eq:prob_cont_bis} and put ourselves in the pure Neumann case $\Gamma=\Gamma_N$. We observe that $\left(\u^\eps,p^\eps \right)$ is the solution to~\eqref{eq:prob_cont_bis} if and only if $p^\eps$ solves
%\begin{align}
%	\begin{cases}\label{burman:eq16}
%		-\Delta p^\eps = -g +\dive \f \qquad&\text{in}\;\Omega,\\
%		\frac{\partial p^\eps}{\partial n} + \eps^{-1}p^\eps = u_N \qquad&\text{on}\;\Gamma.
%	\end{cases}	
%\end{align}
%Let us recall that given $\w:\Omega\to \R^d$ and $\varphi:\Omega\to\R$, we can decompose in an open neighborhood of the boundary
%\begin{align*}
%\w = \w_T + w_n \n,\qquad \nabla \varphi = \nabla_T \varphi + \frac{\partial\varphi}{\partial n}\n,
%\end{align*}
%$\w_T$ and $w_n$ being, respectively, the tangent and normal components of $\w$. The operator $\nabla_T:H^1(\Gamma)\to\bm L^2_T(\Gamma)$ is the tangential gradient and can be defined as in~\cite{monk}. We recall as well the definition of the operator $\dive_T:\bm L^2_T(\Gamma)\to H^{-1}(\Gamma)$, the tangential divergence, defined as the adjoint of the tangential gradient, namely, for every $\v \in \bm L_T^2(\Gamma)$ and $p\in H^1(\Gamma)$
%\begin{align}
%\langle \dive_T \v, p \rangle_\Gamma  = \langle \v, \nabla_T p \rangle_\Gamma,
%\end{align}	
%with $\bm L_T^2(\Gamma):= \{\v \in \bm L^2(\Gamma): \v\cdot\n = 0 \}$.
%Theorem~3.1.1.1 in~\cite{grisvard} states that if $\Omega$ is open, bounded of class $C^2$, then every $\v\in\bm H^1(\Omega)$ satisfies
%\begin{align}\label{burman:eq17}
%\int_\Omega \abs{\dive \v}^2 -\sum_{i,j=1}^d \left(D_j v_i, D_i v_j  \right)_{\Omega} = -2\langle \v_T, \nabla_T v_n \rangle_\Gamma - \int_{\Gamma} \{ (\operatorname{tr}\mathcal B)v_n^2 +\mathcal B(\v_T,\v_T)  \}, 
%\end{align}
%$\mathcal B$ being the second fundamental quadratic form associated to $\Gamma$. Let us apply~\eqref{burman:eq17} to $\v=\nabla p^\eps$. We have
%\begin{align}\label{burman:eq18}
%\int_\Omega \abs{\Delta p^\eps}^2- \sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2\ge -2 \langle \nabla_T p^\eps, \nabla_T u_N \rangle_\Gamma +2\eps^{-1} \int_{\Gamma} \abs{\nabla_T p^\eps}^2,	
%\end{align}	
%since
%\begin{align*}
%-\int_{\Gamma}	\mathcal B(\nabla_T p^\eps,\nabla_T p^\eps)\ge & 0,\qquad -\int_{\Gamma} (\operatorname{tr}\mathcal B) \frac{\partial p^\eps}{\partial n}^2 \ge 0,\\
%-2\langle \nabla_T p^\eps, \nabla_T \frac{\partial p^\eps}{\partial n}\rangle	= & -2\langle \nabla_T p^\eps, \nabla_T u_N \rangle_\Gamma + 2 \eps^{-1} \int_{\Gamma} \abs{\nabla_Tp^\eps}^2,
%\end{align*}	
%having used the non-positiveness of $\mathcal B$ due to the convexity of $\Omega$ (see~\cite{grisvard}) and the boundary conditions of~\eqref{eq:prob_cont_bis}. Note that~\eqref{burman:eq18} in turn implies
%\begin{align*}
%\int_\Omega \abs{\Delta p^\eps}^2- \sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2\ge -2 \langle \nabla_T p^\eps, \nabla_T u_N \rangle_\Gamma,	
%\end{align*}	
%and the last inequality can be rewritten as
%\begin{align*}
%	 \sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2 \le \int_\Omega \abs{\Delta p^\eps}^2 +2 \langle \nabla_T p^\eps, \nabla_T u_N \rangle_\Gamma.
%\end{align*}	
%It is sufficient to bound the term $2 \langle \nabla_T p^\eps, \nabla_T u_N \rangle_\Gamma$.
%
%\textcolor{red}{do not know how to do it!}
%
%For the sake of simplicity, but probably with loss of generality, let us consider the case $u_N=0$ (as in Theorem 3.1.2.3 of~\ref{grisvard}) so that we have
%\begin{align*}
%-2\langle \nabla_T p^\eps,\nabla_T \frac{\partial p^\eps}{\partial n}\rangle_\Gamma = 2 \eps^{-1} \norm{\nabla_T p^\eps}^2_{L^2(\Gamma)},
%\end{align*}
%hence
%\begin{align*}
%	\sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2 \le \int_\Omega \abs{\Delta p^\eps}^2 -2  \eps^{-1} \norm{\nabla_T p^\eps}^2_{L^2(\Gamma)},
%\end{align*}
%and, in particular,
%\begin{align*}
%	\sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2 \le \int_\Omega \abs{\Delta p^\eps}^2.
%	\end{align*}
%Let us bound the other terms part of $\norm{p^\eps}_{H^2(\Omega)}$. Green formula states
%\begin{align*}
%-\left(\Delta p^\eps, p^\eps   \right)_\Omega = \int_\Omega \abs{\nabla p^\eps}^2 - \langle \frac{\partial p^\eps}{\partial n} p^\eps\rangle_\Gamma,	
%\end{align*}	
%so that, using the boundary conditions of~\eqref{eq:prob_cont_bis},
%\begin{align*}
%\norm{\nabla p^\eps}^2_{L^2(\Omega)} =& 	-\left(\Delta p^\eps, p^\eps   \right)_\Omega +  \langle \frac{\partial p^\eps}{\partial n}, p^\eps\rangle_\Gamma =
%-\left(\Delta p^\eps, p^\eps   \right)_\Omega  + \langle u_N - \eps^{-1}p^\eps, p^\eps \rangle_\Gamma \\
%\le & \norm{-\Delta p^\eps}_{L^2(\Omega)} \norm{p^\eps}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)} \norm{p^\eps}_{L^2(\Gamma)} -\eps^{-1} \norm{p^\eps}^2_{L^2(\Gamma)},
%\end{align*}	
%implying
%\begin{align}\label{burman:eq20}
%	\norm{\nabla p^\eps}^2_{L^2(\Omega)} 
%	\le  \norm{-\Delta p^\eps}_{L^2(\Omega)} \norm{p^\eps}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)} \norm{p^\eps}_{L^2(\Gamma)}.
%\end{align}
%Because of the compatibility condition on the data when $\Gamma=\Gamma_N$, we have
%\begin{align*}
%\int_\Gamma p^\eps = \eps \left( \int_\Gamma u_N - \int_\Gamma \frac{\partial p^\eps}{\partial n} \right) = \eps \left( \int_\Gamma u_N - \int_\Omega  \dive \u^\eps \right) = \eps \left( \int_\Gamma u_N - \int_\Omega g \right)=0,
%\end{align*}
%hence, using the Friedrichs inequality,
%\begin{align}\label{burman:eq19}
%\norm{p^\eps}_{L^2(\Omega)}	\le C \left( \norm{\nabla p^\eps}_{L^2(\Omega)} + \int_\Gamma p^\eps \right) = 
%C \norm{\nabla p^\eps}_{L^2(\Omega)}.
%\end{align}	
%By combining the multiplicative trace inequality and~\eqref{burman:eq19}, we obtain
%\begin{align*}
%\norm{p^\eps}_{L^2(\Gamma)}\le C \norm{p^\eps}^{\frac{1}{2}}_{L^2(\Omega)} \norm{\nabla p^\eps}^{\frac{1}{2}}_{L^2(\Omega)} \le C \norm{\nabla p^\eps}^{\frac{1}{2}}_{L^2(\Omega)}\norm{\nabla p^\eps}^{\frac{1}{2}}_{L^2(\Omega)} = C \norm{\nabla p^\eps}_{L^2(\Omega)}.
%\end{align*}
%Combining~\eqref{burman:eq20} and~\eqref{burman:eq19}, we obtain
%\begin{align*}
%\norm{\nabla p^\eps}^2_{L^2(\Omega)} \le C \left( \norm{-\Delta p^\eps}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)}   \right) \norm{\nabla p^\eps}_{L^2(\Omega)},
%\end{align*}	
%so that
%\begin{align*}
%\norm{\nabla p^\eps}_{L^2(\Omega)} \le C  \left( \norm{-\Delta p^\eps}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)}  \right).
%\end{align*}
%Hence,
%\begin{align*}
%\norm{p^\eps}_{H^2(\Omega)} \le \norm{p^\eps}_{L^2(\Omega)} + \norm{\nabla p^\eps}_{L^2(\Omega)} + \left(\sum_{i,j=1}^d \int_\Omega \abs{D^2_{x_i,x_j} p^\eps}^2 \right)^{\frac{1}{2}}	\le 2 \norm{\nabla p^\eps}_{L^2(\Omega)} + \norm{\Delta p^\eps}^2_{L^2(\Omega)} + 2 \langle  \nabla_T p^\eps,\nabla_T u_N\rangle_\Gamma
%\end{align*}	
%\textcolor{red}{Let us assume that we proved the desired bound for $\norm{p^\eps}_{H^{2}(\Omega)}$. Moreover, let us assume that the bound reads as
%\begin{align}\label{burman:eq21}
%\norm{p^\eps}_{H^2(\Omega)} \le C \left( \norm{\f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)} \right).
%\end{align}
%}\\
% In order to prove~\eqref{burman:eq20} for a general $s>1$, we need to show that if $p^\eps$ solves~\eqref{burman:eq16}, then $D^\alpha p^\eps$ is also a solution.
% 
%We define, for every non-negative multi-index $\alpha = \left( \alpha_1,\dots, \alpha_d\right)$, 
% \begin{align}
% D^\alpha \varphi : = \frac{\partial^{\abs{\alpha}} \varphi}{\partial x_1^{\alpha_1} \dots \partial x_d^{\alpha_d}},	
% \end{align}	
%where $\abs{\alpha}:=\alpha_1 +\dots + \alpha_d$.
%
%By linearity of problem~\eqref{burman:eq16} and of the derivatives, it holds
%\begin{align*}
%\begin{cases}
%-\Delta D^s p^\eps = -D^s g +\dive D^s f \qquad &\text{in}\;\Omega, \\
%\frac{\partial}{\partial n} D^s p^\eps +\eps^{-1} D^s p^\eps = D^s u_N \qquad &\text{on}\;\Gamma,	
%\end{cases}	
%\end{align*}	
%so, by applying the previous estimates to $D^s p^\eps$, we find
%\begin{align}\label{burman:eq22}
%\norm{D^s p^\eps}_{H^2(\Omega)} \le C  \left( \norm{D^s\f}_{L^2(\Omega)} + \norm{D^sg}_{L^2(\Omega)} + \norm{D^su_N}_{L^2(\Gamma)} \right).
%\end{align}
%By combining~\eqref{burman:eq21} and~\eqref{burman:eq22}, we obtain
%\begin{align}
%	\norm{ p^\eps}_{H^{s+1}\Omega)} \le C  \left(  \norm{\f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} + \norm{u_N}_{L^2(\Gamma)}+ \norm{D^s\f}_{L^2(\Omega)} + \norm{D^sg}_{L^2(\Omega)} + \norm{D^su_N}_{L^2(\Gamma)} \right).
%\end{align}
%\end{proof}
In order to avoid technicalities, let us assume $\Omega$ to be a convex domain with  a $C^2$ boundary and the Neumann data to be homogeneous. We believe that the same result holds under milder assumptions.
\begin{proposition}\label{prop:stability_eps_simple}
	Let $\left(\u^\eps,p^\eps\right)$ be the solution of~\eqref{eq:prob_cont_bis} and suppose that $\Omega$ is convex, $\Gamma$ is $C^2$ and $u_N=0$. Then there exists $C>0$ such that
	\begin{align}\label{burman:eq20bis_simple}
	\norm{\u^\eps}_{H^{s+1}(\Omega)} \le  C \left( \norm{\f}_{H^{s+2}(\Omega)} + \norm{g}_{H^{s+1}(\Omega)}   \right),
\end{align}
provide that $\f\in \bm H^{s+2}(\Omega)$, $g\in H^{s+1}(\Omega)$.
\end{proposition}
\begin{proof}
	As before, let us consider an equivalent formulation for~\eqref{eq:prob_cont_bis} and, without loss of generality, put ourselves in the pure Neumann case $\Gamma=\Gamma_N$. We observe that $\left(\u^\eps,p^\eps \right)$ is the solution to~\eqref{eq:prob_cont_bis} if and only if $p^\eps$ solves
	\begin{align}
		\begin{cases}\label{burman:eq16_simple}
			-\Delta p^\eps = -g +\dive \f \qquad&\text{in}\;\Omega,\\
			\frac{\partial p^\eps}{\partial n} + \eps p^\eps = 0 \qquad&\text{on}\;\Gamma.
		\end{cases}	
	\end{align}
	Let us recall that given $\w:\Omega\to \R^d$ and $\varphi:\Omega\to\R$, the following decompositions hold in an open neighborhood of the boundary
	\begin{align*}
		\w = \w_T + w_n \n,\qquad \nabla \varphi = \nabla_T \varphi + \frac{\partial\varphi}{\partial n}\n,
	\end{align*}
	$\w_T$ and $w_n$ being, respectively, the tangent and normal components of $\w$. The operator $\nabla_T:H^1(\Gamma)\to\bm L^2_T(\Gamma)$ is the tangential gradient and can be defined as in~\cite{monk}.
%	 We recall as well the definition of the operator $\dive_T:\bm L^2_T(\Gamma)\to H^{-1}(\Gamma)$, the tangential divergence, defined as the adjoint of the tangential gradient, namely, for every $\v \in \bm L_T^2(\Gamma)$ and $p\in H^1(\Gamma)$
%	\begin{align}
%		\langle \dive_T \v, p \rangle_\Gamma  = \langle \v, \nabla_T p \rangle_\Gamma,
%	\end{align}	
%	with $\bm L_T^2(\Gamma):= \{\v \in \bm L^2(\Gamma): \v\cdot\n = 0 \}$.
	Theorem~3.1.1.1 in~\cite{grisvard} states that if $\Omega$ is open, bounded with $\Gamma$ of class $C^2$, then every $\v\in\bm H^1(\Omega)$ satisfies
	\begin{align}\label{burman:eq17_simple}
		\norm{\dive \v}^2_{L^2(\Omega)} -\sum_{i,j=1}^d \left(D_j v_i, D_i v_j  \right)_{\Omega} = -2\langle \v_T, \nabla_T v_n \rangle_\Gamma - \int_{\Gamma} \{ (\operatorname{tr}\mathcal B)v_n^2 +\mathcal B(\v_T,\v_T)  \}, 
	\end{align}
	$\mathcal B(\cdot,\cdot)$ being the second fundamental quadratic form associated to $\Gamma$ and $\operatorname{tr}\mathcal B$ its trace, see~\cite{grisvard} for the definitions. Let us apply~\eqref{burman:eq17_simple} to $\v=\nabla p^\eps$. We have
	\begin{align}\label{burman:eq18_simple}
	\norm{\Delta p^\eps}^2_{L^2(\Omega)}- \sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2\ge 	-2\langle \nabla_T p^\eps, \nabla_T \frac{\partial p^\eps}{\partial n}\rangle_\Gamma,
	\end{align}	
	since
	\begin{align*}
		-\int_{\Gamma}	\mathcal B(\nabla_T p^\eps,\nabla_T p^\eps)\ge  0,\qquad -\int_{\Gamma} (\operatorname{tr}\mathcal B) \frac{\partial p^\eps}{\partial n}^2 \ge 0,
	\end{align*}	
	having used the non-positiveness of $\mathcal B$ due to the convexity of $\Omega$ (see~\cite{grisvard}). Moreover, the boundary conditions of~\eqref{eq:prob_cont_bis} imply
	\begin{align*}
		-2\langle \nabla_T p^\eps, \nabla_T \frac{\partial p^\eps}{\partial n}\rangle_\Gamma	=  2 \eps \norm{\nabla_Tp^\eps}^2_{L^2(\Gamma)},
	\end{align*}
	 hence~\eqref{burman:eq18_simple} in turn implies
	\begin{align*}
		\sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2 \le \norm{\Delta p^\eps}^2_{L^2(\Omega)} -2  \eps \norm{\nabla_T p^\eps}^2_{L^2(\Gamma)},
	\end{align*}
	and, in particular,
	\begin{align*}
		\sum_{i,j=1}^d \int_{\Omega} \abs{D^2_{x_ix_j}p^\eps}^2 \le \norm{\Delta p^\eps}^2_{L^2(\Omega)}.
	\end{align*}
	Let us bound the other terms which are part of $\norm{p^\eps}_{H^2(\Omega)}$. Green formula states
	\begin{align*}
		-\left(\Delta p^\eps, p^\eps   \right)_\Omega =\norm{\nabla p^\eps}^2_{L^2(\Omega)} - \langle \frac{\partial p^\eps}{\partial n} p^\eps\rangle_\Gamma,	
	\end{align*}	
	so that, using the boundary conditions of~\eqref{eq:prob_cont_bis},
	\begin{align*}
		\norm{\nabla p^\eps}^2_{L^2(\Omega)} =& 	-\left(\Delta p^\eps, p^\eps   \right)_\Omega +  \langle \frac{\partial p^\eps}{\partial n}, p^\eps\rangle_\Gamma =
		-\left(\Delta p^\eps, p^\eps   \right)_\Omega  - \langle \eps p^\eps, p^\eps \rangle_\Gamma \\
		\le & \norm{-\Delta p^\eps}_{L^2(\Omega)} \norm{p^\eps}_{L^2(\Omega)} -\eps \norm{p^\eps}^2_{L^2(\Gamma)},
	\end{align*}	
	implying
	\begin{align}\label{burman:eq20_simple}
		\norm{\nabla p^\eps}^2_{L^2(\Omega)} 
		\le  \norm{\Delta p^\eps}_{L^2(\Omega)} \norm{p^\eps}_{L^2(\Omega)}.
	\end{align}
	Because of the compatibility condition on the data when $\Gamma=\Gamma_N$, we have
	\begin{align*}
		\int_\Gamma p^\eps = \eps^{-1} \left( \int_\Gamma u_N - \int_\Gamma \frac{\partial p^\eps}{\partial n} \right) = \eps^{-1} \left( \int_\Gamma u_N - \int_\Omega  \dive \u^\eps \right) = \eps^{-1} \left( \int_\Gamma u_N - \int_\Omega g \right)=0,
	\end{align*}
	hence, using the Friedrichs inequality,
	\begin{align}\label{burman:eq19_simple}
		\norm{p^\eps}_{L^2(\Omega)}	\le C \left( \norm{\nabla p^\eps}_{L^2(\Omega)} + \int_\Gamma p^\eps \right) = 
		C \norm{\nabla p^\eps}_{L^2(\Omega)}.
	\end{align}	
	Combining~\eqref{burman:eq20_simple} and~\eqref{burman:eq19_simple}, we obtain
	\begin{align*}
		\norm{\nabla p^\eps}^2_{L^2(\Omega)} \le C \norm{\Delta p^\eps}_{L^2(\Omega)} \norm{\nabla p^\eps}_{L^2(\Omega)},
	\end{align*}	
	so that
	\begin{align*}
		\norm{\nabla p^\eps}_{L^2(\Omega)} \le C  \norm{\Delta p^\eps}_{L^2(\Omega)}.
	\end{align*}
	Hence,
	\begin{equation}\label{burman:eq21_simple}
		\begin{aligned}
		\norm{p^\eps}_{H^2(\Omega)} \le &\norm{p^\eps}_{L^2(\Omega)} + \norm{\nabla p^\eps}_{L^2(\Omega)} + \left(\sum_{i,j=1}^d \int_\Omega \abs{D^2_{x_i,x_j} p^\eps}^2 \right)^{\frac{1}{2}}	\le C \norm{\nabla p^\eps}_{L^2(\Omega)} + \norm{\Delta p^\eps}_{L^2(\Omega)}\\
		 \le &C \norm{\Delta p^\eps}_{L^2(\Omega)} \le C \left( \norm{\dive \f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)}\right).
		 \end{aligned}
	\end{equation}	
	In order to prove~\eqref{burman:eq20_simple} for a general $s>1$, we need to show that if $p^\eps$ solves~\eqref{burman:eq16_simple}, then $D^\alpha p^\eps$ is also a solution.
	
	We denote, for every non-negative multi-index $\alpha = \left( \alpha_1,\dots, \alpha_d\right)$, 
	\begin{align*}
		D^\alpha \varphi : = \frac{\partial^{\abs{\alpha}} \varphi}{\partial x_1^{\alpha_1} \dots \partial x_d^{\alpha_d}},	
	\end{align*}	
	where $\abs{\alpha}:=\alpha_1 +\dots + \alpha_d$.
	
	By linearity of problem~\eqref{burman:eq16_simple} and of the derivatives, it holds
	\begin{align*}
		\begin{cases}
			-\Delta D^s p^\eps = -D^s g +\dive D^s f \qquad &\text{in}\;\Omega, \\
			\frac{\partial}{\partial n} D^s p^\eps +\eps D^s p^\eps = 0 \qquad &\text{on}\;\Gamma,	
		\end{cases}	
	\end{align*}	
	so, by applying the previous estimates to $D^s p^\eps$, we find
	\begin{align}\label{burman:eq22_simple}
		\norm{D^s p^\eps}_{H^2(\Omega)} \le C  \left( \norm{ D^s \dive\f}_{L^2(\Omega)} + \norm{D^sg}_{L^2(\Omega)}\right).
	\end{align}
	We combine~\eqref{burman:eq21_simple} and~\eqref{burman:eq22_simple} to obtain
	\begin{align}
		\norm{ p^\eps}_{H^{s+1}\Omega)} \le C  \left(  \norm{\dive \f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} +  \norm{D^s\dive \f}_{L^2(\Omega)} + \norm{D^sg}_{L^2(\Omega)} \right).
	\end{align}
Finally, using the relation $u^\eps = \nabla p^\eps +\f$, it holds
\begin{align*}
\norm{\u^\eps}_{H^{s+1}(\Omega)} \le &\norm{\nabla p^\eps}_{H^{s+1}(\Omega)} + \norm{\f}_{H^{s+1}(\Omega)}\le \norm{p^\eps}_{H^{s+2}(\Omega)} + \norm{\f}_{H^{s+1}(\Omega)} \\
\le & C  \left(  \norm{\dive \f}_{L^2(\Omega)} + \norm{g}_{L^2(\Omega)} +  \norm{D^{s+1}\dive \f}_{L^2(\Omega)} + \norm{D^{s+1}g}_{L^2(\Omega)} \right) + \norm{\f}_{H^{s+1}(\Omega)}\\
\le & C \left( \norm{\f}_{H^{s+2}(\Omega)} + \norm{g}_{H^{s+1}(\Omega)}   \right).
\end{align*}
\end{proof}
%----------------------------------------FINITE ELEMENT DISCRETIZATION-----------------------------------------
\section{The finite element discretization}\label{sec:fe_disc}
Let $\left(\mathcal T_h\right)_{h>0}$ denote a family of triangular or quadrilateral meshes  of $\Omega$. It will be useful to partition the collection of edges (or faces if $d=3$) $\mathcal F_h$ of $\mathcal T_h$ into three collections: the internal ones $\mathcal F_h^i$ and the ones lying on $\Gamma_N$ and on $\Gamma_D$, grouped respectively in $\mathcal F_h^\partial(\Gamma_N)$ and $\mathcal F_h^\partial (\Gamma_D)$, $\mathcal F_h^\partial = \mathcal F_h^\partial(\Gamma_N) \cup \mathcal F_h^\partial (\Gamma_D)$. For every $K\in\mathcal T_h$, $h>0$, let $h_K:=\operatorname{diam}(K)$ and $h:=\max_{K\in\mathcal T_h} h_K$. We assume the mesh to be \emph{shape-regular}, i.e., there exists $\sigma>0$, independent of $h$, such that $\max_{K\in\mathcal T_h} \frac{h_K}{\rho_K}\le \sigma$, $\rho_K$ being the diameter of the largest ball inscribed in $K$. Moreover, $\mathcal T_h$ is supposed to be \emph{quasi-uniform} in the sense that there exists $\tau>0$, independent of $h$, such that $\min_{K\in \mathcal T_h} h_K\ge \tau h$.
Let $\varphi:\Omega\to\R$ be smooth enough so that for every $K\in\mathcal T_h$ its restriction $\restr{\varphi}{K}$ can be extended up to the boundary $\partial K$. Then, for all $f\in\mathcal F_h^i$ and a.e. $x\in f$, we define the \emph{jump} of $\varphi$ as
\begin{align*}
	[\varphi]_f(x):=\restr{\varphi}{K_1}(x)-\restr{\varphi}{K_2}(x),
\end{align*}
where $f=\partial K_1\cap \partial K_2$. We may remove the subscript $f$ when it is clear from the context to which edge (face, if $d=3$, respectively) we refer to.

In order to discretize problem~\eqref{eq:prob_cont}, we need to choose a suitable couple of subspaces $ V_h\subset H\left(\dive;\Omega\right)$ and $ Q_h\subset L^2(\Omega)$. In the following, $\hat K$ will be our \emph{reference element}, and, according to the type of mesh employed, it will be either the unit $d$-simplex, i.e., the triangle of vertices $(0,0),(1,0),(0,1)$, or the unit $d$-cube $\left[0,1\right]^d$. 
 
 For the triangular meshes, the \emph{Raviart-Thomas} finite element on $\hat K$ is
 \begin{equation*}
 	\mathbb{RT}_k(\hat K):=\left(\mathbb{P}_k(\hat K)\right)^d\oplus \bm x\tilde{\mathbb P}_k(\hat K),	
\end{equation*}
 while, in the case of quadrilaterals, it reads as follows (see, for instance, \cite{arnold}):
\begin{equation*}
	\mathbb{RT}_k(\hat K):=
	\begin{cases}
		\mathbb{Q}_{k+1,{k}}(\hat K)\times\mathbb{Q}_{k,k+1}(\hat K)\qquad&\text{if}\;d=2,\\
		\mathbb{Q}_{k+1,{k},k}(\hat K)\times \mathbb{Q}_{k,k+1,k}(\hat K)\times\mathbb{Q}_{k,k,k+1}(\hat K)\qquad&\text{if}\;d=3.
	\end{cases}
\end{equation*}
We map the reference element  to a general $K\in\mathcal T_h$ via the \emph{affine map} $F_K:\hat K\to K$, $F_K(\hat x):= B_K \hat x + b_K$, where $B_K\in \mathbb R^{d\times d}$ is diagonal and invertible, and $b_K\in\mathbb R^d$. For $H(\dive;\Omega)$, the natural way to transform functions from $\hat K$ to $K$ is through the \emph{Piola transform}. Namely, given $\hat \u:\hat K\to\mathbb R^d$, we define $\u=\mathcal P_K \hat \u: K\to\mathbb R^d$ by
\begin{equation*}
	\u(x)=\mathcal P_{K} \hat \u (x):=\abs{\det\left(B_K \right)}^{-1}B_K \hat\u(\hat x),\qquad\text{where}\qquad \hat x=B^{-1}_K\left(x-b_K\right).
\end{equation*}
For functions in $L^2(\Omega)$, we just compose them with the affine map, namely $\hat q:\hat K\to\R$ is transformed to $q=\hat q \circ F_K^{-1}:K\to\R$. In this way, we can define the finite-dimensional subspaces:
\begin{equation*}
\begin{aligned}
	V_h&:=\{\v_h \in H\left(\dive;\Omega\right):\restr{\v_h}{K}\in \mathbb{RT}_k(K)\quad\forall\ K\in\mathcal T_h\},\\
	Q_h&:=\{q_h\in L^2\left(\Omega\right):\restr{q_h}{K}\circ F_K\in\mathbb{P}_{k}\left(K\right)\quad\forall\ K\in\mathcal T_h\},\qquad\text{for triangles,}\\
	Q_h&:=\{q_h\in L^2\left(\Omega\right):\restr{q_h}{K}\circ F_K\in\mathbb{Q}_{k}\left(K\right)\quad\forall\ K\in\mathcal T_h\},\qquad\text{for quadrilaterals,}
\end{aligned}
\end{equation*}
where $\mathbb{RT}_k(K) :=\{\mathcal P_{K}\hat\w_h: \hat\w_h\in\mathbb {RT}_k(\hat K) \}$.  Remember that in the pure Neumann case, i.e., $\Gamma=\Gamma_N$, we have to filter out constant discrete pressures by imposing the zero average constraint to the space $Q_h$. 
%and modify the discrete velocities consequently. In this case, let us modify the discrete spaces as follows.
%\begin{align*}
%V_h:=\{\v_h \in V_h:\int_\Gamma \v_h\cdot\n =\int_\Omega g\},\qquad Q_h:=\{q_h\in Q_h:\int_{\Omega}q_h=0 \},\qquad\text{if $\Gamma=\Gamma_N$}.
%\end{align*}
%\begin{align*}
%Q_h:=\{q_h\in Q_h:\int_{\Omega}q_h=0 \},\qquad\text{if $\Gamma=\Gamma_N$}.
%\end{align*}
Let us construct the interpolation operator onto the discrete velocities $r_h:\prod_{K\in\mathcal T_h}\bm H^s(K)  \to V_h$ by gluing together the local interpolation operators $r_K:\bm H^s(K)\to \mathbb {RT}_k(K)$, $s>\frac{1}{2}$, and using the natural degrees of freedom of the Raviart-Thomas finite element. For every $\v\in \bm H^s(K)$, $s>\frac{1}{2}$, $r_K$ is uniquely defined by:
\begin{equation*}
	\begin{cases}
	\langle r_h \v\cdot \n_e, q_h \rangle_e= \langle \v\cdot\n_e, q_h\rangle_e \qquad&\forall\ q_h\in \mathbb{P}_k\left(e\right)\qquad\text{if}\;d=2,\\
		\langle r_h \v\cdot \n_f, q_h \rangle_f= \langle \v\cdot\n_f, q_h \rangle_f\qquad&\forall\ q_h\in \mathbb{Q}_{k}\left(f\right)\;\text{for quadrilaterals},\quad\forall\ q_h\in \mathbb{P}_{k}\left(f\right)\;\text{for triangles}\; \text{if}\;d=3,\\
		\left(r_h\v, \w_h\right)_K = \left(\v, \w_h\right)_K \qquad&\forall\ \w_h\in \psi\left(K\right)\qquad\text{if}\;k>0,\\
	\end{cases}
\end{equation*}
where, for $p>0$, for triangles
\begin{equation*}
	\psi\left(K\right):=\left(\mathbb P_{k-1}(K)\right)^d,
\end{equation*}
and for quadrilaterals
\begin{equation*}
	\psi\left(K\right):=
	\begin{cases}
		\mathbb{Q}_{k-1,{k}}(K)\times\mathbb{Q}_{k,k-1}(K)\qquad&\text{if}\;d=2,\\
		\mathbb{Q}_{k-1,{k},k}(K)\times \mathbb{Q}_{k,k-1,k}(K)\times\mathbb{Q}_{k,k,k-1}(K)\qquad&\text{if}\;d=3,
	\end{cases}
\end{equation*}
for all edges $e$, faces $f$ and triangles/quadrilaterals $K$ of $\mathcal T_h$. The natural choice in order to interpolate onto $Q_h$ is to employ an elementwise $L^2$-orthogonal projection, i.e., $\Pi_h: L^2\left(\Omega\right)\to Q_h$ such that for every $K\in\mathcal T_h$, $\restr{\Pi_h}{K}:=\Pi_K$, where for $\xi\in L^2(\Omega)$,
\begin{align*}
\left(\Pi_K \xi, q_h\right)_K &= \left(\xi, q_h\right)_K \qquad \forall\ q_h\in Q_h.
\end{align*}
for every $K\in\mathcal T_h$.
\begin{remark}
It is worth mentioning that the following Numerical Analysis remains valid if we employ another H(div) discretization instead, such as the so-called Brezzi-Douglas-Marini mixed element~\cite{brezzi_boffi}.
\end{remark}
\begin{proposition}\label{prop:cd}
	The following diagram commutes:
	\begin{equation}\label{comm_diag}
		\begin{CD}
			H(\dive;\Omega) \cap \prod_{K\in\mathcal T_h}\bm H^s(K)   @>\dive>> L^2(\Omega) \\
			@VVr_hV @VV\Pi_hV \\
			V_h @>\dive>> Q_h.
		\end{CD}	
%	\qquad\;\;
%		\begin{CD}
%	H_0(\dive;\Omega) \cap \prod_{K\in\mathcal T_h}\bm H^s(K)    @>\dive>> L^2_0(\Omega) \\
%	@VVr_hV @VV\Pi_hV \\
%	V_h^0 @>\dive>> Q_h^0.
%\end{CD}		
	\end{equation}
In particular, it holds
\begin{align*}
\dive V_h= Q_h.%,\qquad \dive V_h^0 \subseteq Q_h^0.
\end{align*}
\end{proposition}	
\begin{proof}
%	This is a well-established result. See for instance~\cite{ern_guermond}. 
For the commutative diagram note that, for every $\v\in H(\dive;\Omega) \cap \prod_{K\in\mathcal T_h}\bm H^s(K) $, it holds
\begin{align*}
\left( \Pi_h \dive \v,\varphi_h \right)_K	=& \left(\dive \v,\varphi_h \right)_K = -\left( \v,\nabla \varphi_h\right)_K +\langle \varphi_h, \v\cdot\n\rangle_{\partial K}\\
 = &-\left( r_h\v,\nabla \varphi_h\right)_K +\langle \varphi_h, r_h\v\cdot\n\rangle_{\partial K} = \left(\dive r_h\v ,\varphi_h\right)_K\qquad\forall\ \varphi\in\mathbb P_k(K) \;(\text{resp.}\; \mathbb Q_k(K)).
\end{align*}	
A direct calculation readily shows the inclusion $\dive V_h \subseteq Q_h$. Let us prove the other one. Let $q_h\in Q_h$, then, by the surjectivity of $\dive: \bm H^1(\Omega)\to\ L^2(\Omega)$~\cite{brezzi_boffi}, there exists $\v\in H(\dive;\Omega)\cap \prod_{K\in\mathcal T_h}\bm H^s(K)\subseteq \bm H^1(\Omega)$ such that $\dive\v=q_h$. Let us define $\v_h:= r_h\v$. Thanks to the commutativity diagram we have $\dive \v_h=q_h$.
\end{proof}
%For the sake of simplicity of the exposition we are always going to denote the discrete spaces as $V_h$ and $Q_h$. The reader should keep in mind that that in the pure Neumann case one needs to resort the spaces $V_h^0$ and $Q_h^0$.

We are now ready to introduce the discrete formulations we want to analyze. 

\subsubsection{First formulation}
Find $\left(\u_h,p_h\right)\in V_h\times Q_h$ such that
\begin{align}\label{eq:prob_disc}
\begin{cases}
a_h(\u_h,\v_h) + b_1(\v_h,p_h) =\left(\f,\v_h\right)_{\Omega}+   h^{-1}\langle u_N,\v_h\cdot\n \rangle_{\Gamma_N}+\langle p_D,\v_h\cdot\n\rangle_{\Gamma_D}\qquad&\forall\ \v_h\in V_h,\\
b_m(\u_h,q_h) =\left(g,q_h\right)_{\Omega} - m \langle q_h, u_N \rangle_{\Gamma_N}\qquad\qquad\qquad\qquad&\forall\ q_h\in Q_h,
\end{cases}
\end{align}
where $m\in \{0,1\}$. Here,
\begin{align}
	a_h(\u_h,\v_h):=\left(\u_h,\v_h\right)_{\Omega}+  h^{-1} \langle\u_h\cdot\n,\v_h\cdot\n \rangle_{\Gamma_N}\qquad&\forall\ \u_h,\v_h\in V_h,\\
	b_m(\u_h,p_h):= \left(p_h,\dive \u_h\right)_{\Omega}- m \langle p_h,\u_h\cdot\n \rangle_{\Gamma_N}\qquad&\forall\ \u_h\in V_h,p_h\in Q_h.
\end{align}
In what follows just the analysis for the symmetric case $m=1$ will be presented, however numerical results will be provided for the case $m = 0$ as well.

\subsubsection{Second formulation}
Find $\left(\u_h,p_h\right)\in V_h\times Q_h$ such that
\begin{align}\label{eq:prob_disc_bis}
\begin{cases}
a_\eps(\u_h,\v_h) + b_0(\v_h,p_h) =\left(\f,\v_h\right)_{\Omega} + \langle\eps^{-1} u_N+\chi_{\Gamma_D}p_D,\v_h\cdot\n \rangle_{\Gamma_N}+\langle p_D,\v_h\cdot\n\rangle_{\Gamma_D}\qquad&\forall\ \v_h\in V_h,\\
b_0(\u_h,q_h) =\left(g,q_h\right)_{\Omega} \qquad\qquad\qquad\qquad&\forall\ q_h\in Q_h.
\end{cases}
\end{align}
where
\begin{align*}
a_\eps(\u_h,\v_h):=\left(\u_h,\v_h\right)_{\Omega}+ \eps^{-1} \langle\u_h\cdot\n,\v_h\cdot\n \rangle_{\Gamma_N}\qquad&\forall\ \u_h,\v_h\in V_h.
\end{align*}
\begin{remark}
	Let us observe that the non-symmetric version of problem~\eqref{eq:prob_disc}, i.e., with $m=0$, and formulation~\eqref{eq:prob_disc_bis}, thanks to Proposition~\ref{prop:cd} allows for a \emph{weakly divergence-free} numerical solution $\u_h$, namely $\dive \u_h=0$ in the sense of $L^2$, provided that the right hand side $g$ vanishes.
\end{remark}
\begin{lemma}
Formulations~\eqref{eq:prob_disc} and~\eqref{eq:prob_disc_bis} are consistent discretizations of~\eqref{eq:prob_cont} and~\eqref{eq:prob_cont_bis} respectively.
\end{lemma}
\begin{proof}
	It is clear that~\eqref{eq:prob_disc} is a consistent discetization of~\eqref{eq:prob_cont}.
	Let $\left(\u^\eps,p^\eps\right)$ be the solution to~\eqref{eq:prob_cont_bis}. Of course, we have
	\begin{align*}
	b_0(\u^\eps,q_h)=\left(g,q_h\right)\qquad\forall\ q_h\in Q_h.	
	\end{align*}		
	By integrating by parts the first equation of~\eqref{eq:prob_cont_bis}, we obtain
	\begin{align}\label{perturb5}
	\left(\u^\eps,\v_h\right)_{\Omega} + b_0(\v_h,p^\eps)-\langle p^\eps, \v_h\cdot\n\rangle_{\Gamma_N} =\left(\f,\v_h\right)_{\Omega}+\langle p_D,\v_h\cdot\n \rangle_{\Gamma_D}\qquad\forall\ \v_h\in V_h.
	\end{align}
	By performing \emph{static condensation} of the multiplier from the boundary conditions, we obtain
	\begin{align}\label{perturb6}
	p^\eps	= \chi_{\Gamma_D} p_D+\eps^{-1}\left( \u_N-\u^\eps\cdot\n  \right)\qquad\text{on}\;\Gamma_N.
	\end{align}	
	Substituting~\eqref{perturb6} back into~\eqref{perturb5}, we obtain
	\begin{align*}
	a_\eps(\u^\eps,\v_h) + b_0(\v_h,p^\eps) =\left(\f,\v_h\right)_{\Omega}+ \langle \eps^{-1}\u_N + \chi_{\Gamma_D} p_D ,\v_h\cdot\n \rangle_{\Gamma_N}+\langle p_D,\v_h\cdot\n\rangle_{\Gamma_D}\qquad\forall\ \v_h\in V_h.
	\end{align*}
\end{proof}	
For the numerical analysis of~\eqref{eq:prob_disc}, we endow the discrete spaces with the following mesh-dependent norms
\begin{align*}
	\norm{\v_h}^2_{0,h}&:= \norm{\v_h}^2_{L^2(\Omega)} + \sum_{f\in\mathcal F_h^\partial(\Gamma_N)} h^{-1}\norm{\v_h\cdot\n}^2_{L^2(f)},  \\
	\norm{q_h}^2_{1,h}&:= \sum_{K\in\mathcal T_h}\norm{\nabla q_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i}h^{-1}\norm{\left[q_h\right]}^2_{L^2(f)} + \sum_{f\in\mathcal F_h^\partial(\Gamma_D)}h^{-1}\norm{q_h}^2_{L^2(f)},
\end{align*}
while for~\eqref{eq:prob_disc_bis} we are going to employ:
\begin{align*}
	\norm{\v_h}^2_{0,h,\eps}&:= \norm{\v_h}^2_{L^2(\Omega)} + \sum_{f\in\mathcal F_h^\partial(\Gamma_N)} \eps^{-1} \norm{\v_h\cdot\n}^2_{L^2(f)},  \\
		\norm{q_h}^2_{1,h,\eps}&:= \sum_{K\in\mathcal T_h}\norm{\nabla q_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i}h^{-1}\norm{\left[q_h\right]}^2_{L^2(f)} + \sum_{f\in\mathcal F_h^\partial}h^{-1}\norm{q_h}^2_{L^2(f)},
\end{align*}
for every $\v_h\in V_h$ and $q_h\in Q_h$.
\begin{remark}
	Informally speaking, the idea of both approaches is to unbalance the norms in order to go back to the elliptic case. Note that the natural functional setting for the mixed formulation of the Poisson problem is $H(\dive;\Omega)\times L^2(\Omega)$, but here we consider norms that induce the same topology as that of $\left[L^2(\Omega)\right]^d\times H^1(\Omega)$. Moreover, we observe that in both formulations~\eqref{eq:prob_disc} and~\eqref{eq:prob_disc_bis} a superpenalty parameter $\gamma$ is imposed in the flux variable. Indeed, the natural weight, mimicking the $H^{-\frac{1}{2}}$-scalar product, would be $h \langle\u_h\cdot\n, \v_h\cdot\n \rangle_{\Gamma_N}$. However such a weight does not lead to an optimally converging scheme. In addition, this is also what destroys the conditioning (see subsection~\ref{conditioning}).
%	
%	Indeed, if we consider the mixed problem in its strong form~\eqref{eq:prob_cont}, we realize that this second choice allow us to go back to the elliptic case via static condensation of the dual variable. In other words the space of multipliers has been chosen large enough so that $\nabla Q\subseteq V$.
\end{remark}
%----------------------------------------------------------------------------------------------------
\section{Stability estimates}
In this section we carry on at the same time the proofs of the well-posedness of the two discrete formulations.
\begin{proposition}
	There exist $M_{a_h}, M_{a_{\eps}}, M_{b_m}>0$, $m=0,1$, such that	
	\begin{align*}	
		\abs{a_h (\w_h,\v_h)}	\le M_{a_h} \norm{\w_h}_{0,h}\norm{\v_h}_{0,h}\qquad &\forall\ \w_h,\v_h\in V_h,\\
		\abs{a_{\eps} (\w_h,\v_h)}	\le M_{a_\eps} \norm{\w_h}_{0,h,\eps}\norm{\v_h}_{0,h,\eps}\qquad &\forall\ \w_h,\v_h\in V_h,\\
		\abs{b_1(\v_h,q_h)} \le  M_{b_1} \norm{\v_h}_{0,h}\norm{q_h}_{1,h}\qquad &\forall\ \v_h\in V_h,\ q_h\in Q_h, \\
		\abs{b_0(\v_h,q_h)} \le  M_{b_0} \norm{\v_h}_{0,h,\eps}\norm{q_h}_{1,h,\eps}\qquad &\forall\ \v_h\in V_h,\ q_h\in Q_h.
	\end{align*}	
\end{proposition}	
\begin{proof}
	Let $\w_h,\v_h\in V_h$, $q_h\in Q_h$ be arbitrary. It holds
	\begin{align*}
\abs{a_h(\w_h,\v_h)}\le &\norm{\w_h}_{L^2(\Omega)} \norm{\v_h}_{L^2(\Omega)} + h^{-\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(\Gamma_N)}h^{-\frac{1}{2}}\norm{\w_h\cdot\n}_{L^2(\Gamma_N)}\le \norm{\w_h}_{0,h} \norm{\v_h}_{0,h},\\
\abs{a_\eps(\w_h,\v_h)}\le& \norm{\w_h}_{L^2(\Omega)} \norm{\v_h}_{L^2(\Omega)} + \eps^{-\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(\Gamma_N)}\eps^{-\frac{1}{2}}\norm{\w_h\cdot\n}_{L^2(\Gamma_N)}\le \norm{\w_h}_{0,h,\eps} \norm{\v_h}_{0,h,\eps}.
	\end{align*}
By integration by parts, we get
	\begin{align*}
		b_1(\v_h,q_h) =& \left(q_h,\dive\v_h\right)_\Omega - \langle q_h,\v_h\cdot\n\rangle_{\Gamma_N} = \sum_{K\in\mathcal T_h} \left(q_h,\dive \v_h\right)_K - \sum_{f\in\mathcal F_h^\partial(\Gamma_N)}\langle q_h,\v_h\cdot\n\rangle_f\\
		=&-\sum_{K\in\mathcal T_h} \left(\nabla q_h,\v_h\right)_K + \sum_{f\in\mathcal F_h^i}\langle \left[q_h \right],\v_h\cdot\n \rangle_f+ \sum_{f\in\mathcal F_h^\partial(\Gamma_D)}\langle q_h ,\v_h\cdot\n \rangle_f.
	\end{align*}
	Thus,
	\begin{align*}
		\abs{b_1(\v_h,q_h)}\le& \sum_{K\in\mathcal T_h}\norm{\nabla q_h}_{L^2(K)}\norm{\v_h}_{L^2(K)} + \sum_{f\in\mathcal F_h^i} h^{-\frac{1}{2}}\norm{\left[q_h\right]}_{L^2(f)}h^{\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(f)} \\
		 &+ \sum_{f\in\mathcal F_h^\partial(\Gamma_D)} h^{-\frac{1}{2}}\norm{q_h}_{L^2(f)}h^{\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(f)}.
	\end{align*}
We recall some standard inverse inequalities, namely,
\begin{equation}
	\begin{aligned}
		h^{\frac{1}{2}} \norm{\v_h\cdot\n}_{L^2(f)} \lesssim \norm{\v_h}_{L^2(K)}\qquad f\in\mathcal F_h^\partial(\Gamma_D), f\in\mathcal F_h^i, f\subset \partial K \label{eq:disc_inv_ineq}.
\end{aligned}
\end{equation}
In this way we obtain
\begin{align*}
\abs{b_1(\v_h,q_h)}\lesssim 	& \norm{\v_h}_{0,h} \norm{q_h}_{1,h}.
\end{align*}
 On the other hand,
	\begin{align*}
	b_0(\v_h,q_h) =& -\sum_{K\in\mathcal T_h} \left(\nabla q_h,\v_h\right)_K +\langle q_h,\v_h\cdot\n\rangle_{\partial K} = 
	-\sum_{K\in\mathcal T_h} \left(\nabla q_h,\v_h\right)_K+ \sum_{f\in\mathcal F_h^i} \langle \left[q_h\right],\v_h\cdot\n\rangle_f\\
	&  + \sum_{f\in\mathcal F_h^\partial(\Gamma_N)} \langle q_h,\v_h\cdot\n\rangle_f   + \sum_{f\in\mathcal F_h^\partial(\Gamma_D)} \langle q_h,\v_h\cdot\n\rangle_f.
	\end{align*}
We have
	\begin{align*}
	\abs{b_0(\v_h,q_h)}\le & \sum_{K\in\mathcal T_h} \norm{\nabla q_h}_{L^2(K)}\norm{\v_h}_{L^2(K)}+\sum_{f\in\mathcal F_h^i} h^{-\frac{1}{2}}\norm{\left[q_h\right]}_{L^2(f)}h^{\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(f)} \\
	&+\sum_{f\in\mathcal F_h^\partial} h^{-\frac{1}{2}}\norm{q_h}_{L^2(f)}h^{\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(f)} \lesssim \norm{\v_h}_{0,h,\eps}\norm{q_h}_{1,h,\eps},
	\end{align*}
having used again~\eqref{eq:disc_inv_ineq} and $h^{-\frac{1}{2}}<\eps^{-\frac{1}{2}}$ for $\eps \ll h$.  
\end{proof}
\begin{proposition}
	There exist ${\alpha_{a_h}},\alpha_{a_\eps}>0$ such that
	\begin{align*}
		a_{h}(\v_h,\v_h)\ge &\alpha_{a_h} \norm{\v_h}^2_{0,h}\qquad\forall\ \v_h\in V_h,\\
		a_{\eps}(\v_h,\v_h)\ge &\alpha_{a_\eps} \norm{\v_h}^2_{0,h,\eps}\qquad\forall\ \v_h\in V_h.
	\end{align*}
	\begin{proof}
		Let us take $\v_h\in V_h$ arbitrary and compute
		\begin{align*}
			a_h(\v_h,\v_h) = &\norm{\v_h}^2_{L^2(\Omega)}+  h^{-1}\norm{\v_h\cdot\n}^2_{L^2(\Gamma_N)} 
		= \norm{\v_h}^2_{0,h}.
		\end{align*}
		 The other coercivity estimate follows anologously. Hence, $\alpha_{a_h}=\alpha_{a_\eps}=1$.
	\end{proof}
\end{proposition}
\begin{proposition}\label{prop:infsup_fitted}
	There exist $\beta_m>0$, $m\in\{0,1\}$, such that	
	\begin{align*}	
	\inf_{q_h\in Q_h}\sup_{\v_h\in V_h} \frac{b_1(\v_h,q_h)}{\norm{\v_h}_{0,h}\norm{q_h}_{1,h}}	\ge &\beta_1,\\
	\inf_{q_h\in Q_h}\sup_{\v_h\in V_h} \frac{b_0(\v_h,q_h)}{\norm{\v_h}_{0,h,\eps}\norm{q_h}_{1,h,\eps}}	\ge& \beta_0.
	\end{align*}	
\end{proposition}	
\begin{proof}
	We start with $m=1$. Let us fix $q_h\in Q_h$ arbitrary. We construct $\v_h$ by using the dofs of the Raviart-Thomas space.
	\begin{align}
		\langle \v_h\cdot\n,\varphi_h \rangle_f =  h^{-1} \langle \left[q_h\right],\varphi_h\rangle_f\qquad&\forall\ f\in\mathcal F_h^i,\ \varphi_h\in\mathbb P_k(f),\label{stab:eq1}\\
		\langle \v_h\cdot\n,\varphi_h\rangle_f =0\qquad&\forall\ f\in\mathcal F_h^{\partial}(\Gamma_N),\ \varphi_h\in\mathbb P_k(f), \label{stab:eq2}\\
				\langle \v_h\cdot\n,\varphi_h\rangle_f =h^{-1} \langle q_h,\varphi_h\rangle_f\qquad&\forall\ f\in\mathcal F_h^{\partial}(\Gamma_D),\ \varphi_h\in\mathbb P_k(f), \label{stab:eq4}\\
		\left(\v_h,\bm\psi_h \right)_K = -\left(\nabla q_h,\bm\psi_h \right)_K\qquad&\forall\ K\in\mathcal T_h,\ \bm\psi_h\in\left[\mathbb P_{k-1}(K) \right]^d,\ \text{if}\ k>0. \label{stab:eq3}
	\end{align}	
	By using the definition of $\v_h$,
	\begin{align*}
		b_1(\v_h,q_h) =&  \left(q_h,\dive\v_h \right)_{\Omega} - \langle q_h,\v_h\cdot\n\rangle_{\Gamma_N} = \sum_{K\in\mathcal T_h} \left(q_h,\dive\v_h\right)_K - \sum_{f\in\mathcal F_h^{\partial}(\Gamma_N)} \langle q_h,\v_h\cdot\n\rangle_f \\
		=&-\sum_{K\in\mathcal T_h}\left( \nabla q_h,\v_h \right)_K  + \langle q_h, \v_h\cdot\n\rangle_{\partial K} - \sum_{f\in\mathcal F_h^{\partial}(\Gamma_N)} \langle q_h,\v_h\cdot\n\rangle_f \\
		=& -\sum_{K\in\mathcal T_h}\left( \nabla q_h,\v_h \right)_K +\sum_{f\in\mathcal F_h^i} \langle \left[q_h\right],\v_h\cdot\n\rangle_f +\sum_{f\in\mathcal F_h^{\partial}(\Gamma_D)} \langle q_h,\v_h\cdot\n\rangle_f\\
		=& \sum_{K\in\mathcal T_h} \norm{\nabla q_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i}h^{-1} \norm{\left[q_h\right]}^2_{L^2(f)} + \sum_{f\in\mathcal F_h^\partial(\Gamma_D)}h^{-1}\norm{q_h}^2_{L^2(f)}  = \norm{q_h}^2_{1,h}.
	\end{align*}
		Finally, let us show that $\norm{\v_h}_{0,h}\le C \norm{q_h}_{1,h}$. Note that for every $f\in\mathcal F_h^{\partial}(\Gamma_N)$, since $\restr{\v_h\cdot\n}{f} \in\mathbb P_k(f)$, \eqref{stab:eq2} implies
	\begin{align*}
	\norm{\v_h\cdot\n }^2_{L^2(f)} = \langle \v_h\cdot\n,\v_h\cdot\n \rangle_{f} =0 \qquad\Rightarrow\qquad \norm{\v_h\cdot\n}_{L^2(f)}=0.
	\end{align*}
	Then, let us show $\norm{\v_h}_{L^2(\Omega)} \le C \norm{ q_h}_{1,h}$. From~\eqref{stab:eq1} it holds $\restr{\v_h\cdot\n}{f}=h_K^{-1} \restr{\pi_{f,k}\left[q_h\right] }{f}$ for every $f\in\mathcal{F}_h^i$ and from~\eqref{stab:eq3} we have $\restr{\pi_{K,k-1}\v_h}{K} =- \restr{\pi_{K,k-1}\nabla q_h}{K}$ for every $K\in\mathcal T_h$. Note that here $\pi_{K,k-1}$ denotes the $L^2$-orthogonal projection onto $\left[\mathbb P_{k-1}(K)\right]^d$. Similarly for $\pi_{f,k}$. By finite dimensionality it holds $\norm{\hat \v_h}^2_{L^2(\hat K)} \lesssim \norm{\pi_{\hat K,k-1}\hat \v_h}^2_{L^2(\hat K)} + \norm{\hat \v_h\cdot\hat \n}^2_{L^2(\hat f)}$.  Hence, $\norm{\v_h}^2_{L^2(K)}\lesssim \norm{\nabla q_h}^2_{L^2(K)}+h_K^{-1}\norm{[q_h]}^2_{L^2(f)}$, $f$ being an edge (or, respectively, face in 3D) of $K$, which follows by a standard scaling argument (see Proposition 2.1 of~\cite{doi:10.1137/17M1163335}) and  by construction of $\v_h$.
	
	Let us now take $m=0$ and $q_h\in Q_h$. We define $\u_h$ as follows:
		\begin{align}
	\langle \v_h\cdot\n,\varphi_h \rangle_f = h^{-1} \langle \left[q_h\right],\varphi_h\rangle_f\qquad&\forall\ f\in\mathcal F_h^i,\ \varphi_h\in\mathbb P_k(f),\label{stab:eq1bis}\\
	\langle \v_h\cdot\n,\varphi_h\rangle_f = h^{-1}\langle q_h,\varphi_h\rangle_f \qquad&\forall\ f\in\mathcal F_h^{\partial}(\Gamma_N),\ \varphi_h\in\mathbb P_k(f),\label{stab:eq2bis}\\
		\langle \v_h\cdot\n,\varphi_h\rangle_f = h^{-1}\langle q_h,\varphi_h\rangle_f  \qquad&\forall\ f\in\mathcal F_h^{\partial}(\Gamma_D),\ \varphi_h\in\mathbb P_k(f),\label{stab:eq4bis}\\
	\left(\v_h,\bm\psi_h \right)_K = -\left(\nabla q_h,\bm\psi_h \right)_K\qquad&\forall\ K\in\mathcal T_h,\ \bm\psi_h\in\left[\mathbb P_{k-1}(K) \right]^d,\ \text{if}\ k>0\label{stab:eq3bis}. 
	\end{align}	
	\begin{align*}
		b_0(\v_h,q_h) =&  \left(q_h,\dive\v_h \right)_{\Omega} = \sum_{K\in\mathcal T_h} \left(q_h,\dive\v_h\right)_K=-\sum_{K\in\mathcal T_h}\left( \nabla q_h,\v_h \right)_K  +  \langle q_h, \v_h\cdot\n\rangle_{\partial K}  \\
		=& -\sum_{K\in\mathcal T_h}\left( \nabla q_h,\v_h \right)_K +\sum_{f\in\mathcal F_h^i} \langle \left[q_h\right],\v_h\cdot\n\rangle_f +\sum_{f\in\mathcal F_h^\partial(\Gamma_N)} \langle q_h,\v_h\cdot\n\rangle_f +\sum_{f\in\mathcal F_h^\partial(\Gamma_D)} \langle q_h,\v_h\cdot\n\rangle_f\\
		=& \sum_{K\in\mathcal T_h} \norm{\nabla q_h}^2_{L^2(K)}+ \sum_{f\in\mathcal F_h^i} h^{-1}\norm{\left[q_h\right]}^2_{L^2(f)}+\sum_{f\in\mathcal F_h^\partial}h^{-1}\norm{q_h}^2_{L^2(f)}=\norm{q_h}^2_{1,h,\eps}.
	\end{align*}
	We refer to~\cite{konno_robin} for the inequality $\norm{\v_h}_{0,h,\eps}\le C \norm{q_h}_{1,h,\eps}$. 
\end{proof}	


%---------------------------------------------------------------------------------------------------------------
\section{A priori error estimates}
  \begin{lemma}\label{apriori:lemma1_m=1}
  	Let $\left(\bm\u,p\right)$ be the solution of the continuous problem~\eqref{eq:prob_cont} and $\left(\bm\u_h,p_h\right)\in V_h\times Q_h$ the one of the discrete problem~\eqref{eq:prob_disc} with $m=1$. Then
  	\begin{equation}
  	\norm{\bm\u_h - r_h\bm\u}_{0,h}+\norm{p_h-\pi_hp}_{1,h}\lesssim \norm{\bm\u-r_h\bm\u}_{L^2(\Omega)}+ h^{\frac{1}{2}}\sum_{f\in\mathcal F_h^\partial(\Gamma_N)}\norm{p-\pi_h p}_{L^2(f)}.
  	\end{equation}
  \end{lemma}	
  \begin{proof}
The stability estimates previously shown for $a_h(\cdot,\cdot)$ and $b_1(\cdot,\cdot)$ with respect to $\norm{\cdot}_{0,h}$ and $\norm{\cdot}_{1,h}$ imply
  \begin{equation}\label{eq:global_inv_m=1}
  \vertiii{\bm\eta_h,s_h}_h \lesssim \sup_{\left(\bm\v_h,q_h\right)} \frac{\mathcal A_h \left( \left(\bm\eta_h,s_h\right),\left(\bm\v_h,q_h\right)\right)}{\vertiii{\bm\v_h,q_h}_h}\qquad\forall\ \left(\bm\eta_h,s_h \right)\in V_h\times Q_h,
  \end{equation}
where
\begin{align*}
\mathcal A_h \left( \left(\bm\eta_h,s_h\right),\left(\bm\v_h,q_h\right)\right) :=& a_h(\bm\eta_h,\v_h) + b_1(\v_h,s_h) + b_1(\bm\eta_h,q_h),\\
\vertiii{\bm\eta_h,s_h}_h^2:=& \norm{\bm\eta_h}^2_{0,h} + \norm{s_h}^2_{1,h}.
\end{align*}
Using~\eqref{eq:global_inv_m=1}, for $(\bm\u_h-r_h\bm\u,p_h-\pi_hp)$ there exists $\left(\v_h,q_h\right)\in V_h\times Q_h$ such that
\begin{align*}
\norm{\bm\u_h-r_h\bm\u_h}_{0,h}+\norm{p_h-\pi_h p}_{1,h} \le& \sqrt{d} \vertiii{\bm\u_h-r_h\bm\u,p_h-\pi_h p}_h\lesssim 
\frac{\mathcal A_h\left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\v_h,q_h\right)\right)}{\vertiii{\v_h,q_h}_h}.
\end{align*}
Hence, we have
\begin{equation}\label{eq1:apriori_m=1}
\begin{aligned}
\mathcal A_h \left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\v_h,q_h\right)\right) =& \left(\u_h-\u,\v_h\right)_{L^2(\Omega)}+\left(\u-r_h\u,\v_h\right)_{L^2(\Omega)}+h^{-1}\langle \left(\u_h-\u\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N}\\
&+h^{-1}\langle\left(\u-r_h\u\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N}+b_0(\v_h,p_h-p)+b_0(\v_h,p-\pi_hp)\\
&-\langle p_h-p,\v_h\cdot\n \rangle_{\Gamma_N} - \langle p-\pi_h p,\v_h\cdot\n \rangle_{\Gamma_N}\\
 &+b_1(\u_h-\u,q_h)+b_1(\u-r_h\u,q_h).
\end{aligned}
\end{equation}	
By construction of $r_h$ and $\pi_h$ we have, respectively,
\begin{equation}\label{eq:orthogonaly_relations}
\begin{aligned}
h^{-1}\langle (\u-r_h\u)\cdot\n,\v_h\cdot\n \rangle_{\Gamma_N}=0\qquad&\forall\ \v_h\in V_h,\\
b_1(\u-r_h\u,q_h) = -\sum_{K\in\mathcal T_h} \left(\nabla q_h,\u-r_h\u\right)_K + \sum_{f\in\mathcal F_h^i}\langle [q_h],\left(\u-r_h\u\right)\cdot\n \rangle_f=0\qquad&\forall\ q_h\in Q_h, \\
b_0(\v_h,p-\pi_h p)=0\qquad&\forall\ \v_h\in V_h.
\end{aligned}
\end{equation}
By consistency, we have
\begin{align*}
\left(\u_h-\u,\v_h\right)_{L^2(\Omega)}+h^{-1}\langle \left(\u_h-\u\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N}+b_0(\v_h,p_h-p)+\langle p_h-p,\v_h\cdot\n \rangle_{\Gamma_N}=0\qquad&\forall\ \v_h\in V_h,\\
b_1(\u_h-\u,q_h) = 0\qquad &\forall\ q_h\in Q_h.
\end{align*}
Hence, in~\eqref{eq1:apriori_m=1} we are left with
\begin{align*}
\mathcal A_h \left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\v_h,q_h\right)\right) =\left(\u-r_h\u,\v_h\right)_{L^2(\Omega)}
- \langle p-\pi_h p,\v_h\cdot\n \rangle_{\Gamma_N} .
\end{align*}
We have
\begin{align*}
\left(\u-r_h\u,\v_h\right)_{L^2(\Omega)}
- \langle p-\pi_h p,\v_h\cdot\n \rangle_{\Gamma_N} \le \norm{\u-r_h\u}_{L^2(\Omega)}\norm{\v_h}_{L^2(\Omega)} + \sum_{f\in\mathcal F_h^\partial(\Gamma_N)}h^{\frac{1}{2}}\norm{\left(p-\pi_h p\right)}_{L^2(f)}h^{-\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(\Gamma_N)},
\end{align*}
and we can write
\begin{align*}
\norm{\u_h - r_h\u}_{0,h}+\norm{p_h-\pi_h p}_{1,h}\lesssim & \frac{\left(\norm{\u-r_h\u}_{L^2(\Omega)}+h^{\frac{1}{2}}\sum_{f\in\mathcal F_h^\partial(\Gamma_N)}\norm{p-\pi_hp}_{L^2(f)} \right)\vertiii{\v_h,0}_h}{\vertiii{\v_h,q_h}_h} \\
\lesssim& \norm{\u-r_h\u}_{L^2(\Omega)}+h^{\frac{1}{2}}\sum_{f\in\mathcal F_h^\partial(\Gamma_N)}\norm{p-\pi_hp}_{L^2(f)}.
\end{align*}
\end{proof}
% \begin{lemma}\label{apriori:lemma1_ns}
%	Let $\left(\bm\u,p\right)\in V\times Q$ be the solution of the continuous problem~\eqref{eq:prob_cont} and $\left(\bm\u_h,p_h\right)\in V_h\times Q_h$ the one of the discrete problem~\eqref{eq:prob_disc_sym} with $m=0$. Then
%	\begin{equation}
%	\norm{\bm\u_h - r_h\bm\u}_{0,h}+\norm{p_h-\pi_hp}_{1,h,?}\lesssim \norm{\bm\u-r_h\bm\u}_{L^2(\Omega)}+ \sum_{f\in\mathcal F_h^\partial}\norm{\eps^{-\frac{1}{2}}\left(p-\pi_hp\right)}_{L^2(f)}.
%	\end{equation}
%\end{lemma}	
%\begin{proof}
%\textcolor{red}{Let assume that we are able to prove the usual stability estimates for $a_1(\cdot,\cdot)$, $b_0(\cdot,\cdot)$ and $b_1(\cdot,\cdot)$ with respect to $\norm{\cdot}_{0,h}$ and $\norm{\cdot}_{1,h,?}$ (the last norm has subscript ? because so far we do not know which norm on $Q_h$ guarantees at the same time the continuity and inf-sup stability of $b_0(\cdot,\cdot)$ and $b_1(\cdot,\cdot)$).}	Then the following global stability estimates holds:
%	\begin{equation}\label{apriori:eq1}
%	\vertiii{\bm\eta,s_h} \lesssim \sup_{\left(\bm\tau_h,q_h\right)} \frac{\mathcal A \left( \left(\bm\eta_h,s_h\right),\left(\bm\tau_h,q_h\right)\right)}{\vertiii{\bm\tau_h,q_h}}\qquad\forall\ \left(\bm\eta_h,s_h \right)\in V_h\times Q_h,
%	\end{equation}
%	where
%	\begin{align*}
%	\mathcal A \left( \left(\bm\eta_h,s_h\right),\left(\bm\tau_h,q_h\right)\right) :=& a_1(\bm\eta_h,\v_h) + b_1(\v_h,s_h) + b_0(\bm\eta_h,q_h),\\
%	\vertiii{\bm\eta_h,s_h}^2:=& \norm{\bm\eta_h}^2_{0,h} + \norm{s_h}^2_{1,h,?}.
%	\end{align*}
%	Hence, for $(\bm\u_h-r_h\bm\u,p_h-\pi_hp)$ there exists $\left(\v_h,q_h\right)\in V_h\times Q_h$ such that
%	\begin{align*}
%		\norm{\bm\u_h-r_h\bm\u}_{0,h}+\norm{p_h-\pi_h p}_{1,h,?} \le& \sqrt{d} \vertiii{\bm\u_h-r_h\bm\u,p_h-\pi_h p}\lesssim 
%		\frac{\mathcal A \left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\bm\tau_h,q_h\right)\right)}{\vertiii{\bm\tau_h,q_h}}.
%	\end{align*}
%	Hence, we have
%	\begin{align*}
%		\mathcal A \left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\bm\tau_h,q_h\right)\right) =& a_0(\u_h-\u,\v_h)+a_0(\u-r_h\u,\v_h)+\eps\langle \left(\u_h-\u\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma}+\eps\langle\left(\u-r_h\u\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma}\\
%		&+b_0(\v_h,p_h-p)+b_0(\v_h,p-\pi_hp) + \langle p_h-p,\v_h\cdot\n  \rangle_{\Gamma} +\langle p-\pi_hp, \v_h\cdot\n\rangle_{\Gamma}\\
%		&+b_0(\u_h-\u,q_h)+b_0(\u-r_h\u,q_h).
%	\end{align*}
%	The following orthogonality relations hold by definition of $r_h$ and $\pi_h$:
%	\begin{align}
%		\eps\langle\left(\u-r_h\u\right)\cdot\n,\v_h\rangle_{\Gamma} &= 0\qquad\forall\ \v_h\in V_h,\\
%		b_0(\bm\tau_h,p-\pi_h p)&=0 \qquad\forall\ \v_h\in V_h,\\
%		b_0(\u-r_h\u,q_h) =& -\sum_{K\in\mathcal T_h}\left(\nabla q_h,\u-r_h\u\right)_K\\
%		& + \sum_{f\in\mathcal F_h^i}\langle [q_h],\left(\u-r_h\u\right)\cdot\n\rangle_f+ \sum_{f\in\mathcal F_h^\partial}\langle q_h,\left(\u-r_h\u\right)\cdot\n\rangle_f=0\qquad\forall\ q_h\in Q_h.
%		\label{apriori:eq6}
%	\end{align}
%	Moreover, by consistency, we have
%	\begin{align*}
%		a_0(\u_h-\u,\v_h)+\eps \langle \left( \u_h-\u\right)\cdot\n,\v_h\cdot\n\rangle_\Gamma + b_0(\v_h,p_h-p)+\langle p_h-p,\v_h\cdot\n\rangle_\Gamma = &\eps \langle \u_N-\u_h\cdot\n,\v_h\cdot\n\rangle_\Gamma = 0\qquad\forall\ \v_h\in\tilde V_h,\\
%		 b_0(\u_h-\u,q_h) =& 0\qquad\forall\ q_h\in Q_h.
%	\end{align*}
%	Hence,
%	\begin{align*}
%		\mathcal A \left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\bm\tau_h,q_h\right)\right)= & a_0(\u-r_h\u,\v_h)+\langle p-\pi_h p,\v_h\cdot\n\rangle_{\Gamma}\\
%		\le& \norm{\u-r_h\u}_{L^2(\Omega)}\norm{\v_h}_{L^2(\Omega)} + \sum_{f\in\mathcal F_h^\partial}\norm{\eps^{-\frac{1}{2}}\left(p-\pi_h p\right)}_{L^2(f)}\norm{\eps^{\frac{1}{2}}\v_h\cdot\n}_{L^2(\Gamma)},
%	\end{align*}
%and we can write
%\begin{align*}
%\norm{\u_h - r_h\u}_{0,h}+\norm{p_h-\pi_h p}_{1,h,?}\lesssim & \frac{\left(\norm{\u-r_h\u}_{L^2(\Omega)}+\sum_{f\in\mathcal F_h^\partial}\norm{\eps^{-\frac{1}{2}}\left(p-\pi_hp\right)}_{L^2(f)} \right)\vertiii{\v_h,0}}{\vertiii{\v_h,q_h}} \\
%\lesssim& \norm{\u-r_h\u}_{L^2(\Omega)}+\sum_{f\in\mathcal F_h^\partial}\norm{\eps^{-\frac{1}{2}}\left(p-\pi_hp\right)}_{L^2(f)}.
%\end{align*}
%\end{proof}	
%-----------------------------------------------------------------------------------------------------------------------------
%\textcolor{blue}{
%\begin{remark}[A comment on the generalization to the unfitted case]	
%Let us focus on the analysis of formulation~\eqref{eq:prob_disc}. In the unfitted case we lack the orthogonality relations~\eqref{eq:orthogonaly_relations}. We take for instance the first one. We need to recover the penalty parameter $\gamma>0$ such that the term $\gamma \langle  \left(\u-r_h\u \right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N}$ would give rise to an optimal estimate. Note that $\gamma$ appears also in the velocities norm as:
%\begin{align*}
%\norm{\v_h}^2_{0,h}:= \norm{\v_h}^2_{L^2(\Omega)} + \sum_{K\in\mathcal G_h} \gamma\norm{\v_h\cdot\n}^2_{L^2(\Gamma_K)}.
%\end{align*}
% We compute
%\begin{align*}
%\gamma \langle  \left(\u-r_h\u \right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N} \le h^{\frac{1}{2}}\norm{\u-r_h\u}_{L^2(\Gamma_N)}\gamma h^{-\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(\Gamma_N)}\le h^{\frac{1}{2}}\norm{\u-r_h\u}_{L^2(\Gamma_N)}\gamma \norm{\v_h}_{0,h}.
%\end{align*}
%In order to be able to perform the second inequality, we need to choose $\gamma$ such that $\gamma h^{-\frac{1}{2}} = \gamma^{\frac{1}{2}}$, namely $\gamma= h$. In this way we will have issues with the term $\langle p-\pi_h p , \v_h\cdot\n\rangle_{\Gamma_N}$:
%\begin{align}\label{eq:remark_gen}
%	\langle p-\pi_h p , \v_h\cdot\n\rangle_{\Gamma_N} \le \gamma^{-\frac{1}{2}}\norm{p-\pi_h p}_{L^2(\Gamma_N)}\gamma^{\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(\Gamma_N)}\le \left(\sum_{K\in\mathcal G_h }\gamma^{-\frac{1}{2}}\norm{p-\pi_h p}_{L^2(\Gamma_K)}\right) \norm{\v_h}_{0,h}.
%\end{align}
%We observe that for $\gamma= h$ the right hand side of~\eqref{eq:remark_gen} is suboptimal of $1$ order.
%\end{remark}}
 \begin{lemma}\label{apriori:lemma1_pert}
	Let $\left(\bm\u^\eps,p^\eps\right)$ be the solution of the perturbed continuous problem~\eqref{eq:prob_cont_bis} and $\left(\bm\u_h,p_h\right)\in V_h\times Q_h$ the one of the discrete problem~\eqref{eq:prob_disc_bis}. Then
	\begin{equation}
	\norm{\bm\u_h - r_h\bm\u^\eps}_{0,h,\eps}+\norm{p_h-\pi_hp^\eps}_{1,h,\eps}\lesssim \norm{\bm\u^\eps-r_h\bm\u^\eps}_{L^2(\Omega)}.
	\end{equation}
\end{lemma}	
\begin{proof}
The stability estimates previously shown for $a_\eps(\cdot,\cdot)$ and $b_0(\cdot,\cdot)$ with respect to $\norm{\cdot}_{0,h,\eps}$ and $\norm{\cdot}_{1,h,\eps}$ imply
	\begin{equation}\label{apriori:eq1_pert}
\vertiii{\bm\eta,s_h}_{h,\eps} \lesssim \sup_{\left(\v_h,q_h\right)} \frac{\mathcal A_\eps \left( \left(\bm\eta_h,s_h\right),\left(\v_h,q_h\right)\right)}{\vertiii{\v_h,q_h}_{h,\eps}}\qquad\forall\ \left(\bm\eta_h,s_h \right)\in V_h\times Q_h,
\end{equation}
where
\begin{align*}
\mathcal A_\eps \left( \left(\bm\eta_h,s_h\right),\left(\v_h,q_h\right)\right) :=& a_\eps(\bm\eta_h,\v_h) + b_0(\v_h,s_h) + b_0(\bm\eta_h,q_h),\\
\vertiii{\bm\eta_h,s_h}^2:=& \norm{\bm\eta_h}^2_{0,h,\eps} + \norm{s_h}^2_{1,h,\eps}.
\end{align*}
Hence, for $(\bm\u_h-r_h\bm\u^\eps,p_h-\pi_hp^\eps)$ there exists $\left(\v_h,q_h\right)\in V_h\times Q_h$ such that
\begin{align*}
\norm{\bm\u_h-r_h\bm\u^\eps}_{0,h,\eps}+\norm{p_h-\pi_h p^\eps}_{1,h,\eps} \le& \sqrt{d} \vertiii{\bm\u_h-r_h\bm\u^\eps,p_h-\pi_h p^\eps}_{h,\eps}\lesssim 
\frac{\mathcal A_\eps \left( \left(\bm\u_h-r_h\bm\u^\eps,p_h-\pi_h p^\eps\right),\left(\v_h,q_h\right)\right)}{\vertiii{\v_h,q_h}_{h,\eps}}.
\end{align*}
Hence, we have
\begin{align*}
\mathcal A_{\eps} \left( \left(\bm\u_h-r_h\bm\u^\eps,p_h-\pi_h p^\eps\right),\left(\v_h,q_h\right)\right) =& \left(\u_h-\u^\eps,\v_h\right)_{L^2(\Omega)}+\left(\u^\eps-r_h\u^\eps,\v_h\right)_{L^2(\Omega)}+\eps^{-1}\langle \left(\u_h-\u^\eps\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N}\\
&+\eps^{-1}\langle\left(\u^\eps-r_h\u^\eps\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N}
+b_0(\v_h,p_h-p^\eps)\\
&+b_0(\v_h,p^\eps-\pi_hp^\eps) +b_0(\u_h-\u^\eps,q_h)+b_0(\u^\eps-r_h\u^\eps,q_h).
\end{align*}
The following orthogonality relations hold by definition of $r_h$ and $\pi_h$:
\begin{alignat*}{3}
\eps^{-1}\langle\left(\u^\eps-r_h\u^\eps\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N} = &0\qquad&&\forall\ \v_h\in V_h,\\
b_0(\v_h,p^\eps-\pi_h p^\eps)=&0 \qquad&&\forall\ \v_h\in V_h,\\
b_0(\u^\eps-r_h\u^\eps,q_h) = -\sum_{K\in\mathcal T_h}\left(\nabla q_h,\u^\eps-r_h\u^\eps\right)_K\\
 + \sum_{f\in\mathcal F_h^i}\langle [q_h],\left(\u^\eps-r_h\u^\eps\right)\cdot\n\rangle_f+ \sum_{f\in\mathcal F_h^\partial(\Gamma_N)}\langle q_h,\left(\u^\eps-r_h\u^\eps\right)\cdot\n\rangle_f=&0\qquad&&\forall\ q_h\in Q_h.
\end{alignat*}
Moreover, by consistency, we have
\begin{align*}
\left(\u_h-\u^\eps,\v_h\right)_{L^2(\Omega)}+\eps \langle \left( \u_h-\u^\eps\right)\cdot\n,\v_h\cdot\n\rangle_{\Gamma_N} + b_0(\v_h,p_h-p^\eps) =   0\qquad&\forall\ \v_h\in V_h,\\
b_0(\u_h-\u^\eps,q_h) = 0\qquad&\forall\ q_h\in Q_h.
\end{align*}
Hence,
\begin{align*}
\mathcal A_\eps \left( \left(\bm\u_h-r_h\bm\u^\eps,p_h-\pi_h p^\eps\right),\left(\bm\tau_h,q_h\right)\right)=  \left(\u^\eps-r_h\u^\eps,\v_h\right)_{L^2(\Omega)},
\end{align*}
and we can write
\begin{align*}
\norm{\u_h - r_h\u^\eps}_{0,h,\eps}+\norm{p_h-\pi_h p^\eps}_{1,h,\eps}\lesssim  \frac{\norm{\u^\eps-r_h\u^\eps}_{L^2(\Omega)}\vertiii{\v_h,0}_{h,\eps}}{\vertiii{\v_h,q_h}_{h,\eps}} 
\lesssim \norm{\u^\eps-r_h\u^\eps}_{L^2(\Omega)}.
\end{align*}
\end{proof}	

	% If it is not the case, then, by integration by parts, we get
	%\begin{align*}
	%\mathcal A \left( \left(\bm\u_h-r_h\bm\u,p_h-\pi_h p\right),\left(\bm\tau_h,q_h\right)\right)=&
	%\left( \u - r_h\u,\v_h\right)_{\Omega} + \sum_{K\in\mathcal T_h} \left(\nabla \left( p-\pi_h p\right),\v_h \right)_K -\sum_{K\in\mathcal T_h} \langle p-\pi_h p,\v_h\cdot\n \rangle_{\partial K} \\
	%&  + \sum_{f\in\mathcal F_h^{\partial}} \langle p-\pi_h p,\v_h\cdot\n\rangle _f \\
	%=&  \left( \u - r_h\u,\v_h\right)_{\Omega} + \sum_{K\in\mathcal T_h} \left(\nabla \left( p-\pi_h p\right),\v_h \right)_K - \sum_{f\in\mathcal F_h^i} \langle \left[p-\pi_h p\right],\v_h\cdot\n  \rangle_f \\
	%\le & \norm{\u-r_h\u}_{L^2(\Omega)} \norm{\v_h}_{L^2(\Omega)} +  \norm{ p-\pi_h p }_{1,h}\norm{\v_h}_{L^2(\Omega)}.
	%\end{align*}
	%Hence, it seems we do not gain anything.
%	\begin{proposition}\label{apriori:prop1_m=0}
%		Let $\left(\bm\u,p\right) \in \left[H^{r+1}(\Omega)\right]^d\times H^{k+1}(\Omega)$ and $s:=\min\{r,k,p\}$ be the solution of~\eqref{eq:prob_cont} and $\left(\u_h,p_h\right)\in V_h\times Q_h$ the one to~\eqref{eq:prob_disc_sym} for $m=0$.
%		\begin{equation}\label{apriori:eq5_m=0}
%		\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h,ks}\le ???
%		\end{equation}	
%	\end{proposition}	
%	\begin{proof}
%		It follows by Lemma~\ref{apriori:lemma1_m=0} \textcolor{red}{(not available!)} and Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli}.	
%	\end{proof}	
	\begin{proposition}\label{apriori:prop1_m=1}
	Let $\left(\bm\u,p\right) \in \bm H^{r+1}(\Omega)\times H^{t+1}(\Omega)$ and $s:=\min\{r,t,k\}$ be the solution of~\eqref{eq:prob_cont} and $\left(\u_h,p_h\right)\in V_h\times Q_h$ the one to~\eqref{eq:prob_disc} with $m=1$. There exists $C>0$ such that
	\begin{equation}\label{apriori:eq5_m=1}
	\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h}\le C h^{s+1} \left( \norm{\u}_{H^{r+1}(\Omega)} +\norm{p}_{H^{t+1}(\Omega)}\right).
	\end{equation}	
\end{proposition}	
\begin{proof}
	By Lemma~\ref{apriori:lemma1_m=1}, a multiplicative trace inequality for Sobolev functions and standard approximation results for the $L^2$-projection
	\begin{align*}
\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h} \lesssim & \norm{\u-r_h\u}_{L^2(\Omega)} + \sum_{f\in\mathcal F_h^\partial(\Gamma_N)}h^{\frac{1}{2}}\norm{p-\pi_h p}_{L^2(f)} \\
\lesssim & \norm{\u-r_h\u}_{L^2(\Omega)} + \sum_{K\in\mathcal T_h}h^{\frac{1}{2}}\norm{p-\pi_h p}^{\frac{1}{2}}_{L^2(K)} \norm{\nabla\left(p-\pi_h p\right)}^{\frac{1}{2}}_{L^2(K)}  \\
\lesssim &  \norm{\u-r_h\u}_{L^2(\Omega)} + h^{\frac{1}{2}}h^{\frac{t+1}{2}}\norm{p}^{\frac{1}{2}}_{H^{t+1}(\Omega)}h^{\frac{t}{2}} \norm{p}^{\frac{1}{2}}_{H^{t+1}(\Omega)}\\
= &\norm{\u-r_h\u}_{L^2(\Omega)} + h^{t+1}\norm{p}_{H^{t+1}(\Omega)}.
	\end{align*}
By using Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli}, we get
\begin{align*}
\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h} \lesssim h^{r+1} \norm{\u}_{H^{r+1}(\Omega)} + h^{t+1}\norm{p}_{H^{t+1}(\Omega)},
\end{align*}
with $0\le t\le k$ and $0\le r \le k$.
\end{proof}	


%	\begin{proposition}\label{apriori:prop1_ns}
%	Let $\left(\bm\u,p\right) \in \left[H^{r+1}(\Omega)\right]^d\times H^{k+1}(\Omega)$ and $s:=\min\{r,k-\frac{1}{2},p\}$ be the solution of~\eqref{eq:prob_cont} and $\left(\u_h,p_h\right)\in V_h\times Q_h$ the one to~\eqref{eq:prob_disc_sym} for $m=0$.
%	\begin{equation}\label{apriori:eq5_ns}
%	\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h,?}\lesssim h^{s+1} \left( \norm{\u}_{H^{r+1}(\Omega)} +\norm{p}_{H^{k+1}(\Omega)}\right).
%	\end{equation}	
%\end{proposition}	
%\begin{proof}
%	By Lemma~\ref{apriori:lemma1_ns} and trace inequality for Sobolev spaces
%\begin{align*}
%\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h,?} \lesssim & \norm{\u-r_h\u}_{L^2(\Omega)} + \sum_{f\in\mathcal F_h^\partial}\eps^{-\frac{1}{2}}\norm{p_h-\pi_h p}_{L^2(f)} \\
%\lesssim & \norm{\u-r_h\u}_{L^2(\Omega)} + \sum_{K\in\mathcal T_h} \eps^{-\frac{1}{2}}\norm{p_h-\pi_h p}_{H^1(K)} .
%\end{align*}
%\textcolor{red}{By choosing $\eps = \mathcal O(h^{-1})$} and using Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli}, we get
%\begin{align*}
%\norm{\bm\u_h-r_h\bm\u}_{0,h} + \norm{p_h-\pi_h p}_{1,h,?} \lesssim h^{r+1} \norm{\u}_{H^{r+1}(\Omega)} + h^{k+\frac{1}{2}}\norm{p}_{H^{k+1}(\Omega)},
%\end{align*}
%with $0\le r\le p$ and $0\le k\le p$.
%\end{proof}	

	\begin{proposition}\label{apriori:prop1_pert}
	Let $\left(\bm\u^\eps,p^\eps\right) \in \bm H^{r+1}(\Omega)\times H^{t+1}(\Omega)$ and $s:=\min\{r,k\}$ be the solution of the perturbed continuous problem~\eqref{eq:prob_cont_bis} and $\left(\u_h,p_h\right)\in V_h\times Q_h$ the one to~\eqref{eq:prob_disc_bis}. There exists $C>0$ such that
	\begin{equation}\label{apriori:eq5_pert}
	\norm{\bm\u_h-r_h\bm\u^\eps}_{0,h,\eps} + \norm{p_h-\pi_h p^\eps}_{1,h,\eps}\le C h^{s+1} \norm{\u^\eps}_{H^{s+1}(\Omega)}.
	\end{equation}	
\end{proposition}	
\begin{proof}
	By Lemma~\ref{apriori:lemma1_pert} and Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli}, we get
	\begin{align*}
	\norm{\bm\u_h-r_h\bm\u^\eps}_{0,h,\eps} + \norm{p_h-\pi_h p^\eps}_{1,h,\eps} \lesssim h^{s+1} \norm{\u^\eps}_{H^{s+1}(\Omega)}.
	\end{align*}
\end{proof}	

	\begin{remark}
		Let us remark that the quantities $\norm{\u_h-r_h\u_h}_{0,h}$, $\norm{p_h-\pi_h p}_{1,h}$ in~\eqref{apriori:eq5_m=1} and $\norm{p_h-\pi_h p^\eps}_{1,h,\eps}$, $\norm{\u_h-r_h\u^\eps}_{0,h,\eps}$  in~\eqref{apriori:eq5_pert} respectively are super convergent.
	\end{remark}
%	\begin{theorem}\label{apriori:theorem1_m=0}
%		Let $\left(\bm\u,p\right) \in  \left[H^{r+1}(\Omega)\right]^d\times H^{k+1}(\Omega)$ and $s:=\min\{r,k-\frac{1}{2},p\}$ be the solution to~\eqref{eq:prob_cont} and $\left(\bm\u_h,p_h\right) \in  V_h\times Q_h$ the one to~\eqref{eq:prob_disc_sym} for $m=0$. Then
%		\begin{align*}
%			\norm{\u-\u_h}_{L^2(\Omega)}\lesssim &  h^{s+1}\left( \norm{\bm\u}_{H^{r+1}(\Omega)} + \norm{p}_{H^{k+1}(\Omega)}\right).
%		\end{align*}
%	\end{theorem}
%	\begin{proof}
%		Let us proceed by triangular inequality.
%		\begin{align*}
%			\norm{\u-\u_h}_{L^2(\Omega)} \le \norm{\u-r_h\u}_{L^2(\Omega)}+ \norm{r_h\u-\u_h}_{L^2(\Omega)}.
%		\end{align*}
%		The first and the second terms in the rhs scale as $\mathcal O(h^{r+1})$ and $\mathcal O (h^{s+1})$, respectively, because of Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli} and Proposition~\ref{apriori:prop1_m=0} \textcolor{red}{(not available!)}
%	\end{proof}
	\begin{theorem}\label{apriori:theorem1_m=1}
	Let $\left(\bm\u,p\right) \in  \bm H^{r+1}(\Omega)\times H^{t+1}(\Omega)$ be the solution to~\eqref{eq:prob_cont} and $\left(\bm\u_h,p_h\right) \in  V_h\times Q_h$ the one to~\eqref{eq:prob_disc} with $m=1$. Then there exists $C>0$ such that, for $s:=\min\{r,t,k\}$,
	\begin{align*}
	\norm{\u-\u_h}_{L^2(\Omega)}\le C &  h^{s+1}\left( \norm{\bm\u}_{H^{r+1}(\Omega)} + \norm{p}_{H^{t+1}(\Omega)}\right).
	\end{align*}
\end{theorem}
\begin{proof}
	Let us proceed by triangular inequality.
	\begin{align*}
	\norm{\u-\u_h}_{L^2(\Omega)} \le \norm{\u-r_h\u}_{L^2(\Omega)}+ \norm{r_h\u-\u_h}_{L^2(\Omega)}.
	\end{align*}
	The first and the second terms in the rhs scale as $\mathcal O(h^{r+1})$ and $\mathcal O (h^{s+1})$, respectively, because of Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli} and Proposition~\ref{apriori:prop1_m=1}.
\end{proof}
%	\begin{theorem}\label{apriori:theorem1_ns}
%	Let $\left(\bm\u,p\right) \in  \left[H^{r+1}(\Omega)\right]^d\times H^{k+1}(\Omega)$ and $s:=\min\{r,k-\frac{1}{2},p\}$ be the solution to~\eqref{eq:prob_cont} and $\left(\bm\u_h,p_h\right) \in  V_h\times Q_h$ the one to~\eqref{eq:prob_disc_sym} for $m=0$. Then
%	\begin{align*}
%	\norm{\u-\u_h}_{L^2(\Omega)}\lesssim &  h^{s+1}\left( \norm{\bm\u}_{H^{r+1}(\Omega)} + \norm{p}_{H^{k+1}(\Omega)}\right).
%	\end{align*}
%\end{theorem}
%\begin{proof}
%	Let us proceed by triangular inequality.
%	\begin{align*}
%	\norm{\u-\u_h}_{L^2(\Omega)} \le \norm{\u-r_h\u}_{L^2(\Omega)}+ \norm{r_h\u-\u_h}_{L^2(\Omega)}.
%	\end{align*}
%	The first and the second terms in the rhs scale as $\mathcal O(h^{r+1})$ and $\mathcal O (h^{s+1})$, respectively, because of Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli} and Proposition~\ref{apriori:prop1_ns}.
%\end{proof}
	\begin{lemma}\label{apriori:lemma2_pert}
	Let $\left(\bm\u^\eps,p^\eps\right) \in  \bm H^{r+1}(\Omega)\times H^{t+1}(\Omega)$ be the solution to the perturbed continuous problem~\eqref{eq:prob_cont_bis} and $\left(\bm\u_h,p_h\right) \in  V_h\times Q_h$ the one to~\eqref{eq:prob_disc_bis}. Then there exists $C>0$ such that, for $s:=\min\{r,k\}$,
	\begin{align*}
	\norm{\u^\eps-\u_h}_{L^2(\Omega)}\le C   h^{s+1} \norm{\bm\u^\eps}_{H^{s+1}(\Omega)}.
	\end{align*}
\end{lemma}
\begin{proof}
	Let us proceed by triangular inequality.
	\begin{align*}
	\norm{\u^\eps-\u_h}_{L^2(\Omega)} \le \norm{\u^\eps-r_h\u^\eps}_{L^2(\Omega)}+ \norm{r_h\u^\eps-\u_h}_{L^2(\Omega)}.
	\end{align*}
	The first and the second terms in the rhs scale as $\mathcal O(h^{s+1})$, respectively, because of Bramble-Hilbert/Deny-Lions Lemma~\cite{qvalli} and Proposition~\ref{apriori:prop1_pert}.
\end{proof}
	\begin{theorem}\label{apriori:theorem1_pert}
	Let $\left(\bm\u,p\right) \in  \bm H^{r+1}(\Omega)\times H^{t+1}(\Omega)$ and $s:=\min\{r,k\}$ be the solution to the continuous~\eqref{eq:prob_cont} and $\left(\bm\u_h,p_h\right) \in  V_h\times Q_h$ the one to~\eqref{eq:prob_disc_bis}. Assume $\Omega$ to be convex and with a $C^2$ boundary, $\f\in H^{s+2}(\Omega)$, $g\in H^{s+1}(\Omega)$ and $u_N=0$. Then
	\begin{align*}
	\norm{\u-\u_h}_{L^2(\Omega)}=\mathcal O \left(  h^{s+1} \right).
	\end{align*}
\end{theorem}
\begin{proof}
	Let us proceed by triangular inequality.
	\begin{align*}
	\norm{\u-\u_h}_{L^2(\Omega)} \le & \norm{\u-\u^\eps}_{L^2(\Omega)}+ \norm{\u^\eps-\u_h}_{L^2(\Omega)} \lesssim \eps \norm{p-p_D}_{L^2(\Gamma_N)}+ h^{s+1}\norm{\u^\eps}_{H^{s+1}(\Omega)}\\
	 \lesssim  &  \eps \norm{p-p_D}_{L^2(\Gamma_N)}+ h^{s+1}\left( \norm{\f}_{H^{s+2}(\Omega)} + \norm{g}_{H^{s+1}(\Omega)}  \right).
	\end{align*}
We used Lemma~\ref{apriori:lemma2_pert}, Proposition~\ref{prop:conv_eps}, and finally Proposition~\ref{prop:stability_eps_simple}. Finally, let us choose we just choose $\eps=h^{s+1}$.
\end{proof}

\begin{remark}
We observe that for both formulations,~\eqref{eq:prob_disc} and~\eqref{eq:prob_disc_bis}, no additional tuning of the penalty parameter is required, unlike for the standard Nitsche method for the poisson problem~\cite{STENBERG1995139}.
\end{remark}

%\begin{remark}\label{remark:conditioning}
%Proceeding as in~\cite{ern_guermond_cond} it would be possible to prove that the condition number of the stiffness matrix arising from the discretizations~\eqref{eq:prob_disc}, for both $m\in\{0,1\}$,	scales as $h^{-2}$. The penalty parameter for the weak imposition of the Neumann boundary conditions is the responsible of the deterioration of the condition number with respect to the standard mixed finite element discretization of the Poisson problem where the condition number scales as $h^{-1}$. An even worse situation occurs when formulation~\eqref{eq:prob_disc_bis} is employed. In this case the condition number scales as $h^{-\left(s+2 \right)}$, $s=\min\{r,k\}$, $r$ being the Sobolev regularity of the exact solution for the pressure field and $k$ the polynomial degree of the Raviart-Thomas discretization. What has just been said is confirmed numerically in the case of quadrilateral meshes: see Figures~\ref{num_exp:fig6},~\ref{num_exp:fig7},~\ref{num_exp:fig4},~\ref{num_exp:fig5}.
%\end{remark}	


%\begin{remark}[Well-posedness of the pure Dirichlet case in the unfitted-case]
%It is natural to wonder how to apply or how to generalize any of these methods in the general case of a mesh that is not fitted with the boundary of the computational domain. However, such an extension is by no means trivial and is therefore an ongoing project. In this little remark, nevertheless, we show that if the boundary of the domain that is not fitted with the mesh contains only $\Gamma_D$, then the problem remains well posed. 
%	
%So, let us consider the Darcy problem~\eqref{eq:prob_cont} with pure Dirichlet boundary conditions, i.e., $\Gamma=\Gamma_D$, in a domain whose boundary is not fitted with the underlying mesh. It holds $\overline\Omega\subset\mathcal T_h$, but $\mathcal T_h\not\subset\overline\Omega$, and for all $K\in\mathcal T_h$ we assume that $K\cap\Omega\neq \emptyset$.
%
%Find $\left(\u_h,p_h\right)\in V_h\times Q_h$ such that
%\begin{align}\label{dirichlet:pb2}
%\begin{cases}
%\left(\u_h,\v_h\right)_{L^2(\Omega)} + b_0(\v_h,p_h) = \left(\f,\v_h \right)_\Omega+ \langle p_D,\v_h\cdot\n\rangle_{\Gamma} \qquad&\forall\ \v_h\in V_h, \\
%b_0(\u_h,q_h)  = \left(g,q_h\right)_{\Omega}\qquad&\forall\ q_h\in Q_h.
%\end{cases}
%\end{align}	
%We denote as $\Omega_{\mathcal T}$ the extended domain defined as $\overline\Omega_{\mathcal T}:=\bigcup_{K\in\mathcal T_h}K$. Note that the finite element spaces $V_h$ and $Q_h$ this time are defined on the whole $\Omega_{\mathcal T}$,but with an abuse of notation we still denote $V_h$ and $Q_h$ their restrictions to $\Omega$.	
%In order to study the well-posedness of~\eqref{dirichlet:pb2}, the following standard norms are employed:
%\begin{alignat*}{3}
%\norm{\v_h}_{V_h}:=&\norm{\v_h}_{H(\dive;\Omega)}\qquad &&\forall\ \v_h\in V_h,\\
%\norm{q_h}_{Q_h}:=&\norm {q_h}_{L^2(\Omega)}\qquad &&\forall\ q_h\in Q_h.
%\end{alignat*}
%The continuity of both bilinear forms an  the coercivity of $\left(\cdot,\cdot\right)_{L^2(\Omega)}$ in $\Ker B_0$ ($B_0$ is the linear operator associated to the bilinear form $b_0(\cdot,\cdot)$) follows in a straightforward way.  Moreover, it is easy to show that $b_0(\cdot,\cdot)$ is inf-sup stable. Let us sketch its proof for the sake of completeness.
%\begin{proof}
%Given $q_h\in Q_h$, there exists $\v^q \in \bm H^1_0(\Omega)$ (see~\cite{dangelo_scotti}) such that
%\begin{align*}
%	\begin{cases}	
%		\dive \v^q = q_h \quad \text{in}\;\Omega,\\
%		\restr{\v^q}{\Gamma}=\bm 0,\\
%		\norm{\v^q}_{H^1(\Omega)}\lesssim \norm{q_h}_{L^2(\Omega)}.		
%	\end{cases}		
%\end{align*}	
%Let us define
%\begin{equation*}
%\phi:=
%\begin{cases}
%\dive\v^q	 \qquad&\text{in}\;\Omega,\\
%0 \qquad&\text{in}\;\Omega_{\mathcal T}\setminus \overline\Omega.
%\end{cases}	
%\end{equation*}
%As before, there exists $\tilde\v^q\in\bm H^1_0(\Omega_{\mathcal T})$ such that
%\begin{equation*}
%	\begin{cases}	
%	\dive \tilde\v^q = \phi \quad \text{in}\;\Omega_{\mathcal T},\\
%	\restr{\tilde\v^q}{\partial\Omega_{\mathcal T}}=\bm 0,\\
%	\norm{\tilde\v^q}_{H^1(\Omega_{\mathcal T})}\lesssim \norm{\phi}_{L^2(\Omega_{\mathcal T})} = \norm{q_h}_{L^2(\Omega)}.		
%\end{cases}	
%\end{equation*}
% We denote $\v_h:=\restr{r_h(\tilde \v^q)}{\Omega}\in V_h$ and observe that, by the commutative diagram~\eqref{comm_diag} (which still holds in $\Omega_{\mathcal T}$), $\dive\v_h = \Pi_h \phi$, so $\dive\v_h=q_h$ in $\Omega$ in the sense of $L^2$. In particular, it holds
%\begin{align*}
%	b_0(\v_h,q_h)= &\left(q_h,\dive \v_h \right)_{\Omega} = \norm{q_h}^2_{L^2(\Omega)}.
%\end{align*}
%On the other hand, we have
%\begin{align*}
%	\norm{\v_h}_{H(\dive;\Omega)}\le \norm{r_h(\tilde \v^q)}_{H(\dive;\Omega_{\mathcal T})}\lesssim \norm{\tilde\v^q}_{H(\dive;\Omega_{\mathcal T})} \le 	\norm{\tilde\v^q}_{H^1(\Omega_{\mathcal T})}\lesssim \norm{q_h}_{L^2(\Omega)}.
%\end{align*}
%\end{proof}
%\end{remark}


%\section{Neumann b.c. in the unfitted case using Burman's formulation}
%Find $\left(\u_h,p_h\right)\in \tilde V_h\times\tilde Q_h$ such that
%\begin{align}\label{eq:prob_disc_ns_unfitted}
%	\begin{cases}
%		a_1(\u_h,\v_h) + b_1(\v_h,p_h) =  \eps\langle\u_N,\v_h\cdot\n \rangle\qquad&\forall\ \v_h\in \tilde V_h,\\
%		b_0(\u_h,q_h) =\left(f,q_h\right)_{\Omega}\qquad\qquad\qquad\qquad&\forall\ q_h\in \tilde Q_h.
%	\end{cases}
%\end{align}
%Find $\left(\u_h,p_h\right)\in \tilde V_h\times \tilde Q_h$ such that
%\begin{align}\label{eq:prob_disc_sym_unfitted}
%	\begin{cases}
%		a_1(\u_h,\v_h) + b_m(\v_h,p_h) =  \eps\langle\u_N,\v_h\cdot\n \rangle\qquad&\forall\ \v_h\in \tilde V_h,\\
%		b_m(\u_h,q_h) =\left(f,q_h\right)_{\Omega} - m \langle q_h, \u_N \rangle\qquad\qquad\qquad\qquad&\forall\ q_h\in \tilde Q_h,\quad m\in\{0,1\}.
%	\end{cases}
%\end{align}
%Find $\left(\u_h,p_h\right)\in \tilde V_h\times\tilde Q_h$ such that
%\begin{align}\label{eq:prob_disc_pert_unfitted}
%	\begin{cases}
%		a_1(\u_h,\v_h) + b_0(\v_h,p_h) =  \langle\eps\u_N+p_D,\v_h\cdot\n \rangle\qquad&\forall\ \v_h\in \tilde V_h,\\
%		b_0(\u_h,q_h) =\left(f,q_h\right)_{\Omega} \qquad\qquad\qquad\qquad&\forall\ q_h\in \tilde Q_h.
%	\end{cases}
%\end{align}
%Let us endow our finite element spaces with the following mesh-dependent norms:
%\begin{align*}
%	\norm{\bm{\tau}_h}^2_{0,h}&:= \norm{\bm\tau_h}^2_{L^2(\Omega)} + \sum_{K\in\mathcal T_h} \left(h +\eps \right)\norm{\bm\tau_h\cdot\n}^2_{L^2(\Gamma_K)},  \\
%	\norm{q_h}^2_{1,h}&:= \sum_{K\in\mathcal T_h}\norm{\nabla q_h}^2_{L^2(K\cap\Omega)} + \sum_{f\in\mathcal F_h^i}h^{-1}\norm{ \left[q_h\right]}^2_{L^2(f\cap\Omega)},\\
%	\norm{q_h}^2_{1,h,ks}&:= \sum_{K\in\mathcal T_h}\norm{\nabla q_h}^2_{L^2(K\cap\Omega)} + \sum_{f\in\mathcal F_h^i}h^{-1}\norm{ \left[q_h\right]}^2_{L^2(f\cap\Omega)} +\sum_{K\in\mathcal T_h}\left(h+\eps\right)^{-1}\norm{q_h}_{L^2(\Gamma_K)}^2,
%\end{align*}
%where in the last norm the subscript ``ks'' stands for Konno-Schotzau-Stenberg since it has been introduced in~\cite{konno_robin}.
%\begin{proposition}
%	There exist $M_a, M_{b_m}>0$, $m=0,1$, such that	
%	\begin{align*}	
%		\abs{a_1 (\u_h,\v_h)}	\le M_a \norm{\u_h}_{0,h}\norm{\v_h}_{0,h}\qquad &\forall\ \u_h,\v_h\in \tilde V_h,\\
%		\abs{b_1(\v_h,q_h)} \le  M_{b_1} \norm{\v_h}_{0,h}\norm{q_h}_{1,h}\qquad &\forall\ \v_h\in \tilde V_h,\ q_h\in \tilde Q_h, \\
%		\abs{b_0(\v_h,q_h)} \le  M_{b_0} \norm{\v_h}_{0,h}\norm{q_h}_{1,h,ks}\qquad &\forall\ \v_h\in \tilde V_h,\ q_h\in \tilde Q_h.
%	\end{align*}	
%\end{proposition}	
%\begin{proof}
%	Let $\u_h,\v_h\in \tilde V_h$, $q_h\in \tilde Q_h$ be arbitrary.
%	\begin{align*}
%		\abs{a_1(\u_h,\v_h)}\le \norm{\u_h}_{0,h} \norm{\v_h}_{0,h} + \norm{\eps^{\frac{1}{2}}\v_h\cdot\n}_{L^2(\Gamma)}\norm{\eps^{\frac{1}{2}}\u_h\cdot\n}_{L^2(\Gamma)}\le \norm{\u_h}_{0,h} \norm{\v_h}_{0,h},
%	\end{align*}
%	hence $M_a=1$. By integration by parts, we get
%	\begin{align*}
%		b_1(\v_h,q_h) =& \left(q_h,\dive\v_h\right)_\Omega - \langle q_h,\v_h\cdot\n\rangle_{\Gamma} = \sum_{K\in\mathcal T_h} \left(q_h,\dive \v_h\right)_{K\cap\Omega} - \sum_{K\in\mathcal T_h}\langle q_h,\v_h\cdot\n\rangle_{\Gamma_K}\\
%		=&-\sum_{K\in\mathcal T_h} \left(\nabla q_h,\v_h\right)_{K\cap\Omega} + \sum_{f\in\mathcal F_h^i}\langle \left[q_h \right],\v_h\cdot\n \rangle_{f\cap\Omega}.
%	\end{align*}
%	Thus,
%	\begin{align*}
%		\abs{b_1(\v_h,q_h)}\le& \sum_{K\in\mathcal T_h}\norm{\nabla q_h}_{L^2(K\cap\Omega)}\norm{\v_h}_{L^2(K\cap\Omega)} + \sum_{f\in\mathcal F_h^i} \norm{\mathsf h^{-\frac{1}{2}}\left[q_h\right]}_{L^2(f\cap\Omega)}\norm{\mathsf h^{\frac{1}{2}}\v_h\cdot\n}_{L^2(f\cap\Omega)}
%		\lesssim \norm{\v_h}_{0,h} \norm{q_h}_{1,h}.
%	\end{align*}
%	\textcolor{red}{The last passage holds if we use, instead,
%	\begin{align*}
%	\tilde b_1(\v_h,q_h):=\left(q_h,\dive R_h(\v_h)\right)_{\Omega} - \langle q_h, R_h(\v_h)\cdot\n\rangle_{\Gamma},
%	\end{align*}
%since
%  \begin{align*}
%	h^{\frac{1}{2}} \norm{R_h(\v_h)\cdot\n}_{L^2(f\cap\Omega)}\lesssim \norm{\v_h}_{L^2(K')},
%\end{align*}
%where $f\subset\partial K$ and $K'\in\mathcal N(K)$, so that we have
%  \begin{align*}
%  	\sum_{f\in\mathcal F_h^i}h^{\frac{1}{2}} \norm{R_h(\v_h)\cdot\n}_{L^2(f\cap\Omega)}\lesssim \norm{\v_h}_{L^2(\Omega)}.
%  	\end{align*}}
%	On the other hand,
%	\begin{align*}
%		b_0(\v_h,q_h) =& -\sum_{K\in\mathcal T_h} \left(\nabla q_h,\v_h\right)_{K\cap\Omega} + \sum_{f\in\mathcal F_h^i} \langle \left[q_h\right],\v_h\cdot\n\rangle_{f\cap\Omega}  + \sum_{K\in\mathcal T_h} \langle q_h,\v_h\cdot\n\rangle_{\Gamma_K} \\
%		\le & \sum_{K\in\mathcal T_h} \norm{\nabla q_h}_{L^2(K\cap\Omega)}\norm{\v_h}_{L^2(K\cap\Omega)}+\sum_{f\in\mathcal F_h^i} \norm{h^{-\frac{1}{2}}\left[q_h\right]}_{L^2(f\cap\Omega)}\norm{h^{\frac{1}{2}}\v_h\cdot\n}_{L^2(f\cap\Omega)}\\
%		&+\sum_{K\in\mathcal T_h} \norm{h^{-\frac{1}{2}}q_h}_{L^2(\Gamma_K)}\norm{h^{\frac{1}{2}}\v_h\cdot\n}_{L^2(\Gamma_K)}
%		\lesssim  \norm{\v_h}_{0,h}\norm{q_h}_{1,h,ks}.
%	\end{align*}
%\textcolor{red}{As before, the last passage holds if we use
%\begin{align*}
%\tilde b_0(\v_h,q_h) := \left(q_h,\dive R_h(\v_h)\right)_{\Omega}.	
%\end{align*}	
%}
%\end{proof}
%\begin{proposition}
%There exists $\alpha>0$ such that for every $\v_h\in\tilde V_h$
%\begin{equation*}
%a_1(\v_h,\v_h)\ge\alpha \norm{\v_h}^2_{0,h,\Omega}.
%\end{equation*}	
%\end{proposition}	
%\begin{proof}	
%Let us take $\v_h\in\tilde V_h$ arbitrary and compute
%\begin{align*}
%	a_1(\v_h,\v_h) = &\norm{\v_h}^2_{L^2(\Omega)}+ \eps\norm{\v_h\cdot\n}^2_{L^2(\Gamma)}.
%\end{align*}
%\textcolor{red}{Note that we get stuck here since to go on we should have $h^{\frac{1}{2}}\norm{\v_h\cdot\n}_{L^2(\Gamma)}\lesssim \norm{\v_h}_{L^2(\Omega)}$. If we modify the whole velocity/fluxes space by taking $\tilde V_h^\ast$, then for every $\v_h\in \tilde V_h^\ast$, we have
%\begin{align*}
%	a_1(\v_h,\v_h) = &\norm{\v_h}^2_{L^2(\Omega)}+ \eps\norm{\v_h\cdot\n}^2_{L^2(\Gamma)} 
%	\ge  \frac{1}{2} \norm{\v_h}^2_{L^2(\Omega)} + \frac{1}{2C}\norm{\mathsf h^{\frac{1}{2}}\v_h\cdot\n}_{L^2(\Gamma)} + \eps\norm{\v_h\cdot\n}^2_{L^2(\Gamma)} \\
%	\ge &\tilde C \norm{\v_h}^2_{0,h},
%\end{align*}
%where $\tilde C:=\min\{\frac{1}{2},\frac{1}{2C},1\}=\min\{\frac{1}{2},\frac{1}{2C}\}$.}
%\end{proof}	
%Let us define
%\begin{align*}
%	\mathcal T_h(\Omega_I):=&\{K\in \mathcal T_h: K^\mathrm{o}\cap \Omega_I = K^\mathrm o\}, \\
%	\mathcal F_h^i(\Omega_I):=&\{f\in \mathcal F_h^i: f\cap\Omega_I = f\}, \\
%	\mathcal F_h^\partial(\Omega_I):=&\{f\in \mathcal F_h^\partial: f\cap\overline\Omega_I = f\},
%\end{align*}
%and the mesh-dependent norms 
%\begin{align*}
%	\norm{q_h}^2_{1,h,\Omega_I}&:= \sum_{K\in\mathcal T_h(\Omega_I)} \norm{\nabla q_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i(\Omega_I)} h^{-1}\norm{\left[q_h\right]}^2_{L^2(f)}, \\
%		\norm{q_h}^2_{1,h,ks,\Omega_I}&:= \sum_{K\in\mathcal T_h(\Omega_I)} \norm{\nabla q_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i(\Omega_I)} h^{-1}\norm{\left[q_h\right]}^2_{L^2(f)} +\sum_{f\in\mathcal F_h^\partial(\Omega_I)} \left(h+\eps\right)^{-1}\norm{q_h}^2_{L^2(f)}  .
%\end{align*}
%
%
%\begin{lemma}\label{lemma:stab_press1}
%	There exists $C>0$ such that 
%	\begin{equation*}
%		\norm{q_h}_{1,h}\le C \norm{q_h}_{1,h,\Omega_I}\qquad\forall\ q_h\in R_h(\tilde Q_h).	
%	\end{equation*}	
%\end{lemma}	
%\begin{proof}	
%	If $\Gamma_N\cap\Gamma_{trim}=\emptyset$, then $\Omega=\Omega_I$ and $\norm{q_h}_{1,h}=\norm{q_h}_{1,h,\Omega_I}$, hence let us assume $\Gamma_N\cap\Gamma_{trim}\neq\emptyset$. For every $K\in\mathcal T_h$ we assume that either $K\subset\Omega$, i.e. $K$ is a \emph{good element}, or $K$ is a \emph{bad element} and there exists $K'$, its \emph{good neighbor}, such that $K'\subset\Omega$. In the former case we do not have anything show, in the latter it is possible to prove, see~\cite{puppi},
%	\begin{equation*}
%		\norm{\nabla q_h}_{L^2(K\cap\Omega)}\le C \norm{\nabla q_h}_{L^2(K')}.
%	\end{equation*}
%	Hence,
%	\begin{equation*}
%		\sum_{K\in\mathcal T_h} \norm{\nabla q_h}_{L^2(K\cap\Omega)}\le C \sum_{K'\in\mathcal T_h(\Omega_I)}\norm{\nabla q_h}_{L^2(K')}.
%	\end{equation*}
%	We need to show 
%	\begin{equation*}
%		\sum_{f\in\mathcal F_h^i}\norm{\mathsf h^{-\frac{1}{2}}\left[q_h\right]}_{L^2(f)}\le C \norm{q_h}_{1,h,\Omega_I}.
%	\end{equation*}
%	Let $f\in\mathcal F_h^i$ be arbitrary. The following cases are possible.
%	\begin{enumerate}
%		\item $f\in\mathcal F_h^i(\Omega_I)$. Then it is trivial.
%		\item $f\subseteq \overline K\cap\overline K'$, where $K$ is a \emph{bad element} and $K'$ its \emph{good neighbour}. Then, $\left[q_h\right]_f=0$ by construction of our stabilization, hence we do not have anything to show.
%		\item $f\subseteq K_1\cap K_2$, where both $K_i$, $i=1,2$, are \emph{bad elements}, each one with its \emph{good neighbour} $K_i'$, $i=1,2$, respectively. In this case, we have:
%		\begin{align*}
%			\norm{\mathsf h^{-\frac{1}{2}}[q_h]}_{L^2(f\cap\Omega)}= & \norm{\mathsf h^{-\frac{1}{2}}\left(\restr{q_h}{K_1}-\restr{q_h}{K_2} \right)}_{L^2(f\cap\Omega)} \le C\left( \norm{\nabla q_h}_{L^2(K_1)} + \norm{\nabla q_h}_{L^2(K_2)}\right) \\
%			\le & C\left( \norm{\nabla q_h}_{L^2(K_1')} + \norm{\nabla q_h}_{L^2(K_2')}\right),
%		\end{align*}
%		where in the first inequality we used standard trace and inverse estimates and in the second one the stability property of the stabilized space $R_h(\tilde Q_h)$,
%		\item $f\subseteq K_1\cap K_2$, where $K_1$ is a \emph{bad element} and $K_2$ is a \emph{good element}. We proceed as in the previous case.
%	\end{enumerate}	
%\end{proof}
%\begin{lemma}\label{lemma:stab_press2}
%	There exists $C>0$ such that 
%	\begin{equation*}
%		\norm{q_h}_{1,h,ks}\le C \norm{q_h}_{1,h,ks,\Omega_I}\qquad\forall\ q_h\in R_h(\tilde Q_h).	
%	\end{equation*}	
%\end{lemma}	
%\begin{proof}	
%	If $\Gamma_N\cap\Gamma_{trim}=\emptyset$, then $\Omega=\Omega_I$ and $\norm{q_h}_{1,h,ks}=\norm{q_h}_{1,h,ks,\Omega_I}$, hence let us assume $\Gamma_N\cap\Gamma_{trim}\neq\emptyset$. For every $K\in\mathcal T_h$ we assume that either $K\subset\Omega$, i.e. $K$ is a \emph{good element}, or $K$ is a \emph{bad element} and there exists $K'$, its \emph{good neighbor}, such that $K'\subset\Omega$. Because of the previous Lemma, it is sufficient to show
%	\begin{align*}
%		\sum_{f\in\mathcal F_h^\partial}\left(h+\eps\right)^{-1}\norm{q_h}^2_{L^2(f\cap\Omega)}\lesssim \norm{q_h}^2_{1,h,ks,\Omega_I}.
%	\end{align*}
%	Let $f\in\mathcal F_h^\partial$ be arbitrary.
%	\begin{enumerate}
%		\item If $f\in\mathcal F_h^\partial(\Omega_I)$, then we do not have anything to prove.
%		\item Let $f\subseteq \partial K$ where $K$ is a \emph{bad element} with its \emph{good neighbour} $K'$. Then
%		\begin{align*}
%			\left( h+\eps \right)^{-1}\norm{q_h}^2_{L^2(f\cap\Omega)}\le h^{-1}\norm{q_h}^2_{L^2(f\cap\Omega)}\lesssim \norm{\nabla q_h}^2_{L^2(K)}\lesssim \norm{\nabla q_h}^2_{L^2(K')}.
%		\end{align*}	
%	\end{enumerate}
%\end{proof}
%
%
%\begin{proposition}
%There exists $\beta>0$ such that, for $m=0,1$,
%\begin{equation*}
%\inf_{q_h\in\tilde Q_h}\sup_{\v_h\in\tilde V_h} \frac{b_m(\v_h,q_h)}{\norm{\v_h}_{0,h}\norm{q_h}_{1,h}}\ge\beta.
%\end{equation*}	
%\end{proposition}	
%\begin{proof}
%Let us fix $m=1$ and $p_h\in \tilde Q_h$. We construct $\tilde\u_h\in\tilde V_h$ starting from the RT dofs in the bulk of the domain. Firstly we define $\u_h\in\restr{\tilde V_h}{\Omega_I}$ as 
%\begin{align*}
%\langle \u_h\cdot\n,\varphi_h \rangle_f = \mathsf h^{-1} \langle \left[p_h\right],\varphi_h\rangle_f\qquad&\forall\ f\in\mathcal F_h^i(\Omega_I), \forall\ \varphi_h\in\mathbb P_p(f),\\
%\langle \u_h\cdot\n,\varphi_h \rangle_f =0\qquad&\forall\ f\in\mathcal F_h^{\partial}(\Omega_I), \forall\ \varphi_h\in\mathbb P_p(f),\\
%\left(\u_h,\bm\psi_h\right)_K = - \left(\nabla p_h,\bm\psi_h\right)_K\qquad&\forall\ K\in\mathcal T_h(\Omega_I), \forall\ \bm\psi_h\in\left[ \mathbb P_{p-1}(K)\right]^d, \text{if}\; p>0.
%\end{align*}
%Now, let us extend $\u_h$ to $0$ outside $\Omega_I$ as
%\begin{align*}
%\tilde\u_h:=
%\begin{cases}
%\u_h &\text{in}\;\Omega_I,\\
%0 &\text{in}\;\Omega\setminus\overline{\Omega_I}.
%\end{cases}
%\end{align*}
%Note that $\operatorname{supp}\tilde\u_h\subseteq\Omega_I$ and $\tilde\u_h\in\tilde V_h$. It holds
%\begin{align*}
%b_1(\tilde\u_h,p_h)=&\sum_{K\in\mathcal T_h(\Omega_I)}\left(p_h,\dive\tilde \u_h\right)_K  -\sum_{f\in\mathcal F_h^\partial (\Omega_I)} \langle p_h,\tilde \u_h\cdot\n\rangle_f  \\
% =& -\sum_{K\in\mathcal T_h(\Omega_I)}\left(\nabla p_h,\tilde\u_h\right)_K +\sum_{f\in\mathcal F_h^i(\Omega_I)} \langle \left[p_h\right],\tilde\u_h\cdot\n\rangle_{f} \\
%  =& \sum_{K\in\mathcal T_h(\Omega_I)}\norm{\nabla p_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i(\Omega_I)}h^{-\frac{1}{2}}\norm{ \left[p_h\right]}^2_{L^2(f)}= \norm{p_h}^2_{1,h,\Omega_I}.
%\end{align*}
%By Lemma~\ref{lemma:stab_press1} we have $\norm{p_h}_{1,h}\lesssim \norm{p_h}_{1,h,\Omega_I}$ \textcolor{red}{provided that we use $R_h(\tilde Q_h)$ instead of $\tilde Q_h$.} Since $\operatorname{supp}\tilde\u_h\subseteq\Omega_I$ we can proceed as in Proposition~\ref{prop:infsup_fitted} for the boundary-fitted case in order to show $\norm{\tilde\u_h}_{0,h}\lesssim \norm{p_h}_{1,h}$.
%
%Let us now move to the case $m=0$. For a given $p_h\in\tilde Q_h$, let us construct the corresponding velocity/flux $\tilde \u_h\in\restr{\tilde V_h}{\Omega_I}$ as follows
%\begin{align*}
%\langle \u_h\cdot\n,\varphi_h \rangle_f = \mathsf h^{-1} \langle \left[p_h\right],\varphi_h\rangle_f\qquad&\forall\ f\in\mathcal F_h^i(\Omega_I), \forall\ \varphi_h\in\mathbb P_p(f),\\
%\langle \u_h\cdot\n,\varphi_h \rangle_f =\left(h+\eps\right)^{-1}\langle q_h,\varphi_h\rangle_f\qquad&\forall\ f\in\mathcal F_h^{\partial}(\Omega_I), \forall\ \varphi_h\in\mathbb P_p(f),\\
%\left(\u_h,\bm\psi_h\right)_K = - \left(\nabla p_h,\bm\psi_h\right)_K\qquad&\forall\ K\in\mathcal T_h(\Omega_I), \forall\ \bm\psi_h\in\left[ \mathbb P_{p-1}(K)\right]^d, \text{if}\; p>0.
%\end{align*}
%We have
%\begin{align*}
%b_0(\tilde\u_h,p_h) =& \sum_{K\in\mathcal T_h(\Omega_I)} \left( p_h,\dive\tilde \u_h\right)_K = -\sum_{K\in\mathcal T_h(\Omega_I)} \left( \nabla p_h, \tilde\u_h\right)_K + \sum_{f\in\mathcal F_h^i(\Omega_I)}\langle [p_h],\tilde\u_h\cdot\n\rangle_f +\sum_{f\in\mathcal F^\partial_h(\Omega_I)}\langle p_h,\tilde\u_h\cdot\n\rangle_f\\
%=& \sum_{K\in\mathcal T_h(\Omega_I)}\norm{\nabla p_h}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i(\Omega_I)}h^{-\frac{1}{2}}\norm{ \left[p_h\right]}^2_{L^2(f)} + \sum_{f\in\mathcal F_h^\partial (\Omega_I)} \left( h+\eps\right)^{-1}\norm{p_h}^2_{L^2(f)}= \norm{p_h}^2_{1,h,ks,\Omega_I}.
%\end{align*}
%By Lemma~\ref{lemma:stab_press2} we have $\norm{p_h}_{1,h,ks}\lesssim \norm{p_h}_{1,h,ks,\Omega_I}$ \textcolor{red}{provided that we use $R_h(\tilde Q_h)$ instead of $\tilde Q_h$.} Since $\operatorname{supp}\tilde\u_h\subseteq\Omega_I$ we can proceed as in Proposition~\ref{prop:infsup_fitted} for the boundary-fitted case in order to show $\norm{\tilde\u_h}_{0,h}\lesssim \norm{p_h}_{1,h,ks}$.
%\end{proof}	
%
%
%\begin{theorem}\label{thm:approx}
%	There exists $C>0$ such that for every $\left(\u,q\right)\in  \bm H^{k+1}(\Omega)\times H^{r+1}(\Omega)$, letting $s:=\min\{k+1,r,p\}$, it holds:
%	\begin{equation*}	
%		\begin{aligned}	
%			\norm{\u-\tilde r_{h}\u}_{0,h}+ 	\norm{q-\tilde\pi_h^\ast q}_{1,
%				h}\le C h^{s}\left(\norm{\u}_{H^{k+1}(\Omega)}+\norm{q}_{H^{r+1}(\Omega)} \right).
%		\end{aligned}	
%	\end{equation*}	
%\end{theorem}	
%\begin{proof}
%	For the velocities/fluxes, we proceed by employing the standard approximation properties of $r_{h}$ and the boundedness of the Sobolev-Stein extension operator $E:\bm H^{k+1}(\Omega)\to\bm H^{k+1}(\Omega_{\mathcal T})$. First of all, we need to apply the trace inequality of Lemma~\ref{lemma:disc_trace_ineq}:
%	\begin{align*}
%		\norm{\u-\tilde r_{h}\u}^2_{0,h}= &\norm{\u-\tilde r_{h}\u}^2_{L^2(\Omega)}+ \norm{\mathsf h^{\frac{1}{2}}\left(\u-\tilde r_{h}\u\right)\cdot\n}^2_{L^2(\Gamma)} \le \norm{\u-\tilde r_{h}\u}^2_{L^2(\Omega)}+ \norm{\mathsf h^{\frac{1}{2}}\left(\u-\tilde r_{h}\u\right)}^2_{L^2(\Gamma)}\\
%		\le& \norm{E\u- r_{h}E\u}^2_{L^2(\Omega_{\mathcal T})} +C_T\sum_{K\in\mathcal G_h}\norm{E\u-\tilde r_{h}\u}_{L^2(K)}\norm{\mathsf h D\left(E\u-\tilde r_{h}\u\right)}_{L^2(K)}\\
%		=&Ch^{2k+2}\norm{E\u}^2_{H^{k+1}(\Omega_{\mathcal T})}+C_T\sum_{K\in\mathcal G_h}\norm{E\u-\tilde r_{h}\u}_{L^2(K)}\norm{\mathsf h D\left(E\u-\tilde r_{h}\u\right)}_{L^2(K)}\\
%		\le& C h^{2k+2}\norm{\u}^2_{H^{k+1}(\Omega)} + \norm{E\u-\tilde r_{h}\u}_{L^2(\Omega_{\mathcal T})}\norm{\mathsf hD\left(E\u-\tilde r_{h}\u\right)}_{L^2(\Omega_{\mathcal T})}\le C  h^{2k+2}\norm{\u}^2_{H^{k+1}(\Omega)}.
%	\end{align*}
%	Let us move to the pressures/displacements' case. In the following $E:H^{r+1}(\Omega)\to H^{r+1}(\Omega_{\mathcal T})$ will denote the Sobolev-Stein (scalar) extension operator.
%	\begin{align}
%		\norm{q-\tilde \pi^\ast_{h} q}^2_{1,h}=	\sum_{K\in\mathcal T_h}\norm{\nabla\left(q-\tilde \pi^\ast_{h} q\right)}^2_{L^2(K)} + \sum_{f\in\mathcal F_h^i} \norm{\mathsf h^{-{\frac{1}{2}}}\left[q-\tilde \pi^\ast_{h} q\right]}^2_{L^2(f\cap\Omega)}. \label{eq:interp_press}
%	\end{align}	
%	For the volumetric term one we may proceed as in the case of the fluxes. Let us focus on the ``jump part'' of~\eqref{eq:interp_press} and take $f\in\mathcal F_h^i$ arbitrary. There are few cases to be investigated.
%	\begin{itemize}
%\item Let $f\in\mathcal F_h^i(\Omega_I)$ such that $f=K_1\cap K_2$ with both $K_i$, $i=1,2$, \emph{good elements}. Then we have
%\begin{align*}	
%\norm{\mathsf h^{-{\frac{1}{2}}}\left[q-\tilde \pi^\ast_{h} q\right]}_{L^2(f\cap\Omega)} = 	&
%\norm{\mathsf h^{-{\frac{1}{2}}}\left(\restr{\left(q-\tilde \pi^\ast_{h} q\right)}{K_1}-\restr{\left(q-\tilde \pi^\ast_{h} q\right)}{K_2}\right)}_{L^2(f)} \\
%\le & \norm{\mathsf h^{-\frac{1}{2}}\left(q- \pi_{h} q\right)}^{\frac{1}{2}}_{L^2(K_1)}\norm{\nabla\left(q- \pi_{h} q\right)}^{\frac{1}{2}}_{L^2(K_1)}  +\norm{\mathsf h^{-\frac{1}{2}}\left(q- \pi_{h} q\right)}^{\frac{1}{2}}_{L^2(K_2)}\norm{\nabla\left(q-\pi_{h} q\right)}^{\frac{1}{2}}_{L^2(K_2)} \\
%\le & Ch^{r}\left(\norm {q}_{L^2(K_1)}+\norm{q}_{L^2(K_2)} \right).
%\end{align*}	
%\item $f=K\cap K'$, where $K$ is a \emph{bad element} and $K'$ its \emph{good neighbour}.
%\begin{align*}
%	\norm{\mathsf h^{-{\frac{1}{2}}}\left[q-\tilde \pi^\ast_{h} q\right]}_{L^2(f)} = 	&
%	\norm{\mathsf h^{-{\frac{1}{2}}}\left(\restr{\left(q-\tilde \pi^\ast_{h} q\right)}{K}-\restr{\left(q-\tilde \pi^\ast_{h} q\right)}{K'}\right)}_{L^2(f)} \\
%	\le & \underbrace{\norm{\mathsf h^{-{\frac{1}{2}}}\restr{\left(q-\tilde \pi^\ast_{h} q\right)}{K}}_{L^2(f)}}_{\RomanNumeralCaps 1}+\underbrace{\norm{\mathsf h^{-{\frac{1}{2}}}\restr{\left(q-\tilde \pi^\ast_{h} q\right)}{K'}}_{L^2(f)}}_{\RomanNumeralCaps 2} .
%\end{align*}
%Let us focus on $\RomanNumeralCaps 1$. We add and subtract $p:=\mathcal E_{K',K}\left(\Pi_{K'}\left(q \right) \right)\in\mathbb Q_p (K\cup K')$.
%\begin{align*}
%\RomanNumeralCaps 1 \le \underbrace{\norm{\mathsf h^{-\frac{1}{2}} \left( E(q)-p \right)}_{L^2(f)}}_{\RomanNumeralCaps 1 A} + \underbrace{\norm{\mathsf h^{-\frac{1}{2}} \left( p-\tilde \pi_h^\ast q \right)}_{L^2(f)}}_{\RomanNumeralCaps 1 B}.
%\end{align*}
%We have
%\begin{align*}
%\RomanNumeralCaps 1 A \le \norm{\mathsf h^{-\frac{1}{2}} \left( E(q) - \mathcal E_{K',K} \left( \Pi_{K'}\left(q \right) \right) \right)}^{\frac{1}{2}}_{L^2(K)}	\norm{\nabla\left( E(q) - \mathcal E_{K',K} \left( \Pi_{K'}\left(q \right) \right) \right)}^{\frac{1}{2}}_{L^2(K)}	\le C h^r \norm{E(q)}_{H^{r+1}(K)}.
%\end{align*}	
%Note that $\restr{\tilde \pi_h^\ast q}{K}=R_K^p \left( \tilde \pi_h q \right)$ and $\restr{p}{K}=R_K^p\left(p\right)$, hence
%\begin{align*}
%\RomanNumeralCaps 1 B = \norm{\mathsf h^{-\frac{1}{2}} R_K^p \left(q-\tilde \pi_h q\right)}_{L^2(f)} \le C \norm{\nabla \left( q-\tilde \pi_h q \right)}_{L^2(K')} \le C h^r \norm{q}_{H^{r+1}(K')}.
%\end{align*}
%\item $f = K_1\cap K_2$ where $K_i$, $i=1,2$, are both \emph{bad elements} with \emph{good neighbours} $K_i'$, $i=1,2$, respectively.
%\begin{align*}
%\norm{\mathsf h^{-{\frac{1}{2}}}\left[q-\tilde \pi^\ast_{h} q\right]}_{L^2(f\cap\Omega)} = 	&\norm{\mathsf h^{-\frac{1}{2}} \left( \restr{\left(q-\tilde \pi^\ast_h q \right)}{K_1} - \restr{\left( q-\tilde \pi^\ast_h q\right)}{K_2} \right)}_{L^2(f)}	\\
%\le & \underbrace{\norm{\mathsf h^{-\frac{1}{2}} \restr{\left(q-\tilde \pi^\ast_h q \right)}{K_1}}_{L^2(f)}}_{\RomanNumeralCaps 3} +\underbrace{\norm{\mathsf h^{-\frac{1}{2}}\restr{\left( q-\tilde \pi^\ast_h q\right)}{K_2} }_{L^2(f)}}_{\RomanNumeralCaps 4}.
%\end{align*}	
%We can deal with $\RomanNumeralCaps 3$ and $\RomanNumeralCaps 4$ as with $\RomanNumeralCaps 1$ above.
%	\end{itemize}
%\end{proof}	
%Let us focus on the following formulation. Find $(\u_h,p_h)\in \tilde V_h^\ast \times \tilde Q_h^\ast$ such that
%\begin{align}\label{eq:prob_disc_sym_unfitted_final}
%\begin{cases}
%a_1(\u_h,\v_h) + b_1(\v_h,p_h) = \eps\langle \u_N,\v_h\cdot\n \rangle_{\Gamma}\qquad&\forall\ \v_h\in \tilde V_h^\ast,\\
%b_1(\u_h, q_h) = \left(f,q_h\right)_\Omega - \langle q_h,\u_N\rangle_\Gamma\qquad&\forall\ q_h\in \tilde Q_h^\ast.
%\end{cases}
%\end{align}
%\begin{lemma}\label{lemmaPD}
%	Let $\left(\u,p\right)\in \bm H(\dive;\Omega)\times L^2(\Omega)$ and $\left(\u_h,p_h\right)\in \tilde V_h^\ast \times \tilde Q_h^\ast$  be the solutions to the strong and discrete problems~\eqref{eq:prob_cont} and~\eqref{eq:prob_disc_sym_unfitted_final}, respectively. Then, for every $\left(\u_I,p_I \right)\in \tilde V_h^\ast\times \tilde Q_h^\ast$ the following estimates hold.
%	\begin{align*}
%		\norm{\u_h - \u_I}_{0,h} \le& \frac{1}{\alpha}\left(M_a \norm{\u-\u_I}_{0,h} + M_{b_1}\norm{p-p_I}_{1,h}  \right)
%		+ \frac{1}{\beta_1} \left(\frac{M_a}{\alpha}+1\right) M_{b_1}\norm{\u-\u_I}_{0,h}, \\
%		\norm{p_h-p_I}_{1,h} \le & \frac{1}{\beta_1}\left(1+\frac{M_a}{\alpha} \right) \left(M_a \norm{\u-\u_I}_{0,h} + M_{b_1}\norm{p-p_I}_{1,h} \right) 
%		+ \frac{M_a}{\beta^2_1}\left(\frac{M_a}{\alpha}+1\right) M_{b_1}\norm{\u-\u_I}_{0,h}.
%	\end{align*}
%\end{lemma}
%\begin{proof}
%	Let $\left(\u_I,p_I\right)\in\tilde V_h^\ast\times\tilde Q_h^\ast$ be arbitrary. By linearity and consistency $\left(\u_h-\u_I,p_h-p_I \right)\in \tilde V_h^\ast\times \tilde Q_h^\ast$ satisfies the saddle point problem
%	\begin{equation*}
%		\begin{cases}
%			 a_1(\u_h - \u_I,\v_h) + b_1(\v_h,p_h-p_I) =  F(\v_h) \qquad&\forall\ \v_h\in\tilde V_h^\ast,\\
%			b_1(\u_h-\u_I,q_h) =  G_1(q_h)&\forall\ q_h\in \tilde Q_h^\ast,
%		\end{cases}
%	\end{equation*}
%	where
%	\begin{alignat*}{3}
%		 F(\v_h):= & a_1(\u-\u_I,\v_h) + b_1(\v_h,p-p_I)\qquad&&\forall\ \v_h\in\tilde V_h^\ast,\\
%		 G_1(q_h):=&b_1(\u-\u_I,q_h)&&\forall\ q_h\in \tilde Q_h^\ast.
%	\end{alignat*}
%The following stability estimates hold (we refer to~\cite{brezzi_boffi}):
%	\begin{align*}
%		\norm{\u_h - \u_I}_{0,h} \le &\frac{1}{\alpha}\norm{F}_{V'_h}+ \frac{1}{\beta_1} \left(\frac{M_a}{\alpha}+1\right) M_{b_1}\norm{ G_1}_{Q'_h}, \\
%		\norm{p_h-p_I}_{1,h} \le & \frac{1}{\beta_1}\left(1+\frac{M_a}{\alpha} \right) \norm{F}_{V'_h} 
%		+ \frac{M_a}{\beta^2_1}\left(\frac{M_a}{\alpha}+1\right) \norm{G_1}_{Q'_h}.
%	\end{align*}
%	We conclude since, by definition of dual norm, we have
%	\begin{align*}
%		\norm{F}_{V'_h} = &M_a\norm{\u-\u_I}_{0,h}+M_{b_1}\norm{p-p_I}_{1,h}, \\
%		\norm{ G_1}_{Q'_h} = &M_{b_1}\norm{\u-\u_I}_{0,h}.
%	\end{align*}
%\end{proof}
%\begin{theorem}
%	Let $\left(\u,p\right)\in \bm H^{k+1}\left(\Omega\right)\times H^{r+1}\left(\Omega\right)$ be the solution of the strong problem~\eqref{eq:prob_cont}. Then, the finite element solution $\left(\u_h,p_h\right)\in \tilde V_h^\ast\times \tilde Q_h^\ast$ of~\eqref{eq:prob_disc_sym_unfitted_final} satisfies, for $s:=\min\{k+1,r,p\}$,
%	\begin{equation*}
%		\norm{\u-\u_h}_{0,h}+\norm{p-p_h}_{1,h} \le C h^{s} \left(\norm{\u}_{H^{k+1}(\Omega)} + \norm{p}_{H^{r+1}(\Omega)}  \right).
%	\end{equation*}
%\end{theorem}	
%%\begin{remark}
%%Note that if the data $\f$ is regular enough, then the Darcy law (first equation of \eqref{strong_pb2}) implies $\u\in H^s \to p\in H^{s+1}$. This behaviour of the analytical solution is reflected from the numerical point of view in a \emph{super convergence} of the solution for the pressure. \textcolor{red}{To be investigated.}
%%\end{remark}
%\begin{proof}
%	Given $\left(\u_I,p_I \right)\in\tilde V_h^\ast\times \tilde Q_h^\ast$, we proceed by triangular inequality:
%	\begin{align}\label{eq:apriori1}
%		\norm{\u-\u_h}_{0,h}\le& \norm{\u-\u_I}_{0,h}+\norm{\u_h-\u_I}_{0,h},\\
%		\norm{p-p_h}_{1,h}\le & \norm{p-p_I}_{1,h}+ \norm{p_h-p_I}_{1,h}.	
%	\end{align}	
%	Using Lemma~\ref{lemmaPD}, we obtain:
%	\begin{align*}
%		\norm{\u-\u_h}_{0,h}\le&  \norm{\u-\u_I}_{0,h}+\frac{1}{\alpha}\left(M_a \norm{\u-\u_I}_{0,h} + M_{b_1}\norm{p-p_I}_{1,h}  \right)\\
%		& + \frac{1}{\beta_1} \left(\frac{M_a}{\alpha}+1\right) M_{b_1}\norm{\u-\u_I}_{0,h},\\
%		\norm{p-p_h}_{1,h}\le &\norm{p_h-p_I}_{1,h} +\frac{1}{\beta_1}\left(1+\frac{M_a}{\alpha} \right) \left(M_a \norm{\u-\u_I}_{0,h} + M_{b_1}\norm{p-p_I}_{1,h} \right) \\
%		&+ \frac{M_a}{\beta_1^2}\left(\frac{M_a}{\alpha}+1\right) M_{b_1}\norm{\u-\u_I}_{0,h}.
%	\end{align*}
%	Let us choose $\u_I:=\tilde r_{h}\u$ and $p_I:=\tilde\pi^\star_h p$ so that by Theorem~\ref{thm:approx}, we obtain
%	\begin{align*}
%		\norm{\u-\u_h}_{0,h}\le& C h^{k}\left(\norm{\u}_{H^{k+1}(\Omega)} \right)
%		+\frac{1}{\alpha}\max\{M_a, M_{b_1}\}C h^{s}\left(\norm{\u}_{H^{k+1}(\Omega)} +\norm{p}_{H^{r+1}(\Omega)}\right)\\
%		& + \frac{1}{\beta_1} \left(\frac{M_a}{\alpha}+1\right) M_{b_1} C h^{k+1}\norm{\u}_{H^{k+1}(\Omega)} ,\\
%		\norm{p-p_h}_{1,h}\le &C h^{r+1}\norm{p}_{H^{r+1}(\Omega)} +\frac{1}{\beta_1}\left(1+\frac{M_a}{\alpha} \right) \max\{M_a, M_{b_1}\}
%		C h^{s}\left(\norm{\u}_{H^{k+1}(\Omega)} +\norm{p}_{H^{r+1}(\Omega)} \right) \\
%		&+ \frac{M_a}{ \beta^2_1}\left(\frac{M_a}{\alpha}+1\right) M_{b_1}Ch^{k+1}\norm{\u}_{H^{k+1}(\Omega)}.
%	\end{align*}
%\end{proof}	
%\section{Robin b.c. in the unfitted case using Stenberg's formulation}
%\textcolor{red}{Nothing yet...}
